Sparsity enforcing priors in inverse problems via Normal variance mixtures: model selection, algorithms and applications

The sparse structure of the solution for an inverse problem can be modelled using different sparsity enforcing priors when the Bayesian approach is considered. Analytical expression for the unknowns of the model can be obtained by building hierarchical models based on sparsity enforcing distributions expressed via conjugate priors. We consider heavy tailed distributions with this property: the Student-t distribution, which is expressed as a Normal scale mixture, with the mixing distribution the Inverse Gamma distribution, the Laplace distribution, which can also be expressed as a Normal scale mixture, with the mixing distribution the Exponential distribution or can be expressed as a Normal inverse scale mixture, with the mixing distribution the Inverse Gamma distribution, the Hyperbolic distribution, the Variance-Gamma distribution, the Normal-Inverse Gaussian distribution, all three expressed via conjugate distributions using the Generalized Hyperbolic distribution. For all distributions iterative algorithms are derived based on hierarchical models that account for the uncertainties of the forward model. For estimation, Maximum A Posterior (MAP) and Posterior Mean (PM) via variational Bayesian approximation (VBA) are used. The performances of resulting algorithm are compared in applications in 3D computed tomography (3D-CT) and chronobiology. Finally, a theoretical study is developed for comparison between sparsity enforcing algorithms obtained via the Bayesian approach and the sparsity enforcing algorithms issued from regularization techniques, like LASSO and some others.

==> Subsec_Prior_GenHyperbolic.tex <==
\subsection{Generalized Hyperbolic prior: expressed via conjugate priors}
\label{Subsec:GenHyperbolicPrior}
In the following, we present how the Generalized Hyperbolic distribution, a sparsity enforcing prior because of its heavy-tailed form for different structures of the parameters, can be expressed via conjugate priors, namely the Normal distribution and the generalized Inverse Gaussian distribution.
\\
For this part of the work, the following resources were used:
\\
\textcolor{americanrose}{$\left[ 3 \right]$ \textbf{Location and scale mixtures of Gaussians with flexible tail behaviour: Properties, inference and application to multivariate clustering} - D. WRAITH, F. FORBES, Computational Statistics and Data Analysis 90 (2015) 61-73, 30 April 2015.}
\\
The generalised Hyperbolic distribution ($\Gc\Hc$), introduced by Ole Barndorff-Nielsen, is a continuous probability distribution defined as the normal variance-mean mixture where the mixing distribution is the generalized Inverse Gaussian ($\Gc\Ic\Gc$) distribution. Its probability density function is given in terms of modified Bessel function of the second kind, $\Kc_{\lambda}$.
\\
A random variable has a generalized Hyperbolic $\Gc\Hc(x|\lambda,\alpha,\beta,\delta,\mu,\gamma)$ distribution if its probability density function is:
\beq
\Gc\Hc(x|\lambda,\alpha,\beta,\delta,\mu) 
= 
\frac{\left(\frac{\gamma}{\delta}\right)^{\lambda}}{\sqrt{2\pi}\Kc_{\lambda} \left( \delta \gamma \right)}
\;
\frac{\Kc_{\lambda-\frac{1}{2}} \left( \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} \right)}{\left( \sqrt{ \delta^2 + \left( x - \mu \right)^2} / \alpha \right)^{\frac{1}{2}-\lambda}}
\;
\exp \left\lbrace {\beta \left( x - \mu \right)} \right\rbrace
, 
\lambda, \alpha, \beta, \delta, \mu \in \mathbb{R}, \gamma = \sqrt{\alpha^2-\beta^2};
\label{Eq:GenHyperbolicDistribution}
\eeq
We start with the linear model expressed in Equation~\eqref{Eq:LinearModel}. We consider the Generalized Hyperbolic Prior Model (GHPM), Equation~\eqref{Eq:GHPM1}, which considers a  Normal distribution for $\rf_\rj|\rv_{\rf_\rj}$ with the mean $\mu + \beta \rv_{\rf_\rj}$ and variance $\rv_{\rf_\rj}$. The variance $\rv_{\rf_\rj}| \gamma^2, \; \delta^2, \; \lambda$ is modelled as a generalized Inverse Gaussian distribution, with the corresponding parameters $\gamma^2$, $\delta^2$, and $\lambda$:
\beq
\textbf{GHPM:}\;\;\;\;\;\;\;
\left\{\barr{ll}
p(\rf_\rj | \mu, \; \rv_{\rf_\rj}, \; \beta)
=
\Nc\left(\rf_\rj|\mu + \beta \rv_{\rf_\rj}, \; \rv_{\rf_\rj}\right) 
=
\left( 2 \pi \right)^{-\frac{1}{2}} \; \rv_{\rf_\rj}^{-\frac{1}{2}} \; \exp \left\lbrace -\frac{1}{2}\frac{\left( x - \mu - \beta \rv_{\rf_\rj} \right)^2}{\rv_{\rf_\rj}} \right\rbrace
\\[7pt]
p(\rv_{\rf_\rj}|\gamma^2, \; \delta^2, \; \lambda) 
=
\Gc\Ic\Gc(\rv_{\rf_\rj}|\gamma^2, \; \delta^2, \; \lambda)
=
\frac{\left(\frac{\gamma}{\delta}\right)^{\lambda}}{2\Kc_{\lambda} \left( \delta \gamma \right)}
\;
\rv_{\rf_\rj}^{\lambda-1}
\;
\exp \left\lbrace -\frac{1}{2} \left( \gamma^2 \rv_{\rf_\rj} + \delta^2 \rv_{\rf_\rj}^{-1} \right) \right\rbrace,\\[4pt]
\earr\right.
\label{Eq:GHPM1}
\eeq
The expression of the joint probability distribution $\rf_\rj,\rv_{\rf_\rj}| \mu, \; \beta, \; \gamma^2, \; \delta^2, \; \lambda$ is given by Equation~\eqref{Eq:JointGHPM1},
\beq
p\left( \rf_\rj,\rv_{\rf_\rj}| \mu, \; \beta, \; \gamma^2, \; \delta^2, \; \lambda \right) = \Nc\left(\rf_\rj|\mu + \beta \rv_{\rf_\rj}, \; \rv_{\rf_\rj}\right) \; \Gc\Ic\Gc(\rv_{\rf_\rj}|\gamma^2, \; \delta^2, \; \lambda),
\label{Eq:JointGHPM1}
\eeq 
so the marginal is, Equation~\eqref{Eq:MargGHPM1}:
\beq
p(\rf_\rj|\mu, \beta, \gamma^2, \delta^2, \lambda)
=
\frac{\left(\frac{\gamma}{\delta}\right)^{\lambda}}{2 \sqrt{2 \pi} \Kc_{\lambda} \left( \delta \gamma \right)}
\;
\int
\rv_{\rf_\rj}^{\lambda-\frac{3}{2}}
\;
\exp \left\lbrace -\frac{1}{2} \left( \frac{\left( \rf_\rj - \mu - \beta \rv_{\rf_\rj} \right)^2}{\rv_{\rf_\rj}} + \gamma^2 \rv_{\rf_\rj} + \delta^2 \rv_{\rf_\rj}^{-1} \right) \right\rbrace
\;
\d \rv_{\rf_\rj}
\label{Eq:MargGHPM1}
\eeq 
For solving Equation~\eqref{Eq:MargGHPM1} we can identify a $\Gc\Ic\Gc$ inside the integral: 
\beq
\begin{split}
I 
=&
\exp \left\lbrace \beta \left( \rf_\rj - \mu \right) \right\rbrace 
\int
\rv_{\rf_\rj}^{\left( \lambda-\frac{1}{2} \right) -1} 
\exp \left\lbrace -\frac{1}{2} \left(\left[ \beta^{2} + \gamma^{2} \right] \rv_{\rf_\rj} + \left[ \delta^2 + \left( \rf_\rj-\mu \right)^{2} \right] \rv_{\rf_\rj}^{-1} \right) \right\rbrace \d \rv_{\rf_\rj}
\\
=&
\exp \left\lbrace \beta \left( \rf_\rj - \mu \right) \right\rbrace  
\frac{2\Kc_{\lambda-\frac{1}{2}}\sqrt{\left( \beta^{2} + \gamma^{2} \right) \left( \delta^2 + \left(\rf_\rj-\mu \right)^{2} \right)}}{\left( \frac{ \beta^{2} + \gamma^{2} }{ \delta^2 + \left(\rf_\rj-\mu \right)^{2}}\right)^{\frac{\lambda}{2}-\frac{1}{4}}} 
\underbrace{\int \Gc\Ic\Gc \left( \rv_{\rf_\rj} | \lambda-\frac{1}{2}, \left[ \beta^{2} + \gamma^{2} \right], \left[ \delta^2 + \left(\rf_\rj-\mu \right)^{2} \right] \right) \d \rv_{\rf_\rj}}_{1}
\end{split}
\label{Eq:LapIntegral2}
\eeq 
Introducing the notations:
\beq
\alpha^{2} = \beta^{2} + \gamma^{2} 
\;\;\;\; ; \;\;\;\;
q(\rf_\rj)^{2} = \delta^{2} + \left(\rf_\rj-\mu \right)^{2},
\label{Eq:Notat_GHPM1} 
\eeq
the marginal from Equation~\eqref{Eq:MargGHPM1} can be written as:
\beq
p(\rf_\rj|\mu, \beta, \gamma^2, \delta^2, \lambda)
= 
\frac{\left(\frac{\gamma}{\delta}\right)^{\lambda}}{\sqrt{2 \pi} \Kc_{\lambda} \left( \delta \gamma \right)}
\;
\frac{\Kc_{\lambda-\frac{1}{2}}\sqrt{ \alpha q(\rf_\rj) }}{\left( \frac{q(\rf_\rj)}{\alpha}\right)^{\frac{1}{2}-\lambda}} 
\;
\exp \left\lbrace \beta \left( \rf_\rj - \mu \right) \right\rbrace 
\label{Eq:MargGHPM1_1}
\eeq 
Introducing between the parameters the parameter $\alpha$ and excluding the parameter $\gamma$, considering as parameters $\delta$ instead of $\delta^2$ and reordering the parameters we obtain:
\beq
p(\rf_\rj|\lambda, \alpha, \beta, \delta, \mu)
= 
\frac{\left(\frac{\gamma}{\delta}\right)^{\lambda}}{\sqrt{2 \pi} \Kc_{\lambda} \left( \delta \gamma \right)}
\;
\frac{\Kc_{\lambda-\frac{1}{2}}\sqrt{ \alpha q(\rf_\rj) }}{\left( \frac{q(\rf_\rj)}{\alpha}\right)^{\frac{1}{2}-\lambda}} 
\;
\exp \left\lbrace \beta \left( \rf_\rj - \mu \right) \right\rbrace,  \gamma = \sqrt{\alpha^{2} - \beta^{2}}  
\label{Eq:MargGHPM1_2}
\eeq 
The interest of this distribution is that is of a very general form, being the superclass of, among others, the Student-t ($\Sc t - t$) distribution for the particular set of parameters $\Gc\Hc \left( -\frac{\nu}{2}, 0, 0, \sqrt{\nu}, \mu \right)$ - Subsection~\eqref{Subsubsec:GenHyperbolicAsStt}, the Hyperbolic ($\Hc$) distribution for the particular set of parameters $\Gc\Hc(x|\lambda = 1,\alpha,\beta,\delta,\mu) $ - Subsection~\eqref{Subsubsec:GenHyperbolicAsHyp}, the Laplace ($\Lc$) distribution for the particular set of parameters $\Gc\Hc(x|\lambda = 1, \alpha = b^{-1}, \beta = 0, \delta \searrow  0, \mu) $ - Subsection~\eqref{Subsubsec:GenHyperbolicAsLap}, the variance-gamma ($\Vc\Gc$) distribution for the particular set of parameters $\Gc\Hc(x|\lambda,\alpha,\beta,\delta \searrow 0,\mu)$ - Subsection~\eqref{Subsubsec:GenHyperbolicAsVarGam}, the Normal-Inverse Gaussian ($\Nc\Ic\Gc$) distribution $\Gc\Hc(x|\lambda,\alpha=-\frac{1}{2},\beta,\delta,\mu)$ - Subsection~\eqref{Subsubsec:GenHyperbolicAsNIG}. %the Normal-Inverse Gamma ($\Nc\Ic\Gc am$) distribution for the particular set of parameters $\Gc\Hc(x|?,?,?,?,?)$ - Subsection~\eqref{Subsubsec:GenHyperbolicAsNIGamma}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Subsub: Generalized Hyperbolic as Student-t %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Generalized Hyperbolic: Student-t distribution}
\label{Subsubsec:GenHyperbolicAsStt}
$X \sim \Gc\Hc(x|\lambda = \frac{-\nu}{2},\alpha \searrow 0,\beta = 0, \delta = \sqrt{\nu},\mu)$ has a Student's t-distribution with $\nu$ degrees of freedom, $\Sc t-t \left( x | \mu, \nu \right)$.\\ 
Fixing the asymmetry parameter $\beta = 0$, as an immediate consequence $\gamma=\alpha$ and $\exp \left\lbrace \beta \left( x - \mu \right) \right\rbrace = 1$. The particular case of the probability density function is:
\beq
\Gc\Hc(x|\lambda,\alpha,\beta=0,\delta,\mu) 
= 
\frac{\left(\frac{\alpha}{\delta}\right)^{\lambda}}{\sqrt{2\pi}\Kc_{\lambda} \left( \alpha \delta \right)}
\;
\frac{\Kc_{\lambda-\frac{1}{2}} \left( \alpha \delta \sqrt{ 1 + \frac{ \left( x - \mu \right)^2}{\delta^2}} \right)}{\left( \delta \sqrt{ 1 + \frac{\left( x - \mu \right)^2}{\delta^2}} / \alpha \right)^{\frac{1}{2}-\lambda}}.
\label{Eq:GenHyperbolicDistributionAsStudent}
\eeq 
Fixing $\delta^2 = \nu$ and considering $\alpha \searrow 0$, the particular case of the probability density function is:
\beq
\begin{split}
\Gc\Hc(x|\lambda,\alpha \searrow 0,\beta = 0, \delta = \sqrt{\nu},\mu) 
&= 
\frac{1}{\sqrt{2\pi}}
\left(\frac{\alpha}{\sqrt{\nu}}\right)^{\lambda}
\left( \frac{\sqrt{\nu}}{\alpha} \sqrt{ 1 + \frac{\left( x - \mu \right)^2}{\nu}} \right)^{\lambda-\frac{1}{2}}
\;
\frac{\Kc_{\lambda-\frac{1}{2}} \left( \alpha \sqrt{\nu} \sqrt{ 1 + \frac{ \left( x - \mu \right)^2}{\nu}} \right)}{\Kc_{\lambda} \left( \alpha \sqrt{\nu} \right)}
\\
&= 
\frac{1}{\sqrt{2\pi}}
\left(\frac{\alpha}{\sqrt{\nu}}\right)^{\frac{1}{2}}
\left( 1 + \frac{\left( x - \mu \right)^2}{\nu} \right)^{\frac{1}{2} \left( \lambda - \frac{1}{2} \right)}
\;
\frac{\Kc_{\lambda-\frac{1}{2}} \left( \alpha \sqrt{\nu} \sqrt{ 1 + \frac{ \left( x - \mu \right)^2}{\nu}} \right)}{\Kc_{\lambda} \left( \alpha \sqrt{\nu} \right)}.
\end{split}
\label{Eq:GenHyperbolicDistributionAsStudent1}
\eeq
Since we considered $\alpha \searrow 0 $, for both arguments of the modified Bessel functions of the second kind appearing in Equation~\eqref{Eq:GenHyperbolicDistributionAsStudent1} we have $ \alpha \sqrt{\nu} \sqrt{ 1 + \frac{ \left( x - \mu \right)^2}{\nu}} \searrow 0 $ and $ \alpha \sqrt{\nu} \searrow 0 $ so for computing the values of the two modified Bessel functions of the second kind we can use the asymptotic relations for small arguments:
\beq
\begin{split}
\Kc_{\lambda}\left( x \right) &\sim \Gamma \left( \lambda \right) \; 2^{\lambda-1} \; x^{-\lambda}, \; \mbox{as} \; x \searrow 0 \; \mbox{and} \; \lambda > 0
\\
\Kc_{\lambda}\left( x \right) &\sim \Gamma \left( - \lambda \right) \; 2^{-\lambda-1} \; x^{\lambda}, \; \mbox{as} \; x \searrow 0 \; \mbox{and} \; \lambda < 0.
\end{split}
\label{Eq:ModifiedBesselAsymptoticRelation}
\eeq
We have:
\beq
\begin{split}
\Kc_{\lambda-\frac{1}{2}} \left( \alpha \sqrt{\nu} \sqrt{ 1 + \frac{ \left( x - \mu \right)^2}{\nu}} \right) &= \Gamma \left( \frac{1}{2} - \lambda \right) 2^{-\lambda + \frac{1}{2} - 1} \left( \alpha \sqrt{\nu} \right)^{\lambda - \frac{1}{2}} \left( 1 + \frac{\left( x - \mu \right)^2}{\nu} \right)^{\frac{1}{2}\left(\lambda - \frac{1}{2}\right)}
\\
\Kc_{\lambda} \left( \alpha \sqrt{\nu} \right) &= \Gamma \left( - \lambda \right) 2^{-\lambda - 1} \left( \alpha \sqrt{\nu} \right)^{\lambda} 
\end{split}
\label{Eq:ModifiedBesselValues}
\eeq
Using Equation~\eqref{Eq:ModifiedBesselValues} in Equation~\eqref{Eq:GenHyperbolicDistributionAsStudent1}, the particular case of the probability density function becomes:
\beq
\begin{split}
\Gc\Hc(x|\lambda,\alpha \searrow 0,\beta = 0, \delta = \sqrt{\nu},\mu) 
&= 
\frac{1}{\sqrt{2\pi}}
\left(\frac{\alpha}{\sqrt{\nu}}\right)^{\frac{1}{2}}
\sqrt{2}
\left( \alpha \sqrt{\nu} \right)^{-\frac{1}{2}}
\;
\frac{\Gamma \left( \frac{1}{2} - \lambda \right) }{\Gamma \left( - \lambda \right)}
\;
\left( 1 + \frac{\left( x - \mu \right)^2}{\nu} \right)^{\lambda - \frac{1}{2}}
\end{split}
\label{Eq:GenHyperbolicDistributionAsStudent2}
\eeq
Finally, fixing $\lambda = -\frac{\nu}{2}$, Equation~\eqref{Eq:GenHyperbolicDistributionAsStudent2} becomes:
\beq
\begin{split}
\Gc\Hc(x|\lambda = \frac{-\nu}{2},\alpha \searrow 0,\beta = 0, \delta = \sqrt{\nu},\mu) 
&= 
\frac{1}{\sqrt{\nu\pi}}
\;
\frac{\Gamma \left( \frac{\nu+1}{2} \right) }{\Gamma \left( \frac{\nu}{2} \right)}
\;
\left( 1 + \frac{\left( x - \mu \right)^2}{\nu} \right)^{-\frac{\nu + 1}{2}}
=
\Sc t-t \left( x | \mu, \nu \right).
\end{split}
\label{Eq:GenHyperbolicDistributionAsStudent3}
\eeq
Figure~\eqref{fig:St_GenHypAsMStu} presents four Student-t probability density functions with different means ($\mu=0$, blue and red, $\mu=1$, yellow and $\mu=-1$, violet) and different degrees of freedom ($\nu=1$, blue and yellow, $\nu=1,5$, red and $\nu=0.5$, violet). 
Figure~\eqref{fig:GHSt_GenHypAsMStu} presents the Generalized Hyperbolic probability density function for parameters $\Gc\Hc (x | \lambda = -\nu/2, \alpha \searrow 0, \beta = 0, \delta = \sqrt{\nu}, \mu)$ with $\nu$ and $\mu$ set with the same numerical values as the corresponding ones from Figure~\eqref{fig:St_GenHypAsMStu}. For $\alpha$, the numerical values is $0.001$.
Figure~\eqref{fig:GHStVsSt_GenHypAsMStu} presents the comparison between the four Student-t probability density functions and the corresponding Generalized Hyperbolic probability density functions, $ \Sc t-t $ vs. $ \Gc\Hc $. In all forth cases the probability density functions are superposed. 
Figure~\eqref{fig:Log_GHStVsSt_GenHypAsMStu} presents the comparison between the logarithm of distributions, $ - \log \Sc t-t$ vs. $ - \log \Gc\Hc$.  
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering
                \includegraphics[width=7.4cm,height=4cm]{Fig_M_Stt}
                \caption{$ \Sc t-t \left( x | \mu , \nu \right) $}
                \label{fig:St_GenHypAsMStu}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_GenHyp_M_Stt}
                \caption{\small{$ \Gc\Hc \left( x | \lambda = -\frac{\nu}{2}, \alpha = 0.001, \beta = 0, \delta = \sqrt{\nu}, \mu=0 \right) $}}
                \label{fig:GHSt_GenHypAsMStu}
        \end{subfigure}        
\par\bigskip       
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_M_SttVsGenHyp_M_Stt}
                \caption{$ \Sc t-t $ vs. $ \Gc\Hc $}
                \label{fig:GHStVsSt_GenHypAsMStu}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LogM_SttVsGenHyp_M_Stt}
                \caption{$ - \log \Sc t-t $ vs. $ - \log \Gc\Hc $}
                \label{fig:Log_GHStVsSt_GenHypAsMStu}
        \end{subfigure}                                         
        \caption{Four Student-t probability density functions with different means ($\mu=0$, blue and red, $\mu=1$, yellow and $\mu=-1$, violet) and different degrees of freedom ($\nu=1$, blue and yellow, $\nu=1,5$, red and $\nu=0.5$, violet), Figure~\eqref{fig:St_GenHypAsMStu} and the corresponding Generalized Hyperbolic probability density functions, with parameters set as in Equation~\eqref{Eq:GenHyperbolicDistributionAsStudent3}, with $\alpha = 0.001$, Figure~\eqref{fig:GHSt_GenHypAsStu}. Comparison between the distributions, $\Sc t-t$ vs. $\Gc\Hc$, Figure~\eqref{fig:GHStVsSt_GenHypAsStu} and between the logarithm of the distributions $\log \Sc t-t$ vs. $\log \Gc\Hc$, Figure~\eqref{fig:Log_GHStVsSt_GenHypAsStu}.}
        \label{fig:Comp_GenHypAsMStu}
\end{figure}
Figure~\eqref{fig:GHStVsSt_GenHypAsStu} presents the comparison between the standard Student-t probability density function, $\Sc t-t \left( x | \mu=0, \nu=1 \right)$ (reported in Figure~\eqref{fig:St_GenHypAsStu}) and the Generalized Hyperbolic density function for parameters $\Gc\Hc (x | \lambda = -\frac{\nu}{2} = \frac{1}{2}, \alpha \searrow 0, \beta = 0, \delta = \sqrt{\nu} = 1, \mu=0)$ (reported in Figure~\eqref{fig:GHSt_GenHypAsStu}), showing that the two probability density functions are almost superposed. Figure~\eqref{fig:Log_GHStVsSt_GenHypAsStu} presents the comparison between the logarithm of the two distributions, $ - \log \Sc t-t$ vs. $ - \log \Gc\Hc$. In this case, the numerical value for $\alpha$ is $0.01$. 
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering
                \includegraphics[width=7.4cm,height=4cm]{Fig_Stt}
                \caption{$ \Sc t-t \left( x | \mu = 0 , \nu = 1 \right) $}
                \label{fig:St_GenHypAsStu}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_GenHyp_St}
                \caption{\small{$ \Gc\Hc \left( x | \lambda = -\frac{\nu}{2}, \alpha = 0.01, \beta = 0, \delta = \sqrt{\nu}, \mu=0 \right) $}}
                \label{fig:GHSt_GenHypAsStu}
        \end{subfigure}        
\par\bigskip       
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_SttVsGenHyp_St}
                \caption{$ \Sc t-t $ vs. $ \Gc\Hc $}
                \label{fig:GHStVsSt_GenHypAsStu}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LogSttVsGenHyp_St}
                \caption{$ -\log \Sc t-t $ vs. $ -\log \Gc\Hc $}
                \label{fig:Log_GHStVsSt_GenHypAsStu}
        \end{subfigure}                                         
        \caption{The standard Student-t distribution ($\nu=1$), Figure~\eqref{fig:St_GenHypAsStu} and the Generalized Hyperbolic distribution, with parameters set as in Equation~\eqref{Eq:GenHyperbolicDistributionAsStudent3}, Figure~\eqref{fig:GHSt_GenHypAsStu}. Comparison between the two distribution, $\Sc t-t$ vs. $\Gc\Hc$, Figure~\eqref{fig:GHStVsSt_GenHypAsStu} and between the logarithm of the distributions $-\log \Sc t-t$ vs. $-\log \Gc\Hc$, Figure~\eqref{fig:Log_GHStVsSt_GenHypAsStu}.}
        \label{fig:Comp_GenHypAsStu}
\end{figure}
The behaviour of the Generalized Hyperbolic density function $\Gc\Hc (x | \lambda = -\nu/2, \alpha \searrow 0, \beta = 0, \delta = \sqrt{\nu}, \mu=0)$ depending on $\alpha$ is presented in Figure~\eqref{fig:GHStVsSt_GenHypAsStu1}: a comparison between the standard Student-t probability density function $\Sc t-t \left( x | \mu=0, \nu=1 \right)$ (in blue) and the Generalized Hyperbolic density function $\Gc\Hc (x | \lambda = - \frac{\nu}{2} = -\frac{1}{2}, \alpha \searrow 0, \beta = 0, \delta = \sqrt{\nu} = 1, \mu=0)$ for $\alpha=1$ (in red), $\alpha=0.1$ (in yellow), $\alpha=0.01$ (in violet) and $\alpha=0.001$ (in green) is presented in Figure~\eqref{fig:GHStVsSt_GenHypAsStu1}. The difference between those four Generalized Hyperbolic density functions and the Student-t density function is presented in Figure~\eqref{fig:GHStMinusSt_GenHypAsStu1}. 
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_SttVsGenHyp_StMultiple}
                \caption{$ \Sc t-t $ vs. $ \Gc\Hc$ with $\alpha \in \left\lbrace 1, 0.1, 0.01, 0.001 \right\rbrace$}
                \label{fig:GHStVsSt_GenHypAsStu1}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_SttMinusGenHyp_StMultiple}
                \caption{$ \Gc\Hc - \Sc t-t $ for $\alpha \in \left\lbrace 1, 0.1, 0.01, 0.001 \right\rbrace$}
                \label{fig:GHStMinusSt_GenHypAsStu1}
        \end{subfigure}                                         
        \caption{The behaviour of the Generalized Hyperbolic density function $\Gc\Hc (x | \lambda = -\nu/2, \alpha \searrow 0, \beta = 0, \delta = \sqrt{\nu}, \mu=0)$ depending on $\alpha$.}
        \label{fig:Comp_GenHypAsStu1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Subsub: Generalized Hyperbolic as Hyperbolic %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Generalized Hyperbolic: Hyperbolic distribution}
\label{Subsubsec:GenHyperbolicAsHyp}
$X \sim \Gc\Hc(x|\lambda = 1,\alpha,\beta,\delta,\mu) $ has a Hyperbolic distribution, $\Hc \left( x | \alpha, \beta, \delta, \mu \right)$.\\
The goal of this section is to derive the Hyperbolic distribution from the Generalized Hyperbolic distribution. The interest is given by the fact that the Hyperbolic distribution is a \textit{heavy-tailed} distribution and therefore can be successfully used as a sparsity enforcing prior. The Hyperbolic distribution is a continuous probability distribution, for the logarithm of the probability density function is a hyperbola, therefore the distribution decreases exponentially, which is more slowly than the Normal distribution. It is suitable to model phenomena where numerically large values are more probable than is the case for the Normal distribution. The origin of the distribution is the observation by Ralph Alger Bagnold, that the logarithm of the histogram of the empirical size distribution of sand deposits tends to form a hyperbola. The Hyperbolic distribution has the following probability density function:
\beq
\Hc \left( x | \alpha, \beta, \delta, \mu \right)
=
\frac{\gamma}{2\alpha\delta \Kc_{1} \left( \delta \gamma \right)}
\exp \left\lbrace - \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2 } + \beta \left( x - \mu \right) \right\rbrace,
\gamma = \sqrt{ \alpha^2 - \beta^2 }
\label{Eq:HyperbolicDistribution}
\eeq
For the particular case of the Generalized Hyperbolic distribution with $\lambda = 1$, the probability density function is:
\beq
\Gc\Hc(x|\lambda = 1,\alpha,\beta,\delta,\mu) 
= 
\frac{1}{\sqrt{2\pi}}
\;
\frac{\gamma}{\delta}
\;
\left( \frac{\sqrt{ \delta^2 + \left( x - \mu \right)^2}}{ \alpha} \right)^{\frac{1}{2}}
\;
\frac{\Kc_{\frac{1}{2}} \left( \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} \right)}{\Kc_{1} \left( \delta \gamma \right)}
\;
\exp\left\lbrace\beta \left( x - \mu \right)\right\rbrace,
\label{Eq:GenHyperbolicDistributionAsHyp}
\eeq
For $\lambda=\frac{1}{2}$, the modified Bessel function of the second kind $\Kc_{\lambda} \left( x \right)$ can be stated explicitly with:
\beq
\Kc_{\frac{1}{2}} \left( x \right) = \Kc_{-\frac{1}{2}} \left( x \right) = \sqrt{\frac{\pi}{2x}} \exp \left\lbrace -x \right\rbrace, x > 0,
\label{Eq:ModifiedBesselExplicitly}
\eeq
so:
\beq
\Kc_{\frac{1}{2}} \left( \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} \right) 
=
\left(\frac{\pi}{2\alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2}}\right)^{\frac{1}{2}} 
\exp \left\lbrace -\alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} \right\rbrace. 
\label{Eq:GenHyperbolicDistributionAsHyp1}
\eeq
Plugging Equation~\eqref{Eq:GenHyperbolicDistributionAsHyp1} in Equation~\eqref{Eq:GenHyperbolicDistributionAsHyp}:
\beq
\Gc\Hc(x|\lambda = 1,\alpha,\beta,\delta,\mu) 
= 
\frac{\gamma}{2 \alpha \delta \Kc_{1} \left( \delta \gamma \right)}
\;
\exp \left\lbrace -\alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} + \beta \left( x - \mu \right) \right\rbrace
=
\Hc \left( x | \alpha, \beta, \delta, \mu \right).
\label{Eq:GenHyperbolicDistributionAsHyp2}
\eeq
Figure~\eqref{fig:Hyp_GenHypAsHyp} presents four Hyperbolic probability density functions $\Hc \left( x |\alpha,\beta,\delta,\mu \right)$ with different parameters.  
Figure~\eqref{fig:GHHyp_GenHypAsHyp} the corresponding Generalized Hyperbolic density functions for parameters $\Gc\Hc (x | \lambda = 1,\alpha,\beta,\delta,\mu)$.
The Hyperbolic probability density functions and the corresponding Generalized Hyperbolic density functions are superposed, Figure~\eqref{fig:GHHypVsHyp_GenHypAsHyp}.
Figure~\eqref{fig:Log_GHHypVsHyp_GenHypAsHyp} presents the comparison between the logarithm of the two distributions, $-\log \Hc$ vs. $-\log \Gc\Hc$.
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_Hyp.eps}
                \caption{$ \Hc \left( x | \alpha,\beta, \delta, \mu \right) $}
                \label{fig:Hyp_GenHypAsHyp}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_GenHyp_Hyp.eps}
                \caption{\small{$ \Gc\Hc \left( x | \lambda = 1, \alpha, \beta, \delta, \mu \right) $}}
                \label{fig:GHHyp_GenHypAsHyp}
        \end{subfigure}        
\par\bigskip        
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_HypVsGenHyp_Hyp.eps}
                \caption{$ \Hc $ vs. $ \Gc\Hc $}
                \label{fig:GHHypVsHyp_GenHypAsHyp}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LogHypVsGenHyp_Hyp.eps}
                \caption{$ -\log \Hc $ vs. $ -\log \Gc\Hc$}
                \label{fig:Log_GHHypVsHyp_GenHypAsHyp}
        \end{subfigure}                                       
        \caption{The Hyperbolic distribution, Figure~\eqref{fig:Hyp_GenHypAsHyp} and the Generalized Hyperbolic distribution, with parameters set as in Equation~\eqref{Eq:GenHyperbolicDistributionAsHyp2}, Figure~\eqref{fig:GHHyp_GenHypAsHyp}. Comparison between the two distribution, $\Hc$ vs. $\Gc\Hc$, Figure~\eqref{fig:GHHypVsHyp_GenHypAsHyp} and between the logarithm of the distributions $-\log \Hc$ vs. $-\log \Gc\Hc$, Figure~\eqref{fig:Log_GHHypVsHyp_GenHypAsHyp}.}
        \label{fig:Comp_GenHypAsHyp}
\end{figure}
The Hyperbolic distribution can be expressed using the Generalized Hyperbolic Prior Model (GHPM), Equation~\eqref{Eq:GHPM1} by fixing $\lambda =1$, . 
\beq
\textbf{HypPM:}\;\;\;\;\;\;\;
\left\{\barr{ll}
p(\rf_\rj | \mu, \; \rv_{\rf_\rj}, \; \beta)
=
\Nc\left(\rf_\rj|\mu + \beta \rv_{\rf_\rj}, \; \rv_{\rf_\rj}\right) 
=
\left( 2 \pi \right)^{-\frac{1}{2}} \; \rv_{\rf_\rj}^{-\frac{1}{2}} \; \exp \left\lbrace -\frac{1}{2}\frac{\left( x - \mu - \beta \rv_{\rf_\rj} \right)^2}{\rv_{\rf_\rj}} \right\rbrace
\\[7pt]
p(\rv_{\rf_\rj}|\gamma^2, \; \delta^2, \; \lambda) 
=
\Gc\Ic\Gc(\rv_{\rf_\rj}|\gamma^2, \; \delta^2, \; \lambda = 1)
=
\frac{\left(\frac{\gamma}{\delta}\right)}{2\Kc_{1} \left( \delta \gamma \right)}
\;
\exp \left\lbrace -\frac{1}{2} \left( \gamma^2 \rv_{\rf_\rj} + \delta^2 \rv_{\rf_\rj}^{-1} \right) \right\rbrace,\\[4pt]
\earr\right.
\label{Eq:GHPM_Hyp}
\eeq

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Subsub: Generalized Hyperbolic as Laplace %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Generalized Hyperbolic: Laplace distribution}
\label{Subsubsec:GenHyperbolicAsLap}
$X \sim \Gc\Hc(x|\lambda = 1, \alpha = b^{-1}, \beta = 0, \delta \searrow  0, \mu) $ has a Laplace distribution, $\Lc \left( x | \mu, b \right)$.\\
The goal of this section is to derive the Laplace distribution from the Generalized Hyperbolic distribution. The Laplace distribution has the following probability density function:
\beq
\Lc \left( x | \mu, b \right) = \frac{1}{2b} \exp \left\lbrace -\frac{\lvert x-\mu \rvert}{b} \right\rbrace
\eeq
Considering $\lambda=1$ in the expression of the Generalized Hyperbolic probability density function, a Hyperbolic distribution is obtained, Subsection~\eqref{Subsubsec:GenHyperbolicAsHyp}. Fixing $\beta=0$ implies $\gamma=\alpha$ and the expression of the probability density function becomes:
\beq
\begin{split}
\Gc\Hc(x|\lambda = 1, \alpha, \beta = 0, \delta ,\mu) 
= 
\Hc(x|\alpha, \beta = 0, \delta ,\mu) 
=
\frac{1}{2\delta\Kc_{1}\left( \delta \alpha \right)}
\exp 
\left\lbrace 
- \alpha \sqrt{\delta^2 + \left( x-\mu \right)^2} 
\right\rbrace
\end{split}
\label{Eq:GenHyperbolicDistributionAsLaplace}
\eeq
Further, considering $\delta \searrow  0$, for the expression of the modified Bessel function of the second degree $\Kc_{1}\left( \delta \alpha \right)$ the asymptotic relation for small arguments presented in Equation~\eqref{Eq:ModifiedBesselAsymptoticRelation} can be used, obtaining:
\beq
\Kc_{1}\left( \delta \alpha \right) = \alpha^{-1} \delta^{-1}, \mbox{ for } \delta \searrow  0.
\label{Eq:GenHyperbolicDistributionAsLaplace2}
\eeq
Using Equation~\eqref{Eq:GenHyperbolicDistributionAsLaplace2} in Equation~\eqref{Eq:GenHyperbolicDistributionAsLaplace}, the expression of the probability density function becomes:
\beq
\begin{split}
\Gc\Hc(x|\lambda = 1, \alpha, \beta = 0, \delta \searrow  0, \mu) 
= 
\Hc(x|\alpha, \beta = 0, \delta \searrow  0, \mu) 
=
\frac{1}{2\alpha^{-1}}
\exp 
\left\lbrace 
- \frac{\lvert x-\mu \rvert}{\alpha^{-1}}  
\right\rbrace.
\end{split}
\label{Eq:GenHyperbolicDistributionAsLaplace3}
\eeq
Finally, for $\alpha = b^{-1}$, the standard Laplace probability density function is obtained:
\beq
\begin{split}
\Gc\Hc(x|\lambda = 1, \alpha = b^{-1}, \beta = 0, \delta \searrow  0, \mu) 
= 
\Hc(x|\alpha = b^{-1}, \beta = 0, \delta \searrow  0, \mu) 
=
\frac{1}{2b}
\exp 
\left\lbrace 
- \frac{\lvert x-\mu \rvert}{b}  
\right\rbrace
=
\Lc \left( x | \mu, b \right)
\end{split}
\label{Eq:GenHyperbolicDistributionAsLaplace4}
\eeq
Figure~\eqref{fig:L_GenHypAsMLap} presents four Laplace probability density functions $\Lc \left( x | \mu, b \right)
$ with different means values ($\mu=0$, blue and red, $\mu=1$, yellow and $\mu=-1$, violet) and different scale parameter values ($b=1$, blue and violet, $b=2$, red and $b=0.5$, yellow).
Figure~\eqref{fig:GHL_GenHypAsMLap} presents the Generalized Hyperbolic probability density function for parameters $\Gc\Hc(x|\lambda = 1, \alpha = b^{-1}, \beta = 0, \delta \searrow  0, \mu)$ with $\mu$ and $b$ set with the same numerical values as the corresponding ones from Figure~\eqref{fig:L_GenHypAsMLap}. For $\delta$, the numerical values is $0.001$.
Figure~\eqref{fig:GHLVsL_GenHypAsMLap} presents the comparison between the four Laplace probability density functions and the corresponding Generalized Hyperbolic probability density functions, $ \Lc $ vs. $ \Gc\Hc $. In all forth cases the probability density functions are superposed. 
Figure~\eqref{fig:Log_GHLVsL_GenHypAsMLap} presents the comparison between the logarithm of distributions, $ - \log \Lc $ vs. $ - \log \Gc\Hc$.  
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering
                \includegraphics[width=7.4cm,height=4cm]{Fig_M_Lap}
                \caption{$ \Lc \left( x | \mu, b \right) $}
                \label{fig:L_GenHypAsMLap}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_GenHyp_M_Lap}
                \caption{\small{$ \Gc\Hc(x|\lambda = 1, \alpha = b^{-1}, \beta = 0, \delta \searrow  0, \mu) $}}
                \label{fig:GHL_GenHypAsMLap}
        \end{subfigure}        
\par\bigskip       
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_M_LapVsGenHyp_M_Lap}
                \caption{$ \Lc $ vs. $ \Gc\Hc $}
                \label{fig:GHLVsL_GenHypAsMLap}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LogM_LapVsGenHyp_M_Lap}
                \caption{$ - \log \Lc $ vs. $ - \log \Gc\Hc $}
                \label{fig:Log_GHLVsL_GenHypAsMLap}
        \end{subfigure}                                         
        \caption{Four Laplace probability density functions with different means values ($\mu=0$, blue and red, $\mu=1$, yellow and $\mu=-1$, violet) and different scale parameter values ($b=1$, blue and violet, $b=2$, red and $b=0.5$, yellow), Figure~\eqref{fig:L_GenHypAsMLap} and the corresponding Generalized Hyperbolic probability density functions, with parameters set as in Equation~\eqref{Eq:GenHyperbolicDistributionAsLaplace4}, with $\delta = 0.001$, Figure~\eqref{fig:GHL_GenHypAsMLap}. Comparison between the distributions, $ \Lc $ vs. $\Gc\Hc$, Figure~\eqref{fig:GHLVsL_GenHypAsMLap} and between the logarithm of the distributions $\log \Lc $ vs. $\log \Gc\Hc$, Figure~\eqref{fig:Log_GHLVsL_GenHypAsMLap}.}
        \label{fig:Comp_GenHypAsMLap}
\end{figure}
Figure~\eqref{fig:GHLVsL_GenHypAsL} presents the comparison between the standard Laplace probability density function, $\Lc \left( x | \mu = 0, b = 1 \right)$ (reported in Figure~\eqref{fig:L_GenHypAsL}) and the Generalized Hyperbolic density function for parameters $\Gc\Hc (x | \lambda = 1, \alpha = b^{-1} = 1, \beta = 0, \delta = 0.01, \mu = 0)$ (presented in Figure~\eqref{fig:GHL_GenHypAsL}), showing the two distributions superposed. Figure~\eqref{fig:Log_GHLVsL_GenHypAsL} presents the comparison between the logarithm of the two distributions, $- \log \Lc$ vs. $- \log \Gc\Hc$.
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_Lap.eps}
                \caption{$ \Lc \left( x | \mu = 0, b =1 \right)$}
                \label{fig:L_GenHypAsL}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_GenHyp_Lap.eps}
                \caption{\small{$ \Gc\Hc(x | \lambda = 1, \alpha = b^{-1} = 1, \beta = 0, \delta = 0.01, \mu = 0) $}}
                \label{fig:GHL_GenHypAsL}
        \end{subfigure}        
\par\bigskip        
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LapVsGenHyp_Lap.eps}
                \caption{$ \Lc $ vs. $ \Gc\Hc $}
                \label{fig:GHLVsL_GenHypAsL}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LogLapVsGenHyp_Lap.eps}
                \caption{$- \log \Lc $ vs. $- \log \Gc\Hc $}
                \label{fig:Log_GHLVsL_GenHypAsL}
        \end{subfigure}                                       
        \caption{The standard Laplace distribution, Figure~\eqref{fig:L_GenHypAsL} and the Generalized Hyperbolic distribution, with parameters set as in Equation~\eqref{Eq:GenHyperbolicDistributionAsLaplace4}, Figure~\eqref{fig:GHL_GenHypAsL}. Comparison between the two distribution, $ \Lc $ vs. $ \Gc\Hc $, Figure~\eqref{fig:GHLVsL_GenHypAsL} and between the logarithm of the distributions $- \log \Lc $ vs. $- \log \Gc\Hc $, Figure~\eqref{fig:Log_GHLVsL_GenHypAsL}.}
        \label{fig:Comp_GenHypAsL}
\end{figure}
The behaviour of the Generalized Hyperbolic density function $\Gc\Hc (x | \lambda = 1, \alpha = b^{-1} = 1, \beta = 0, \delta \searrow 0, \mu = 0)$ depending on $\delta$ is presented in Figure~\eqref{fig:GHLVsL_GenHypAsL1}: a comparison between the Laplace probability density function (in blue) and the Generalized Hyperbolic density function $\Gc\Hc (x | \lambda = 1, \alpha = b^{-1} = 1, \beta = 0, \delta \searrow 0, \mu = 0)$ for $\delta=1$ (in red), $\delta=0.1$ (in yellow), $\delta=0.01$ (in violet) and $\delta=0.001$ (in green) is presented in Figure~\eqref{fig:GHLVsL_GenHypAsL1}. The difference between those four Generalized Hyperbolic density functions and the Laplace density function is presented in Figure~\eqref{fig:GHLMinusL_GenHypAsL1}. 
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LapVsGenHyp_LMultiple}
                \caption{$ \Lc $ vs. $ \Gc\Hc$ for $\delta \in \left\lbrace 1, 0.1, 0.01, 0.001 \right\rbrace$}
                \label{fig:GHLVsL_GenHypAsL1}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LapMinusGenHyp_LMultiple}
                \caption{$ \Gc\Hc - \Lc $ for $\delta \in \left\lbrace 1, 0.1, 0.01, 0.001 \right\rbrace$}
                \label{fig:GHLMinusL_GenHypAsL1}
        \end{subfigure}                                         
        \caption{The behaviour of the Generalized Hyperbolic density function $\Gc\Hc (x | \lambda = 1, \alpha = b^{-1}, \beta = 0, \delta \searrow 0, \mu)$ depending on $\delta$.}
        \label{fig:Comp_GenHypAsL1}
\end{figure}
The Laplace distribution can be expressed using the Generalized Hyperbolic Prior Model (GHPM), Equation~\eqref{Eq:GHPM1} by fixing $ \lambda = 1, \alpha = b^{-1}, \beta = 0, \delta \searrow 0$: 
\beq
\textbf{LPM:}\;\;\;\;
\left\{\barr{ll}
p(\rf_\rj | \mu, \; \rv_{\rf_\rj}, \; \beta)
=
\Nc\left(\rf_\rj|\mu + \beta \rv_{\rf_\rj}, \; \rv_{\rf_\rj}\right) 
=
\left( 2 \pi \right)^{-\frac{1}{2}} \; \rv_{\rf_\rj}^{-\frac{1}{2}} \; \exp \left\lbrace -\frac{1}{2}\frac{\left( x - \mu - \beta \rv_{\rf_\rj} \right)^2}{\rv_{\rf_\rj}} \right\rbrace
\\[7pt]
p(\rv_{\rf_\rj}|\gamma^2, \; \delta^2 \searrow 0, \; \lambda = 1) 
=
\Gc\Ic\Gc(\rv_{\rf_\rj}|\gamma^2, \; \delta^2 \searrow 0, \; \lambda = 1)
=
\Ec(\rv_{\rf_\rj}|\frac{1}{2 b^2})
=
\frac{1}{2 b^2}
\;
\exp \left\lbrace -\frac{1}{2 b^2} \rv_{\rf_\rj} \right\rbrace,\\[4pt]
\earr\right.
\label{Eq:GHPM_Lap}
\eeq

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Subsub: Generalized Hyperbolic as V-G  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Generalized Hyperbolic: Variance-Gamma distribution}
\label{Subsubsec:GenHyperbolicAsVarGam}
$X \sim \Gc\Hc(x|\lambda,\alpha,\beta,\delta \searrow 0,\mu)$ has a variance-gamma distribution, $\Vc-\Gc(x|\alpha,\beta,\lambda,\mu)$.\\
The goal of this section is to derive the Variance-Gamma distribution from the Generalized Hyperbolic distribution. The Variance-Gamma distribution, a.k.a. generalized Laplace distribution or Bessel function distribution is a continuous probability distribution that is defined as the normal variance-mean mixture where the mixing density is the gamma distribution. The tails of the distribution decrease more slowly than the normal distribution. It is therefore suitable to model phenomena where numerically large values are more probable than is the case for the normal distribution. In particular, it can be successfully used for modelling sparse phenomena. Examples are returns from financial assets and turbulent wind speeds. The distribution was introduced in the financial literature by Madan and Seneta \textcolor{americanrose}{(\textit{D.B. Madan and E. Seneta (1990): The variance gamma (V.G.) model for share market returns, Journal of Business, 63, pp. 511–524.})}. The Variance-Gamma distributions form a subclass of the generalised hyperbolic distributions. The fact that there is a simple expression for the moment generating function implies that simple expressions for all moments are available. The Variance-Gamma distribution has the following probability density function:
\beq
\Vc-\Gc(x|\alpha,\beta,\lambda,\mu) 
= 
\frac{\gamma^{2\lambda} \lvert x - \mu \rvert^{\lambda-\frac{1}{2}}\Kc_{\lambda-\frac{1}{2}} \left( \alpha \lvert x - \mu \rvert \right)
}{\sqrt{\pi} \Gamma \left( \lambda \right) \left( 2 \alpha \right)^{\lambda-\frac{1}{2}}} 
\;
\exp \left\lbrace {\beta \left( x - \mu \right)} \right\rbrace
, 
\lambda > 0, \gamma = \sqrt{\alpha^2-\beta^2};
\label{Eq:VarianceGammaDistribution}
\eeq
Considering $\delta \searrow 0$, the particular form of the Generalized Hyperbolic distribution becomes:
\beq
\Gc\Hc(x|\lambda,\alpha,\beta,\delta \searrow 0,\mu) 
= 
\frac{{\gamma}^{\lambda}\lvert x - \mu \rvert^{\lambda - \frac{1}{2}}\Kc_{\lambda-\frac{1}{2}} \left( \alpha \lvert x - \mu \rvert \right)}{{\delta}^{\lambda} \sqrt{2\pi} {\alpha}^{\lambda - \frac{1}{2}} \Kc_{\lambda} \left( \delta \gamma \right)}
\;
\exp \left\lbrace {\beta \left( x - \mu \right)} \right\rbrace
\label{Eq:GenHyperbolicDistributionAsVarGam}
\eeq
Since $\delta \searrow  0$, for the expression of the modified Bessel function of the second degree $\Kc_{\lambda} \left( \delta \gamma \right)$ the asymptotic relation for small arguments presented in Equation~\eqref{Eq:ModifiedBesselAsymptoticRelation} can be used, obtaining:
\beq
\Kc_{\lambda} \left( \delta \gamma \right) = \Gamma \left( \lambda \right) 2^{\lambda-1} \left( \delta \gamma \right)^{-\lambda}, \mbox{ for } \delta \searrow  0.
\label{Eq:GenHyperbolicDistributionAsVarGam2}
\eeq
Using Equation~\eqref{Eq:GenHyperbolicDistributionAsVarGam2} in Equation~\eqref{Eq:GenHyperbolicDistributionAsVarGam}, the particular form of the Generalized Hyperbolic distribution becomes:
\beq
\Gc\Hc(x|\lambda,\alpha,\beta,\delta \searrow 0,\mu) 
= 
\frac{{\gamma}^{2\lambda}\lvert x - \mu \rvert^{\lambda - \frac{1}{2}}\Kc_{\lambda-\frac{1}{2}} \left( \alpha \lvert x - \mu \rvert \right)}{ \sqrt{\pi} \Gamma \left( \lambda \right) \left({2\alpha}\right)^{\lambda - \frac{1}{2}}}
\;
\exp \left\lbrace {\beta \left( x - \mu \right)} \right\rbrace
=
\Vc-\Gc(x|\alpha,\beta,\lambda,\mu)
\label{Eq:GenHyperbolicDistributionAsVarGam3}
\eeq
Figure~\eqref{fig:GHVGVsVG_GenHypAsVG} presents the comparison between the Variance-Gamma probability density function, $\Vc-\Gc(x|\alpha,\beta,\lambda,\mu)$ (presented in Figure~\eqref{fig:VG_GenHypAsVG}) and the Generalized Hyperbolic density function for parameters $\Gc\Hc(x|\lambda,\alpha,\beta,\delta \searrow 0,\mu)$ (presented in Figure~\eqref{fig:GHVG_GenHypAsVG}). Figure~\eqref{fig:Log_GHVGVsVG_GenHypAsVG} presents the comparison between the logarithm of the two distributions, $\log \Vc-\Gc$ vs. $\log \Gc\Hc$.
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_VG.eps}
                \caption{$ \Vc-\Gc(x|\alpha,\beta,\lambda,\mu) $}
                \label{fig:VG_GenHypAsVG}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_GenHyp_VG.eps}
                \caption{\small{$ \Gc\Hc(x|\lambda,\alpha,\beta,\delta \searrow 0,\mu) $}}
                \label{fig:GHVG_GenHypAsVG}
        \end{subfigure}        
\par\bigskip        
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_VGVsGenHyp_VG.eps}
                \caption{$ \Vc-\Gc $ vs. $ \Gc\Hc $}
                \label{fig:GHVGVsVG_GenHypAsVG}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LogVGVsGenHyp_VG.eps}
                \caption{$ \log \Vc-\Gc $ vs. $ \log \Gc\Hc$}
                \label{fig:Log_GHVGVsVG_GenHypAsVG}
        \end{subfigure}                                       
        \caption{The Variance-Gamma distribution, Figure~\eqref{fig:VG_GenHypAsVG} and the Generalized Hyperbolic distribution, with parameters set as in Equation~\eqref{Eq:GenHyperbolicDistributionAsVarGam3}, Figure~\eqref{fig:GHVG_GenHypAsVG}. Comparison between the two distribution, $\Vc-\Gc$ vs. $\Gc\Hc$, Figure~\eqref{fig:GHVGVsVG_GenHypAsVG} and between the logarithm of the distributions $\log \Vc-\Gc$ vs. $\log \Gc\Hc$, Figure~\eqref{fig:Log_GHVGVsVG_GenHypAsVG}.}
        \label{fig:Comp_GenHypAsVG}
\end{figure}
The Variance-Gamma distribution can be expressed using the Generalized Hyperbolic Prior Model (GHPM), Equation~\eqref{Eq:GHPM1} by fixing $\delta \searrow 0$: 
\beq
\textbf{V-GPM:}\;\;
\left\{\barr{ll}
p(\rf_\rj | \mu, \; \rv_{\rf_\rj}, \; \beta)
=
\Nc\left(\rf_\rj|\mu + \beta \rv_{\rf_\rj}, \; \rv_{\rf_\rj}\right) 
=
\left( 2 \pi \right)^{-\frac{1}{2}} \; \rv_{\rf_\rj}^{-\frac{1}{2}} \; \exp \left\lbrace -\frac{1}{2}\frac{\left( x - \mu - \beta \rv_{\rf_\rj} \right)^2}{\rv_{\rf_\rj}} \right\rbrace
\\[7pt]
p(\rv_{\rf_\rj}|\gamma^2, \; \delta^2 \searrow 0, \; \lambda = 1) 
=
\Gc\Ic\Gc(\rv_{\rf_\rj}|\gamma^2, \; \delta^2 \searrow 0, \; \lambda = 1)
=
\Ic\Gc(\rv_{\rf_\rj}|\lambda, \frac{\gamma^2}{2})
=
\frac{\left( \frac{\gamma^2}{2} \right)^{\lambda-1}}{\Gamma \left( \lambda \right)} \rv_{\rf_\rj}^{\lambda-1} \exp \left\lbrace -\frac{\gamma^2}{2} \rv_{\rf_\rj} \right\rbrace,\\[4pt]
\earr\right.
\label{Eq:GHPM_Lap}
\eeq

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   Subsub: Generalized Hyperbolic as NIG   %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Generalized Hyperbolic: Normal-Inverse Gaussian distribution}
\label{Subsubsec:GenHyperbolicAsNIG}
$X \sim \Gc\Hc(x|\lambda=-\frac{1}{2},\alpha,\beta,\delta,\mu)$ has a Normal-Inverse Gaussian distribution.\\
The goal of this section is to derive the Normal-Inverse Gaussian distribution from the Generalized Hyperbolic distribution. The interest is given by the fact that the Normal-Inverse Gaussian distribution can be a \textit{heavy-tailed} distribution and therefore can be successfully used as a sparsity enforcing prior. The Normal-Inverse Gaussian distribution is a continuous probability distribution, defined as the Normal variance-mean mixture, where the mixing density is the Inverse Gaussian distribution. The parameters of the Normal-Inverse Gaussian distribution can be used to construct a heaviness and skewness plot called the NIG-triangle. The Normal-Inverse Gaussian distribution has the following probability density function:
\beq
\Nc\Ic\Gc \left( x | \alpha, \beta, \delta, \mu \right)
= \frac{\alpha \delta \Kc_{1} \left( \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2 } \right)}{\pi \sqrt{ \delta^2 + \left( x - \mu \right)^2 }}
\exp \left\lbrace \gamma \delta + \beta \left( x - \mu \right) \right\rbrace
\label{Eq:NIGDistribution}
\eeq
Considering $\lambda = - \frac{1}{2}$, the Generalized Hyperbolic distribution is:
\beq
\Gc\Hc(x|\lambda,\alpha=-\frac{1}{2},\beta,\delta,\mu) 
= 
\frac{\left( \frac{\gamma}{\delta} \right)^{-\frac{1}{2}}}{\sqrt{2\pi}\Kc_{-\frac{1}{2}}\left( \gamma \delta \right)}
\frac{\Kc_{1} \left( \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} \right)}{\left( \frac{\sqrt{ \delta^2 + \left( x - \mu \right)^2}}{\alpha} \right)^{\frac{1}{2}-\lambda}}
\exp \left\lbrace \beta \left( x - \mu \right) \right\rbrace
\label{Eq:GenHyperbolicDistributionAsNIG}
\eeq
Using the fact that for $\lambda=\frac{1}{2}$, the modified Bessel function of the second kind $\Kc_{\lambda} \left( x \right)$ can be stated explicitly, Equation~\eqref{Eq:ModifiedBesselExplicitly}, we express  $\Kc_{-\frac{1}{2}} \left( \gamma \delta \right)$:
\beq
\Kc_{\frac{1}{2}} \left( \gamma \delta \right) 
=
\left(\frac{\pi}{2\gamma \delta}\right)^{\frac{1}{2}} 
\exp \left\lbrace -\gamma \delta \right\rbrace. 
\label{Eq:GenHyperbolicDistributionAsNIG2}
\eeq
Plugging Equation~\eqref{Eq:GenHyperbolicDistributionAsNIG2} in Equation~\eqref{Eq:GenHyperbolicDistributionAsNIG}:
\beq
\Gc\Hc(x|\lambda=-\frac{1}{2},\alpha,\beta,\delta,\mu) 
= 
\frac{\alpha \delta \Kc_{1} \left( \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} \right)}{\pi \sqrt{ \delta^2 + \left( x - \mu \right)^2}}
\exp \left\lbrace \gamma \delta + \beta \left( x - \mu \right) \right\rbrace
=
\Nc\Ic\Gc \left( x | \alpha, \beta, \delta, \mu \right)
\label{Eq:GenHyperbolicDistributionAsNIG3}
\eeq
Figure~\eqref{fig:GHNIGVsNIG_GenHypAsNIG} presents the comparison between the Normal-Inverse Gaussian probability density function, $\Nc\Ic\Gc(x|\alpha,\beta,\delta,\mu)$ (presented in Figure~\eqref{fig:NIG_GenHypAsNIG}) and the Generalized Hyperbolic density function for parameters $\Gc\Hc(x|\lambda=-\frac{1}{2},\alpha,\beta,\delta,\mu) $ (presented in Figure~\eqref{fig:GHNIG_GenHypAsNIG}). Figure~\eqref{fig:Log_GHNIGVsNIG_GenHypAsNIG} presents the comparison between the logarithm of the two distributions, $\log \Nc\Ic\Gc$ vs. $\log \Gc\Hc$.
\begin{figure}[!htb]
        \centering
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_NIG.eps}
                \caption{$ \Nc\Ic\Gc(x|\alpha,\beta,\delta,\mu) $}
                \label{fig:NIG_GenHypAsNIG}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_GenHyp_NIG.eps}
                \caption{\small{$ \Gc\Hc(x|\lambda=-\frac{1}{2},\alpha,\beta,\delta,\mu) $}}
                \label{fig:GHNIG_GenHypAsNIG}
        \end{subfigure}        
\par\bigskip        
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_NIGVsGenHyp_NIG.eps}
                \caption{$ \Nc\Ic\Gc $ vs. $ \Gc\Hc $}
                \label{fig:GHNIGVsNIG_GenHypAsNIG}
        \end{subfigure}                               
        \begin{subfigure}{0.49\textwidth}
          		\centering        
                \includegraphics[width=7.4cm,height=4cm]{Fig_LogNIGVsGenHyp_NIG.eps}
                \caption{$ \log \Nc\Ic\Gc $ vs. $ \log \Gc\Hc$}
                \label{fig:Log_GHNIGVsNIG_GenHypAsNIG}
        \end{subfigure}                                       
        \caption{The Normal-Inverse Gaussian distribution, Figure~\eqref{fig:NIG_GenHypAsNIG} and the Generalized Hyperbolic distribution, with parameters set as in Equation~\eqref{Eq:GenHyperbolicDistributionAsNIG3}, Figure~\eqref{fig:GHNIG_GenHypAsNIG}. Comparison between the two distribution, $\Nc\Ic\Gc$ vs. $\Gc\Hc$, Figure~\eqref{fig:GHNIGVsNIG_GenHypAsNIG} and between the logarithm of the distributions $\log \Nc\Ic\Gc$ vs. $\log \Gc\Hc$, Figure~\eqref{fig:Log_GHNIGVsNIG_GenHypAsNIG}.}
        \label{fig:Comp_GenHypAsNIG}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   Subsub: Generalized Hyperbolic as NIG   %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsubsection{Generalized Hyperbolic: Normal-Inverse-Gamma distribution}
\label{Subsubsec:GenHyperbolicAsNIGam}
$X \sim \Gc\Hc(x|?,?,?,?,?)$ has a Normal-Inverse-Gamma distribution.\\
The goal of this section is to derive the Normal-Inverse-Gamma distribution from the Generalized Hyperbolic distribution. In probability theory and statistics, the Normal-Inverse-Gamma distribution (or Gaussian-Inverse-Gamma distribution) is a four-parameter family of multivariate continuous probability distributions. It is the conjugate prior of a normal distribution with unknown mean and variance. The Normal-Inverse Gaussian distribution has the following probability density function:
\beq
\Nc\Ic\Gc am\left( x, v | \alpha, \beta, \delta, \mu \right)
= 
\frac{\sqrt{\lambda}}{\sqrt{2 \pi v}}
\;
\frac{\beta^{\alpha}}{\Gamma\left( \alpha \right)}
\;
\left(\frac{1}{v}\right)^{\alpha-1}
\;
\exp \left\lbrace \frac{ 2 \beta  + \lambda \left( x - \mu \right)^2 }{2 v} \right\rbrace
\label{Eq:NIGamDistribution}
\eeq
Considering $\lambda = - \frac{1}{2}$, the Generalized Hyperbolic distribution is:
\beq
\Gc\Hc(x|\lambda,\alpha,\beta,\delta,\mu) 
= 
\frac{\left(\frac{\gamma}{\delta}\right)^{\lambda}}{\sqrt{2\pi}\Kc_{\lambda} \left( \delta \gamma \right)}
\;
\frac{\Kc_{\lambda-\frac{1}{2}} \left( \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} \right)}{\left( \sqrt{ \delta^2 + \left( x - \mu \right)^2} / \alpha \right)^{\frac{1}{2}-\lambda}}
\;
\exp \left\lbrace {\beta \left( x - \mu \right)} \right\rbrace
, 
\lambda, \alpha, \beta, \delta, \mu \in \mathbb{R}, \gamma = \sqrt{\alpha^2-\beta^2};
\label{Eq:GenHyperbolicDistributionAsNIGam}
\eeq
Using the fact that for $\lambda=\frac{1}{2}$, the modified Bessel function of the second kind $\Kc_{\lambda} \left( x \right)$ can be stated explicitly, Equation~\eqref{Eq:ModifiedBesselExplicitly}, we express  $\Kc_{-\frac{1}{2}} \left( \gamma \delta \right)$:
\beq
\Kc_{\frac{1}{2}} \left( \gamma \delta \right) 
=
\left(\frac{\pi}{2\gamma \delta}\right)^{\frac{1}{2}} 
\exp \left\lbrace -\gamma \delta \right\rbrace. 
\label{Eq:GenHyperbolicDistributionAsNIGam2}
\eeq
Plugging Equation~\eqref{Eq:GenHyperbolicDistributionAsNIG2} in Equation~\eqref{Eq:GenHyperbolicDistributionAsNIG}:
\beq
\Gc\Hc(x|\lambda,\alpha=-\frac{1}{2},\beta,\delta,\mu) 
= 
\frac{\alpha \delta \Kc_{1} \left( \alpha \sqrt{ \delta^2 + \left( x - \mu \right)^2} \right)}{\pi \sqrt{ \delta^2 + \left( x - \mu \right)^2}}
\exp \left\lbrace \gamma \delta + \beta \left( x - \mu \right) \right\rbrace
=
\Nc\Ic\Gc \left( x | \alpha, \beta, \delta, \mu \right)
\label{Eq:GenHyperbolicDistributionAsNIG3}
\eeq
\fi


==> Subsec_Prior_SparsityEnforcingPriors.tex <==
\subsection{Some Sparsity enforcing priors}
\label{Subsec:SparsityEnforcingPriors}
A large number of sparsity enforcing priors are mentioned in the literature. Mainly, the sparsity enforcing priors can be classified in three categories, \textit{Generalized Gaussian distributions}, \textit{ Heavy-tailed distributions} and \textit{ Mixture Models distributions}, Figure~\eqref{Fig:MindMapSparsityEnforcingPriors}.
\iffalse
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{enumerate} [a)]
\item \textbf{ Generalized Gaussian}
\item \textbf{ Heavy-tailed distributions}
\item \textbf{ Mixture Models}
\end{enumerate}
\end{minipage}
\end{center}
\fi
\begin{figure}[!htb]
\center
\tikzset{level 1 concept/.append style={font=\sf, sibling angle=120,level distance = 5.2cm}}
\tikzset{level 2 concept/.append style={font=\sf, sibling angle=60,level distance = 2.6cm}}
%\tikzset{level 3 concept/.append style={font=\sf, sibling angle=39,level distance = 2cm}}
%\tikzset{level 4 concept/.append style={font=\sf, sibling angle=39,level distance = 1.3cm}}
%\tikzset{every node/.append style={scale=2}}
\begin{tikzpicture}[mindmap, grow cyclic, every node/.style=concept, concept color=purple!80, text=white]
\node{\textbf{Sparsity Prior: $p(\fb)$}}
   child [concept color=purple!80] { node {\textbf{Generalized Gaussian}}
        %child { node {\textbf{Gaussian}}}        
    }
   child [concept color=purple!80] { node {\textbf{Heavy-tailed}}
        %child { node {\textbf{Conjugate Priors}}}
    }
   child [concept color=purple!80] { node {\textbf{Mixture Models}}
        %child { node {\textbf{Gen. Gaussian}}}
        %child { node {\textbf{Symmetric Weibull}}}
        %child { node {\textbf{Student-t}}}
        %child { node {\textbf{Elastic Net}}}
        %child { node {\textbf{Gen. Hyperbolic}}}
        %child { node {\textbf{Dirichlet}}}                                
    };
\end{tikzpicture}
        \caption{Three main classes of sparsity enforcing priors: generalized Gaussian, heavy-tailed and mixture models}
\label{Fig:MindMapSparsityEnforcingPriors}
\end{figure}
Some prior distributions that can be considered are: \textbf{a)} Generalized Gaussian (GG) distribution with the particular case, the Laplace distribution; \textbf{b)} Weibull (W) distribution with Symmetric Rayleigh (SR) distribution as a particular case; \textbf{c)} Student-t (St) distribution with Cauchy (C) distribution as particular case; \textbf{d)} Elastic Net distribution, derived from regularization techniques; \textbf{e)} Generalized Hyperbolic model; \textbf{f)} Dirichlet and with Symmetric Dirichlet (SD) as particular case; \textbf{g)} Mixture of Gaussians, with \textbf{(i)} Mixture of two centred Gaussians (MoG2), one with very small and one with a large variance, with Bernoulli-Gauss (BG) (also called Spike and slab) as a particular case, \textbf{(ii)} Mixture of three Gaussians (MoG3), one centred with very small variance and two symmetrically centred on positive and negative axes and large variances; \textbf{(iii)} Mixture of one Gaussian and one or two Gammas (MoG-Gammas), and \textbf{h)} Bernoulli-Multinomial (BMult) or mixture of Dirichlet (MoD).
\iffalse
\begin{enumerate} [a)]
\item \textbf{ Generalized Gaussian (GG) distribution with the particular case, the Laplace distribution;}
\item \textbf{ Weibull (W) distribution with Symmetric Rayleigh (SR) distribution as a particular case;}
\item \textbf{ Student-t (St) distribution with Cauchy (C) distribution as particular case;}
\item \textbf{ Elastic Net distribution, derived from regularization techniques;}
\item \textbf{ Generalized Hyperbolic model;}
\item \textbf{ Dirichlet and with Symmetric Dirichlet (SD) as particular case;}
\item \textbf{ Mixture of Gaussians, with:}
\begin{enumerate} 
\item \textbf{ Mixture of two centred Gaussians (MoG2), one with very small and one with a large variance, with Bernoulli-Gauss (BG) (also called Spike and slab) as a particular case}
\item \textbf{ Mixture of three Gaussians (MoG3), one centred with very small variance and two symmetrically centred on positive and negative axes and large variances;}
\item \textbf{ Mixture of one Gaussian and one or two Gammas (MoG-Gammas)}
\end{enumerate}
\item \textbf{ Bernoulli-Multinomial (BMult) or mixture of Dirichlet (MoD)}
\end{enumerate}
\fi
Indeed, one class of distributions that can naturally impose sparsity is the the class of the heavy tailed distributions. This is due to the fact that when the linear forward model allows sparse solutions, the heavy tailed distributions will enforce such solutions by allowing important probabilities for high values. A comparison between a heavy-tailed distribution and the Normal distribution is presented in Figure~\eqref{Fig:HeavyTailedVsNormal}.
\begin{figure}[!htb]
    \centering
    \par\bigskip       
    \includegraphics[width=15cm,height=7cm]{Fig_NorVsSttVsLap.eps}
    \caption{One class of sparsity enforcing priors: \textbf{heavy-tailed distributions}. The standard \textcolor{cobalt}{Normal} distribution $\Nc\left( x | \mu=0, \mbox{var}=1 \right)$ vs. standard \textcolor{cinnabar}{Student-t} distribution $\Sc t-t\left( x | \mu=0, \nu=1 \right)$ and standard \textcolor{chromeyellow}{Laplace} distribution $\Lc\left( x | \mu=0, b=1 \right)$}
    \label{Fig:HeavyTailedVsNormal}
\end{figure}
Some heavy-tailed distributions that can be considered as sparsity enforcing prior are presented in the following subsections. 
\subsubsection{Generalized Gaussian $ \left( \Gc\Gc \right)$ distribution: particular case Laplace $ \left( \Lc \right)$  distribution}
\beq
\Gc\Gc(x|\mu, \alpha, \beta) = \frac{\beta}{2\alpha\Gamma\left(\frac{1}{\beta} \right)} \; \exp \left\lbrace {-\left(\frac{|x-\mu|}{\alpha}\right)}^{\beta}\right\rbrace, \; \alpha, \beta \in \mathbb{R_+}, \; \mu \in \mathbb{R} \; ;
\eeq
Particular cases for $\Gc\Gc$ distribution: The $\Gc\Gc$ family includes the \textbf{Laplace} distribution when $\beta$ = 1. As $\beta \rightarrow \infty$, the density converges pointwise to a uniform density on $\left( \mu -\alpha ,\mu +\alpha \right)$.
So, the $\Gc\Gc$ distribution allows for tails that are either \textbf{heavier} than Normal distribution tails (when $ \beta < 2 $) or \textbf{lighter} than normal (when $\beta >2$). Therefore, in the \textbf{sparsity} context, the $\Gc\Gc$ distribution with $ \beta < 2 $, is a possible choice for sparsity enforcing prior. As mentioned, the Laplace distribution is obtained for $\beta = 1$:
\begin{itemize}
\item \textbf{Laplace} distribution, for $\beta = 1$ and $\alpha = b$:
\beq
\Gc\Gc(x|\mu, \alpha = b, \beta = 1) = 
\Lc(x|\mu,b) = \frac{1}{2 b} \; \exp \left\lbrace {\frac{|x-\mu|}{b}}\right\rbrace, \; b \in \mathbb{R_+}, \; \mu \in \mathbb{R} \; ;
\eeq
\end{itemize} 
\subsubsection{Symmetric Weibull $ \left( \Sc\Wc \right)$ distribution (with the particular case Symmetric Rayleigh $ \left( \Sc\Rc \right)$ distribution)}
\beq
\Sc\Wc(x|k,b) = b \; k \; {|x|}^{k-1} \exp \left\lbrace -b \; {|x|}^{k}\right\rbrace, \; k, b \in \mathbb{R_+} \; ;
\eeq
Particular case for $\Sc\Wc$ distribution: The $\Sc\Wc$ family includes the \textbf{Symmetric Rayleigh} distribution when $k$ = 2 and $\beta = \frac{1}{2{\sigma}^2}$. As mentioned, the Symmetric Rayleigh distribution is obtained for $k$ = 2 and $\beta = \frac{1}{2{\sigma}^2}$:
\begin{itemize}
\item \textbf{Symmetric Rayleigh} distribution, for $k$ = 2 and $\beta = \frac{1}{2{\sigma}^2}$:
\beq
\Sc\Wc(x| k = 2, b = \frac{1}{2{\sigma}^2}) = 
\Sc\Wc(x| \sigma) = \frac{|x|}{{\sigma}^2} \; \exp \left\lbrace {\frac{{|x|}^2}{2{\sigma}^2}}\right\rbrace \; ;
\eeq
\end{itemize} 
\subsubsection{Student-t $ \left( \Sc t-t \right)$ distribution (with the particular case Cauchy $ \left( \Cc \right)$ distribution)}
\beq
\Sc t-t(x|\nu) = \frac{\Gamma\left(\frac{\nu+1}{2} \right)}{\sqrt{\pi\nu}\Gamma\left(\frac{\nu}{2} \right)} \left( 1 + \frac{x^2}{\nu} \right)^{\left(-\frac{\nu + 1}{2}\right)}, \; \nu \in \mathbb{R_+}, \; \Gamma \textrm{ representing the Gamma function};
\eeq
Particular case for $\Sc t-t$ distribution: The $\Sc t-t$ family includes the \textbf{Cauchy} distribution when $\nu$ = 1. As mentioned, the Cauchy distribution is obtained for $\nu$ = 1:
\begin{itemize}
\item \textbf{Cauchy} distribution, for $\nu$ = 1:
\beq
\Sc t-t(x| \nu = 1) = 
\Cc(x) = \frac{1}{\pi \left( 1 + x^2\right)} \; ;
\eeq
\end{itemize} 

\subsubsection{Elastic Net}
Oobtained via the product of a Normal distribution and a Laplace distribution. I think this distribution might be expressed via conjugate priors since the Laplace distribution can be expressed via a Normal distribution and an Inverse Gamma. TO BE DEVELOPED.
\subsubsection{Generalized Hyperbolic}
\subsubsection{Dirichlet}
\subsubsection{Mixture of Gaussians}

However, we are aiming for an algorithm that can produce \textit{analytical expressions} for the estimates of the model unknowns. One way to do this, i.e. to obtain analytical expressions for the unknowns of the model is to use conjugate priors for the expressions of the prior law. We will see that, doing this, during the iterations of the algorithm, the estimates are expressed as the parameters of one of the conjugate priors.
\\
One example, where this approach was proven to give good results is the case of the Student-t distribution, that can be expressed via conjugate priors, i.e. the Normal distribution and the Inverse Gamma distribution. More precisely, the Student-t distribution can be expressed as the marginal of a Normal distribution for which the variance is modelled as an Inverse Gamma distribution. 

\beq
\Sc t-t \left( x | \alpha, \beta \right) = \int \Nc \left( x | \mu, v_{x} \right)
\Ic \Gc \left( v_{x} | \alpha, \beta \right) \d v_x
\label{Eq:Student}
\eeq
\textcolor{mahogany}{\textbf{Goal:} The goal is to develop the corresponding algorithms for each sparsity enforcing law that can be expressed via conjugate priors and compare them. This comparison can be done on more levels:}
\begin{itemize}

\item \textcolor{mahogany}{Which prior gives the best results in terms of the accuracy of the estimation?}

\item \textcolor{mahogany}{Which prior is more adapted for which application? (in such Bayesian approaches the performances of a certain prior may depend on the particularities of applications.)}

\item \textcolor{mahogany}{Which prior is more/less sensible to initialization?}

\item \textcolor{mahogany}{Which prior results in an algorithm with the fastest convergence?}
\end{itemize}
\textcolor{mahogany}{\textbf{Further:} To complete the image, a similar discussion must be done for the estimation part. which estimators are to be used? What is the list of the \textit{available} estimators and which are the advantages and disadvantages of each?} 
\\
The class of heavy-tailed distributions is a good start for priors that enforce sparsity. However, we place this work in the context of such heavy tailed distributions that in particular can be expressed via \textit{conjugate priors}.

==> Subsec_St_nsStL_un_IS.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%					New SubSubSection			 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{IS: Student-t hierarchical model: non-stationary Student-t uncertainties model, unknown uncertainties variances}
\label{Subsec:St_nsStL_un_IS}
\begin{itemize}
\item the hierarchical model is using as a \textbf{prior} the \textbf{Student-t} distribution;
\item the Student-t prior distribution is expressed via \textbf{StPM}, Equation~\eqref{Eq:StPM1}, considering the variance $\rvb_\rf$ as unknown;
\item the \textbf{likelihood} is derived from the distribution proposed for modelling the uncertainties vector $\repsilonb$;
\item for the uncertainties vector $\repsilonb$ a \textbf{non-stationary Student-t uncertainties model} is proposed, i.e. a multivariate Student-t distribution expressed via \textbf{StPM} is used under the following assumption:\\
%\begin{itemize}
a) the variance vector $\rvb_{\repsilon}$ is \textbf{unknown}; 
%\end{itemize}
\end{itemize}
\beq
\rotatebox{90}{\hspace{-1.55cm}Student-t nsStL UNK} \;
\vline
\left.\barr{ll}
Likelihood: \textbf{nsStL:}\;
\left\{\barr{ll}
\begin{split}
p\left( \bgb | \rfb, \rvb_{\repsilon} \right) 
=
\Nc\left( \bgb | \bHb\rfb, \rVb_{\repsilon} \right) 
\propto 
\prod_{i=1}^{N} & \rv_{\repsilon_\ri}^{-\frac{1}{2}}
\exp \left\lbrace - \frac{1}{2}\| \rVb_{\repsilon}^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \| \right\rbrace, 
\end{split} 
\\[7pt]
p\left( \rvb_{\repsilon} | \alpha_{\epsilon}, \beta_{\epsilon} \right)
= \prod_{i=1}^{N} \Ic\Gc\left( \rv_{\repsilon_\ri} | \alpha_{\epsilon}, \beta_{\epsilon} \right) \propto  \prod_{i=1}^{N} \rv_{\repsilon_\ri}^{-\alpha_{\epsilon}-1} \; \exp \left\lbrace - \sum_{i=1}^{N}\frac{\beta_{\epsilon}}{\rv_{\repsilon_\ri}} \right\rbrace,
\\[7pt]
\hspace{5.55cm}
\rVb_{\repsilon} = \diag{\rvb_{\repsilon}},\; \rvb_{\repsilon} = \left[\ldots,\rv_{\repsilon_{\ri}}, \ldots\right],
\\[5pt]
\earr\right.
\\[37pt]
Likelihood: \textbf{nsStL:}\;
\left\{\barr{ll}
p(\rfb|\rzb,\rvb_{\rxi}) = \Nc(\rfb| \bDb\rzb, \; \rVb_{\rxi}) \propto \det{\rVb_{\rxi}}^{-\frac{1}{2}} \; \exp \left\lbrace - \frac{1}{2}\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \| \right\rbrace,
\\[6.7pt]
p(\rvb_{\rxi}|\alpha_{f}, \beta_{f}) = \prod_{j=1}^{M} \Ic\Gc(\rv_{\rxi_\rj}|\alpha_{\xi}, \beta_{\xi}) \propto  \prod_{j=1}^{M} \rv_{\rxi_\rj}^{-\alpha_{\xi}-1} \; \exp \left\lbrace - \sum_{j=1}^{M}\frac{\beta_{\xi}}{\rv_{\rxi_\rj}} \right\rbrace,
\\[7pt]
\hspace{5.65cm}
\rVb_{\rxi} = \diag{\rvb_{\rxi}},\; \rvb_{\rxi} = \left[\ldots,\rv_{\rxi_{\rj}}, \ldots\right],
\\[5pt]
\earr\right.
\\[37pt]
Prior:\;\;\;\;\;\;\;\textbf{StPM:}\;\;
\left\{\barr{ll}
p(\rzb|\zerob,\rvb_{\rz}) = \Nc(\rzb| \zerob, \; \rVb_{\rz}) \propto \det{\rVb_{\rz}}^{-\frac{1}{2}} \; \exp \left\lbrace - \frac{1}{2}\| \rVb_{\rz}^{-\frac{1}{2}} \rzb \| \right\rbrace,
\\[6.7pt]
p(\rvb_{\rz}|\alpha_{z}, \beta_{z}) = \prod_{j=1}^{M} \Ic\Gc(\rv_{\rz_\rj}|\alpha_{z}, \beta_{z}) \propto  \prod_{j=1}^{M} \rv_{\rz_\rj}^{-\alpha_{z}-1} \; \exp \left\lbrace - \sum_{j=1}^{M}\frac{\beta_{z}}{\rv_{\rz_\rj}} \right\rbrace,\\[7pt]
\hspace{5.65cm}
\rVb_{\rz} = \diag{\rvb_{\rz}},\; \rvb_{\rz} = \left[\ldots,\rv_{\rz_{\rj}}, \ldots\right].\\[4pt]
\earr\right.
\earr\right.
\label{Eq:St_nsStL_un_IS}
\eeq
The hierarchical model showed in Figure~\eqref{Fig:FromForwardModelHierarchicalModel2}, which is build over the linear forward model, Equation~\eqref{Eq:LinearModel} and Equation~\eqref{Eq:SparsityViaTransformation}, using as a prior for $\rzb$ a Student-t distribution, expressed via the Student-t Prior Model (StPM), Equation~\eqref{Eq:StPM1} and modelling the uncertainties of the model $\repsilonb$ and $\rxib$ using the non-stationary Student-t Uncertainties Model (nsStUM), Equation~\eqref{Eq:nsStUM}, is presented in Equation~\eqref{Eq:St_nsStL_un_IS}. The posterior distribution is obtained via the Bayes rule, Equation~\eqref{Eq:Post_St_nsStL_un_IS}:
\beq
\begin{split}
p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, & \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})
\propto  
p\left( \bgb | \rfb, \rvb_{\repsilon} \right) 
p\left( \rvb_{\repsilon} | \alpha_{\epsilon}  \beta_{\epsilon} \right) 
p(\rfb|\rzb,\rvb_{\rxi})
p(\rvb_{\rxi}|\alpha_{f}, \beta_{f})
p(\rzb|\zerob,\rvb_{\rz})
p(\rvb_{\rz}|\alpha_{z}, \beta_{z})
\\& 
\propto 
\;
\prod_{i=1}^{N} \rv_{\repsilon_\ri}^{-\frac{1}{2}}\exp \left\lbrace - \frac{1}{2}\| \rVb_{\repsilon}^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \| \right\rbrace 
\;
\prod_{i=1}^{N} \rv_{\repsilon_\ri}^{-\alpha_{\epsilon}-1} \; \exp \left\lbrace - \sum_{i=1}^{N}\frac{\beta_{\epsilon}}{\rv_{\repsilon_\ri}} \right\rbrace
\\&
\;\;\;\;\;
\det{\rVb_{\rxi}}^{-\frac{1}{2}} \; \exp \left\lbrace - \frac{1}{2}\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \| \right\rbrace
\;
\prod_{j=1}^{M} \rv_{\rxi_\rj}^{-\alpha_{\xi}-1} \; \exp \left\lbrace - \sum_{j=1}^{M}\frac{\beta_{\xi}}{\rv_{\rxi_\rj}} \right\rbrace
\\&
\;\;\;\;\;
\det{\rVb_{\rz}}^{-\frac{1}{2}} \; \exp \left\lbrace - \frac{1}{2}\| \rVb_{\rz}^{-\frac{1}{2}} \rzb \| \right\rbrace
\;
\prod_{j=1}^{M} \rv_{\rz_\rj}^{-\alpha_{z}-1} \; \exp \left\lbrace - \sum_{j=1}^{M}\frac{\beta_{z}}{\rv_{\rz_\rj}} \right\rbrace
\end{split}
\label{Eq:Post_St_nsStL_un_IS}
\eeq
The goal is to estimate the unknowns of the hierarchical model, namely $\rfb$, the main unknown of the linear forward model expressed in Equation~\eqref{Eq:LinearModel}, $\rzb$, the main unknown of Equation~\eqref{Eq:SparsityViaTransformation}, supposed sparse and consequently modelled using the Student-t distribution and the three variances appearing in the hierarchical model, Equation~\eqref{Eq:St_nsStL_un_IS}, the variance corresponding to the sparse structure $\rzb$, namely $\rvb_\rz$ and the two variances corresponding to the uncertainties of model $\repsilonb$, and $\rxib$, namely $\rvb_\repsilon$ and $\rvb_\rxi$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%					JMAP Estimation				 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Joint MAP estimation}
\label{Subsubsec:JMAP_St_nsStL_un_IS}
First, the Joint Maximum A Posterior (JMAP) estimation is considered: the unknowns are estimated on the basis of the available data $\bgb$, by maximizing the posterior distribution:
\beq
\begin{split}
\left( \rfbh, \; \rzbh, \; \rvbh_\rxi, \; \rvbh_\repsilon, \; \rvbh_\rz \right)
&=
\operatorname*{arg\,max}_{\left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)} p(\rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz | \bgb, \; \alpha_{\xi}, \; \beta_{\xi}, \; \alpha_{\epsilon}, \; \beta_{\epsilon}, \alpha_{z}, \; \beta_{z})
\\&
=
\operatorname*{arg\,min}_{\left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)} \Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right),
\end{split}
\eeq 
where for the second equality the criterion $\Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon \; \rvb_\rz \right)$ is defined as:
\beq
\Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right) = -\ln  p \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz | \bgb, \; \alpha_{\xi}, \; \beta_{\xi}, \; \alpha_{\epsilon}, \; \beta_{\epsilon}, \alpha_{z}, \; \beta_{z} \right)
\label{Eq:Def_L_Criterion_IS}
\eeq
The MAP estimation corresponds to the solution minimizing the criterion $\Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)$.
From the analytical expression of the posterior distribution, Equation~\eqref{Eq:Post_St_nsStL_un_IS} and the definition of the criterion $\Lc$,  Equation~\eqref{Eq:Def_L_Criterion_IS}, we obtain:
\beq
\begin{split}
\Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)
&
=
-\ln  p \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz | \bgb, \; \alpha_{\xi}, \; \beta_{\xi}, \; \alpha_{\epsilon}, \; \beta_{\epsilon}, \alpha_{z}, \; \beta_{z} \right)
\\&
+
\frac{1}{2}\| \rVb_{\repsilon}^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \|
+
\left( \alpha_{\epsilon} + \frac{3}{2} \right) \sum_{i=1}^{N} \ln \rv_{\repsilon_\ri} 
+
\sum_{i=1}^{N}\frac{\beta_{\epsilon}}{\rv_{\repsilon_\ri}} 
\\&
+
\frac{1}{2}\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
+
\left( \alpha_{\xi} + \frac{3}{2} \right) \sum_{i=1}^{N} \ln \rv_{\rxi_\ri} 
+
\sum_{i=1}^{N}\frac{\beta_{\xi}}{\rv_{\rxi_\ri}}
\\&
+
\frac{1}{2}\| \rVb_{\rz}^{-\frac{1}{2}} \rzb \|
+
\left(\alpha_{z} + \frac{3}{2} \right) \sum_{j=1}^{M} \ln \rv_{\rz_\rj}
+
\sum_{j=1}^{M}\frac{\beta_{f}}{\rv_{\rz_\rj}}
\end{split}
\label{Eq:L_Criterion_IS}
\eeq
One of the simplest optimisation algorithm that can be used is an alternate optimization of the criterion $\Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)
$ with respect to the each unknown:
\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%						New Item			 	 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item With respect to $\rfb$:
\beq
\begin{split}
\frac{\partial \Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)}{\partial \rfb}=0
&\Leftrightarrow
\frac{\partial}{\partial \rfb}
\left(
\| \rVb_\repsilon^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \|
+
\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
\right) = 0
\\
&\Leftrightarrow
-\bHb^T \rVb_\repsilon^{-1} \left( \bgb - \bHb \rfb \right) 
+ 
\rVb_\rxi^{-1} \left( \rfb - \bDb\rzb \right) 
= 0
\\
&
\Leftrightarrow 
\left( \bHb^T \rVb_\repsilon^{-1} \bHb + \rVb_\rxi^{-1} \right) \rfb  = 
\bHb^T \rVb_\repsilon^{-1} \bgb + \rVb_\rxi^{-1} \bDb\rzb
\\
&
\Rightarrow
\rfbh 
=
\left( \bHb^T \rVb_\repsilon^{-1} \bHb + \rVb_\rxi^{-1} \right)^{-1} 
\left( \bHb^T \rVb_\repsilon^{-1} \bgb + \rVb_\rxi^{-1} \bDb\rzb \right)
\end{split}
\nonumber
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%						New Item			 	 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item With respect to $\rzb$:
\beq
\begin{split}
\frac{\partial \Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)}{\partial \rzb}=0
&\Leftrightarrow
\frac{\partial}{\partial \rfb}
\left(
\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
+
\| \rVb_{\rz}^{-\frac{1}{2}} \rzb \|
\right)= 0
\\
&\Leftrightarrow
-\bDb^T \rVb_\rxi^{-1} \left( \rfb - \bDb\rzb \right) 
+ 
\rVb_\rz^{-1} \rzb  
= 0
\\
&
\Leftrightarrow 
\left( \bDb^T \rVb_\rxi^{-1} \bDb + \rVb_\rz^{-1} \right) \rzb  = 
\bDb^T \rVb_\rxi^{-1} \rfb
\\
&
\Rightarrow
\rzbh 
=
\left( \bDb^T \rVb_\rxi^{-1} \bDb + \rVb_\rz^{-1} \right)^{-1} \bDb^T \rVb_\rxi^{-1} \rfb
\end{split}
\nonumber
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%						New Item			 	 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item With respect to $\rv_{\repsilon_\ri}$, $i \in \left\lbrace 1,2,\ldots, N \right\rbrace$:\\
First, we develop the norm $\| \rVb_\repsilon^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \|$:
\beq
\begin{split}
\| \rVb_\repsilon^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \|
&= 
\bgb^{T} \rVb_\repsilon^{-1} \bgb
-
2 \bgb^{T} \rVb_\repsilon^{-1} \bHb \rfb
+
\bHb^{T} \rfb^{T} \rVb_\repsilon^{-1} \bHb \rfb
\\
&=
\sum_{i=1}^{N} \rv_{\repsilon_\ri}^{-1} \bg_\bi^{2}
-
2 \sum_{i=1}^{N} \rv_{\repsilon_\ri}^{-1} \bg_\bi \bH_\bi \rfb 
+
\sum_{i=1}^{N} \rv_{\repsilon_\ri}^{-1} \rfb^{T} \bH_\bi^{T} \bH_\bi \rfb,
\nonumber
\end{split}
\eeq
where $\bHb_\bi$ denotes the line i of the matrix $\bHb$, $i\in \left\lbrace 1,2,\ldots,N \right\rbrace$, i.e. $\bHb_\bi = \left[ \bh_{\bi\blue{1}}, \bh_{\bi\blue{1}}, \ldots, \bh_{\bi\bM} \right]$. 
\beq
\begin{split}
\frac{\partial \Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)}{\partial \rv_{\repsilon_\ri}}=0
&
\Leftrightarrow
\frac{\partial}{\partial \rv_{\repsilon_\ri}}
\left[
\left( \alpha_{\epsilon} + \frac{3}{2} \right)\ln \rv_{\repsilon_\ri}
+
\left(\beta_{\epsilon} + \frac{1}{2} \left( \bg_\bi^{2} - 2 \bg_\bi \bHb_\bi \rfb  + \rfb^{T} \bHb_\bi^{T} \bHb_\bi \rfb \right)
\right) \rv_{\repsilon_\ri}^{-1}
\right]
=0
\\
&
\Leftrightarrow
\left( \alpha_{\epsilon} + \frac{3}{2} \right) \rv_{\repsilon_\ri}
-
\left(\beta_{\epsilon} + \frac{1}{2} \left( \bg_\bi - \bHb_\bi \rfb  \right)^2 \right)=0
\\
&
\Rightarrow
\rvh_{\repsilon_\ri} = \frac{\beta_{\epsilon} + \frac{1}{2} \left( \bg_\bi - \bHb_\bi \rfb \right)^2}{\alpha_{\epsilon} + \frac{3}{2}}
\end{split}
\nonumber
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%						New Item			 	 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item With respect to $\rv_{\rxi_\rj}$, $j \in \left\lbrace 1,2,\ldots, M \right\rbrace$:\\
First, we develop the norm $\| \rVb_\rxi^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|$:
\beq
\begin{split}
\| \rVb_\rxi^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
&= 
\rfb^{T} \rVb_\rxi^{-1} \rfb
-
2 \rfb^{T} \rVb_\rxi^{-1} \bDb \rzb
+
\bDb^{T} \rzb^{T} \rVb_\rxi^{-1} \bDb \rzb
\\
&=
\sum_{j=1}^{M} \rv_{\rxi_\rj}^{-1} \rf_\rj^{2}
-
2 \sum_{j=1}^{M} \rv_{\rxi_\rj}^{-1} \rf_\rj \bD_\bj \rzb 
+
\sum_{j=1}^{M} \rv_{\rxi_\rj}^{-1} \rzb^{T} \bD_\bj^{T} \bD_\bj \rzb,
\nonumber
\end{split}
\eeq
where $\bDb_\bj$ denotes the line j of the matrix $\bDb$, $j\in \left\lbrace 1, 2, \ldots, M \right\rbrace$, i.e. $\bDb_\bj = \left[ \bd_{\bj\blue{1}}, \bd_{\bj\blue{1}}, \ldots, \bd_{\bj\bM} \right]$. 
\beq
\begin{split}
\frac{\partial \Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)}{\partial \rv_{\rxi_\rj}}=0
&
\Leftrightarrow
\frac{\partial}{\partial \rv_{\rxi_\rj}}
\left[
\left( \alpha_{\xi} + \frac{3}{2} \right)\ln \rv_{\rxi_\rj}
+
\left(\beta_{\xi} + \frac{1}{2} \left( \rf_\rj^{2} - 2 \rf_\rj \bDb_\bj \rzb  + \rzb^{T} \bDb_\bj^{T} \bHb_\bj \rzb \right)
\right) \rv_{\rxi_\rj}^{-1}
\right]
=0
\\
&
\Leftrightarrow
\left( \alpha_{\xi} + \frac{3}{2} \right) \rv_{\rxi_\rj}
-
\left(\beta_{\xi} + \frac{1}{2} \left( \rf_\rj - \bDb_\bi \rzb  \right)^2 \right)=0
\\
&
\Rightarrow
\rvh_{\rxi_\rj} = \frac{\beta_{\xi} + \frac{1}{2} \left( \rf_\rj - \bDb_\bj \rzb \right)^2}{\alpha_{\xi} + \frac{3}{2}}
\end{split}
\nonumber
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%						New Item			 	 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item With respect to $\rv_\rz_\rj$, $j \in \left\lbrace 1,2,\ldots, M \right\rbrace$:
\beq
\begin{split}
\frac{\partial \Lc \left( \rfb, \; \rzb, \; \rvb_\rxi, \; \rvb_\repsilon, \; \rvb_\rz \right)}{\partial \rv_{\rz_\rj}}=0
&
\Leftrightarrow
\frac{\partial}{\partial \rv_{\rz_\rj}}
\left[
\left( \alpha_z + \frac{3}{2}  \right)\ln \rv_{\rz_\rj}
+
\left( \beta_z + \frac{1}{2} \rz_\rj^2 \right)
\rv_{\rz_\rj}^{-1}
\right]
=0
\\
&
\Leftrightarrow
\left( \alpha_z + \frac{3}{2}  \right) \rv_{\rz_\rj}
-
\left( \beta_z + \frac{1}{2} \rz_\rj^2 \right)
=0
\\
&
\Rightarrow
\rvh_{\rz_\rj} = \frac{\beta_z + \frac{1}{2} \rz_\rj^2}{\alpha_z + \frac{3}{2}}
\end{split}
\nonumber
\eeq
\end{itemize}
The iterative algorithm obtained via JMAP estimation is presented Figure~\eqref{Fig:IA_JMAP_St_nsStL_un_IS}.
\tikzstyle{cloud} = [draw=blue!30!green,fill=orange!12, ellipse, thick, node distance=6em, text width=12em, text centered, minimum height=4em, minimum width=12em]
\tikzstyle{boxbig} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=6.5em, text width=25em, text centered, minimum height=5em, minimum width=25em]
\tikzstyle{boxhuge} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=4.5em, text width=34em, text centered, minimum height=5em, minimum width=34em]
\tikzstyle{box} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=7.5em, text width=21em, text centered, minimum height=5em, minimum width=21em]
\tikzstyle{boxsmall} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=9em, text width=9em, text centered, minimum height=4em, minimum width=9em]
%\tikzstyle{fancytitle} =[fill=green!24, text=white, ellipse]
%\tikzstyle{container} = [draw, rectangle, dashed, inner sep=2em]
\tikzstyle{line} = [draw=blue!30!green, -latex']
%\begin{figure}[htbp]
\begin{figure}[!htb]
\centering
\begin{center}
\begin{tikzpicture}[auto]
    \node [boxhuge, scale=0.9] (f) {\Large{$\rfbh = \left( \bHb^T \rVb_\repsilon^{-1} \bHb + \rVb_\rxi^{-1} \right)^{-1} \left( \bHb^T \rVb_\repsilon^{-1} \bgb + \rVb_\rxi^{-1} \bDb\rzb \right)$}
\\[8pt]
\normalsize{(a) - update estimated $\rfb$} 
};

	\node [boxbig, below of=f, node distance=9.6em, scale=0.9] (z) {\Large{$\rzbh =\left( \bDb^T \rVb_\rxi^{-1} \bDb + \rVb_\rz^{-1} \right)^{-1} \bDb^T \rVb_\rxi^{-1} \rfb$}
\\[5pt]
\normalsize{(a) - update estimated $\rfb$} 
};

    \node [box, below of=z, node distance=9.6em, scale=0.9] (vxi)
{\Large{$ \rvh_{\rxi_\rj} = \frac{\beta_{\xi} + \frac{1}{2} \left( \rf_\rj - \bDb_\bj \rzb \right)^2}{\alpha_{\xi} + \frac{3}{2}} $}
\\[5pt]
\normalsize{(b) - update estimated variances $\rv_{\rf_\rj}$} 
};

    \node [box, below of=vxi, node distance=9.6em, scale=0.9] (veps) {\Large{$\rvh_{\repsilon_\ri} = \frac{\beta_{\epsilon} + \frac{1}{2} \left( \bg_\bi - \bHb_\bi \rfbh \right)^2}{\alpha_{\epsilon} + \frac{3}{2}}$}
\\[5pt]
\normalsize{(c) - update estimated uncertainties variances $\rv_{\repsilon_\ri}$}     
};

    \node [box, below of=veps, node distance=9.6em, scale=0.9] (vz) {\Large{$\rvh_{\rz_\rj} = \frac{\beta_z + \frac{1}{2} \rz_\rj^2}{\alpha_z + \frac{3}{2}}$}
\\[5pt]
\normalsize{(c) - update estimated uncertainties variances $\rv_{\repsilon_\ri}$}     
};


    \node [boxsmall, above right = 0.1cm and 0.7cm of vxi, node distance=17em, scale=0.9] (Vxi) {\Large{$\rVbh_\rxi = \diag {\rvbh_{\rxi}}$}
\\[5pt]
\normalsize{(d)}
};

    \node [boxsmall, below left = -3.4cm and 0.7cm of veps, node distance=17em, scale=0.9] (Veps) {\Large{$\rVbh_\repsilon = \diag {\rvbh_{\repsilon}}$}
\\[5pt]
\normalsize{(e)} 
};

    \node [boxsmall, above right = 0.1cm and 2.4cm of vz, node distance=17em, scale=0.9] (Vz) {\Large{$\rVbh_\rz = \diag {\rvbh_{\rz}}$}
\\[5pt]
\normalsize{(e)} 
};


\node [cloud, above of=f, scale=0.9] (init)
{\Large{Initialization}};  

    \path [line] (f) -- (z)[near start];
    \path [line] (z) -- (vxi);
    \path [line] (vxi) -- (veps);
    \path [line] (veps) -- (vz);    
    \path [line] (Vxi) |- (f);
    \path [line] (Vxi) |- (z);
    \path [line] (Veps) |- (f);
    \path [line] (Vz) |- (z);    
    \path [line] (vxi) -| (Vxi);
    \path [line] (veps) -| (Veps);
    \path [line] (vz) -| (Vz);
    \path [line] (z) -| (f);
    \path [line] (init) -- (f);   
\end{tikzpicture}
\end{center}
\caption{Indirect sparsity (via $\rzb$) - Iterative algorithm corresponding to Joint MAP estimation for Student-t hierarchical model, non-stationary Student-t uncertainties model}
\label{Fig:IA_JMAP_St_nsStL_un_IS}
\end{figure}

\begin{algorithm}
\caption{Joint MAP - Student-t hierarchical model, non-stationary Student-t uncertainties model}
\begin{algorithmic}[1]
\Ensure INITIALIZATION $\rfbh^{(0)}$ \Comment{Where $\rfbh^{(0)} = \rfbh$ via a basic estimation method or $\rfbh^{(0)} = \zerob$}
\Function{JMAP}{$\alpha_{\epsilon},\beta_{\epsilon},\alpha_{f},\beta_{f},\bgb,\bHb,\rfb^{(0)},M,N,NoIter$} \Comment{$\alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{f}, \beta_{f}$ are set in modeling phase, Eq.~\eqref{Eq:St_nsStL_un_IS}}

\For{$n = 0$ to ${IterNumb}$}

\For{$j = 1$ to ${M}$}

\State $\rvh_{\rf_\rj}^{(n)} = \frac{\beta_f + \frac{1}{2} (\rfh_\rj^{(n)})^2}{\alpha_f + \frac{3}{2}}$ \Comment{$\rvh_{\rf_\rj}^{(n)}$ is computed using $\alpha_{f},\beta_{f},\rfb^{(n)}$}

\EndFor

\State $\rVbh_\rf^{(n)} = \diag {\rvbh_{\rf}^{(n)}}$ \Comment{The diagonal matrix $\rVbh_\rf^{(n)}$ is build using $\rvh_{\rf_\rj}^{(n)}$, $j \in \left\lbrace 1,2,\ldots, M\right\rbrace$}

\For{$i = 1$ to ${N}$}

\State $\rvh_{\repsilon_\ri}^{(n)} = \frac{\beta_{\epsilon} + \frac{1}{2} \left( \bg_\bi - \bHb_\bi \rfbh^{(n)} \right)^2}{\alpha_{\epsilon} + \frac{3}{2}}$ \Comment{$\rvh_{\repsilon_\ri}^{(n)}$ is computed using $\alpha_{\epsilon},\beta_{\epsilon}, \bg_\bi, \bHb_\bi, \rfb^{(n)}$} 

\EndFor

\State $\rVbh_\repsilon^{(n)} = \diag {\rvbh_{\repsilon}^{(n)}}$ \Comment{The diagonal matrix $\rVbh_\repsilon^{(n)}$ is build using $\rvh_{\repsilon_\ri}^{(n)}$, $i \in \left\lbrace 1,2,\ldots, N \right\rbrace$}

\State $\rfbh^{(n+1)}  = \left( \bHb^T \left(\rVbh_\repsilon^{(n)}\right)^{-1} \bHb + \left( \rVbh_\rf^{(n)}\right)^{-1} \right)^{-1} \bHb^T \left(\rVbh_\repsilon^{(n)}\right)^{-1} \bgb$ \Comment{New value $\rfbh^{(n+1)}$}

\EndFor

\Return $\left( \rfbh^{(n+1)}, \rvbh_\rf^{(n)}, \rvbh_{\repsilon}^{(n)} \right)$ , $n = NoIter$
\EndFunction
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%		PM Estimation partial separability		 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Posterior Mean estimation via VBA, partial separability}
\label{Subsubsec:PM_PS_St_nsStL_un_IS}
In this subsection, the Posterior Mean (PM) estimation is considered. The Joint MAP computes the mod of the posterior distribution. The PM computes the mean of the posterior distribution. One of the advantages of this estimator is that it minimizes the Mean Square Error (MSE). Computing the posterior means of any unknown needs great dimensional integration. For example, the mean corresponding to $\rfb$ can be computed from the posterior distribution using Equation~\eqref{Eq:PM_Computation_F_IS},
\beq
E_p \left\lbrace \rfb \right\rbrace = \iiint \rfb \; p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \d\rfb  \d\rzb \d\rvb_{\rxi} \d\rvb_{\repsilon} \d\rvb_{\rz}.
\label{Eq:PM_Computation_F_IS}
\eeq
In general, these computations are not easy. One way to obtain approximate estimates is to approximate $p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})$ by a separable one $q(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) = q_1(\rfb) q_2(\rzb)  q_3(\rvb_{\rxi}) q_4(\rvb_{\repsilon}) q_5(\rvb_{\rz}) $, then computing the posterior means using the separability. The mean corresponding to $\rfb$ is computed using the corresponding separable distribution $q_1(\rfb)$, Equation~\eqref{Eq:PM_Computation_F_Separable}, 
\beq
E_{q_{1}} \left\lbrace \rfb \right\rbrace = \int \rfb \; q_1(\rfb) \d\rfb.
\label{Eq:PM_Computation_F_Separable_IS}
\eeq
If the approximation of the posterior distribution with a separable one can be done in such a way that conserves the mean, i.e. Equation~\eqref{Eq:PM_Conservation_IS},
\beq
E_q \left\lbrace x \right\rbrace = E_p \left\lbrace x \right\rbrace, 
\label{Eq:PM_Conservation_IS}
\eeq
for all the unknowns of the model, a great amount of computational cost is gained. In particular, for the proposed hierarchical model, Equation~\eqref{Eq:St_nsStL_un_IS}, the posterior distribution, Equation~\eqref{Eq:Post_St_nsStL_un_IS}, is not a separable one, making the analytical computations of the PM very difficult. One way the compute the PM in this case is to first approximate the posterior law $p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})$ with a separable law $q(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})$, Equation~\eqref{Eq:Posterior_Approximation_IS},
\beq
\begin{split}
p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})
&\approx 
q(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})
\\&
=
q_1(\rfb) \; q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon}) \; q_5(\rvb_{\rz})\label{Eq:Posterior_Approximation_IS}
\end{split}
\eeq
where the notations from Equation~\eqref{Eq:Posterior_Approximation_Notations1_IS} are used
\beq
q_{3}(\rvb_{\rxi}) = \prod_{j=1}^{M} q_{2j}(\rv_{\rxi_\rj}),
\;\;;\;\;
q_{4}(\rvb_{\repsilon}) = \prod_{i=1}^{N} q_{3i}(\rv_{\repsilon_\ri})
\;\;;\;\;
q_{5}(\rvb_{\rz}) = \prod_{j=1}^{M} q_{3i}(\rv_{\rz_\rj}) 
\label{Eq:Posterior_Approximation_Notations1_IS}
\eeq
by minimizing of the Kullback-Leibler divergence, defined as:
\small
\beq
\begin{split}
\mbox{KL} & \left( q(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})
 : p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \right) =
\\
&=\iint \ldots \int q(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \; \ln\frac{q(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})} {p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})} \d\rfb  \d\rzb \d\rvb_{\rxi} \d\rvb_{\repsilon} \d\rvb_{\rz},
\label{Eq:Kullback-Leibler_IS}
\end{split}
\eeq
\normalsize
where the notations from Equation~\eqref{Eq:Posterior_Approximation_Notations2_IS} are used
\beq
\d \rvb_{\rxi} = \prod_{j=1}^{M} \d \rv_{\rxi_\rj}
\;\;;\;\;
\d \rvb_{\repsilon} = \prod_{i=1}^{N} \d \rv_{\repsilon_\ri}
\;\;;\;\;
\d \rvb_{\rz} = \prod_{j=1}^{M} \d \rv_{\rz_\rj}.
\label{Eq:Posterior_Approximation_Notations2_IS}
\eeq
Equation~\eqref{Eq:Posterior_Approximation_Notations1_IS} is selecting a partial separability for the approximated posterior distribution $q(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})$ in the sense that a total separability is imposed for the distributions corresponding to the three variances appearing in the hierarchical model, $q_3\left( \rvb_{\rxi} \right)$, $q_4\left( \rvb_{\repsilon} \right)$ and $q_5\left( \rvb_{\rz} \right)$ but not for the distribution corresponding to $\rfb$ and $\rzb$. Evidently, a full separability can be imposed, by adding the supplementary conditions $q_{1}(\rfb) = \prod_{j=1}^{M} q_{1j}(\rf_\rj)$ and $q_{3}(\rzb) = \prod_{j=1}^{M} q_{2j}(\rz_\rj)$ in Equation~\eqref{Eq:Posterior_Approximation_Notations1_IS}. This case is considered in Subsection~\eqref{Subsubsec:PM_FS_St_nsStL_un_IS}. The minimization can be done via alternate optimization resulting the following proportionalities from Equations~\eqref{Eq:VBA_Proportionalities1_IS},~\eqref{Eq:VBA_Proportionalities2_IS},~\eqref{Eq:VBA_Proportionalities3_IS},~\eqref{Eq:VBA_Proportionalities4_IS} and ~\eqref{Eq:VBA_Proportionalities5_IS},  
\begin{subequations}
\begin{align}
%\left\{\barr{ll}
&q_1(\rfb) \;\;\; \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon}) \; q_5(\rvb_{\rz})} \right\rbrace,
\label{Eq:VBA_Proportionalities1_IS}
\\[4pt]
&q_2(\rzb) \;\;\; \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon}) \; q_5(\rvb_{\rz})} \right\rbrace,
\label{Eq:VBA_Proportionalities2_IS}
\\[4pt]  
&q_{3j}(\rv_{\rxi_\red{j}}) \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_{3-j}(\rvb_{\rxi_\rj}) \; q_4(\rvb_{\repsilon}) \; q_5(\rvb_{\rz})} \right\rbrace,
\nonumber 
\\&
\hspace{341pt}j \in \left\lbrace 1,2 \ldots, M \right\rbrace,  
\label{Eq:VBA_Proportionalities3_IS}
\\[4pt]
&q_{4i}(\rv_{\repsilon_\ri}) \; \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_{4-i}(\rvb_{\repsilon_\ri}) \; q_5(\rvb_{\rz})} \right\rbrace,
\nonumber 
\\&
\hspace{342pt}i \in \left\lbrace 1,2 \ldots, N \right\rbrace,
\label{Eq:VBA_Proportionalities4_IS}
\\[4pt]
&q_{5j}(\rv_{\rz_\red{j}}) \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon}) \; q_{5-j}(\rvb_{\rz_\rj})} \right\rbrace,
\nonumber 
\\&
\hspace{341pt}j \in \left\lbrace 1,2 \ldots, M \right\rbrace,
\label{Eq:VBA_Proportionalities5_IS}
\end{align}
\end{subequations}
using the notations:
\beq
q_{3-j}(\rv_{\rxi_\red{j}})=\displaystyle \prod_{k=1,k \neq j}^{M} q_{3k}(\rv_{\rxi_\red{k}})
\;\;\;;\;\;\;
q_{4-i}(\rv_{\repsilon_\ri})=\displaystyle \prod_{k=1,k \neq i}^{N} q_{4k}(\rv_{\repsilon_\rk})
\;\;\;;\;\;\;
q_{5-j}(\rv_{\rz_\red{j}})=\displaystyle \prod_{k=1,k \neq j}^{M} q_{5k}(\rv_{\rz_\red{k}})
\label{Eq:Def_q_Minus_IS}
\eeq
and also
\beq
\biggl\langle u(x) \biggr\rangle_{v(y)}= \displaystyle \int u(x) v(y) \d y. 
\label{Eq:Def_Integral_IS}
\eeq
Via Equation~\eqref{Eq:Def_L_Criterion_IS} and Equation~\eqref{Eq:L_Criterion_IS}, the analytical expression of logarithm of the posterior distribution is obtained, Equation~\eqref{Eq:Log_Posterior_IS}:
\beq
\begin{split}
\ln  p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right)
=&
-
\frac{1}{2}\| \rVb_{\repsilon}^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \|
-
\left( \alpha_{\epsilon} + \frac{3}{2} \right) \sum_{i=1}^{N} \ln \rv_{\repsilon_\ri} 
-
\sum_{i=1}^{N}\frac{\beta_{\epsilon}}{\rv_{\repsilon_\ri}} 
\\&
-
\frac{1}{2}\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
-
\left( \alpha_{\xi} + \frac{3}{2} \right) \sum_{j=1}^{M} \ln \rv_{\rxi_\rj} 
-
\sum_{j=1}^{M}\frac{\beta_{\xi}}{\rv_{\rxi_\rj}}
\\&
-
\frac{1}{2}\| \rVb_{\rz}^{-\frac{1}{2}} \rzb \|
-
\left(\alpha_{z} + \frac{3}{2} \right) \sum_{j=1}^{M} \ln \rv_{\rz_\rj}
-
\sum_{j=1}^{M}\frac{\beta_{f}}{\rv_{\rz_\rj}}
\end{split}
\label{Eq:Log_Posterior_IS}
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%			Computation of q_1(f) I				 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_1(\rfb)$ (first part).}
The proportionality relation corresponding to $q_1(\rfb)$ is established in Equation~\eqref{Eq:VBA_Proportionalities1_IS}. In the expression of $p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right)$ all the terms free of $\rfb$ can be regarded as constants. Via Equation~\eqref{Eq:Log_Posterior_IS} the integral $\left\langle \right\rangle$ defined in Equation~\eqref{Eq:Def_Integral_IS} becomes:
\beq
\begin{split}
\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}
=&
%\\
%&
-\frac{1}{2}
\biggl\langle 
\|\rVb_{\repsilon}^{-\frac{1}{2}} \left(\bgb - \bHb\rfb\right) \|
\biggr\rangle_{ q_4(\rvb_{\repsilon}) }
\\&
-\frac{1}{2}
\biggl\langle 
\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
\biggr\rangle_{ q_2(\rzb) q_3(\rvb_{\rxi}) }.
\end{split}
\label{Eq:q1_Integral_1_IS}
\eeq
Introducing the notations:
\beq
\begin{split}
\rvt_{\rxi_\rj} = \biggl\langle \rv_{\rxi_\rj}^{-1} \biggr\rangle_{q_{3j}\left( \rv_{\rxi_\rj} \right)}
\;\;;\;\;
\rvbt_{\rxi}\;&=\;
\begin{bmatrix}
\rvt_{\rxi_\red{1}} \ldots 
\rvt_{\rxi_\rj} \ldots 
\rvt_{\rxi_\rM}
\end{bmatrix}^T
\;\;;\;\;
\rVbt_{\rxi} = \diag {\rvbt_{\rxi}}\;
\\
\rvt_{\repsilon_\ri}
=
\biggl\langle \rv_{\repsilon_\ri}^{-1} \biggr\rangle_{q_{4i}\left( \rv_{\repsilon_\ri} \right)}
\;\;;\;\;
\rvbt_\repsilon\;&=\;
\begin{bmatrix}
\rvt_{\repsilon_\red{1}}
\ldots 
\rvt_{\repsilon_\ri}
\ldots 
\rvt_{\repsilon_\rN}
\end{bmatrix}^T
\;\;;\;\;
\rVbt_\repsilon = \diag {\rvbt_\repsilon}
\end{split}
\label{Eq:q1_Integral_Not1_IS}
\eeq
the integral from Equation~\eqref{Eq:q1_Integral_1_IS} becomes:
\beq
\begin{split}
\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_2(\rzb) \;q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}
=&
-\frac{1}{2} \|\rVbt_{\repsilon}^{\frac{1}{2}} \left(\bgb - \bHb\rfb\right) \| 
\\&
- 
\frac{1}{2} \biggl\langle \| \rVbt_{\rxi}^{\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|\biggr\rangle_{q_2(\rzb)}.
\end{split}
\label{Eq:q1_Integral_2_IS}
\eeq
Evidently, $\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_2(\rzb) \;q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}$ is a quadratic form with respect to $\rfb$. The proportionality from Equation~\eqref{Eq:VBA_Proportionalities1_IS} leads to the following corollary:
\begin{corollary}
$q_1 \left( \rfb \right)$ is a multivariate Normal distribution.
\label{Co:q1}
\end{corollary} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%			Computation of q_2(z)				 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_2(\rzb)$.}
The proportionality relation corresponding to $q_2(\rzb)$ is established in Equation~\eqref{Eq:VBA_Proportionalities2_IS}. In the expression of $p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right)$ all the terms free of $\rzb$ can be regarded as constants. Via Equation~\eqref{Eq:Log_Posterior_IS} the integral $\left\langle \right\rangle$ defined in Equation~\eqref{Eq:Def_Integral_IS} becomes:
\beq
\begin{split}
\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_1(\rfb) \; q_3(\rvb_{\rxi}) \; q_5(\rvb_{\rz})}
=&
-\frac{1}{2}
\biggl\langle 
\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
\biggr\rangle_{q_1(\rfb) q_3(\rvb_{\rxi}) }
\\&
-\frac{1}{2}
\biggl\langle 
\| \rVb_{\rz}^{-\frac{1}{2}} \rzb \|
\biggr\rangle_{ q_5(\rvb_{\rz}) }.
\end{split}
\label{Eq:q2_Integral_1_IS}
\eeq
Using the notations introduced in Equation~\eqref{Eq:q2_Integral_Not1_IS} and introducing the notations:
\beq
\begin{split}
\rvt_{\rz_\rj} = \biggl\langle \rv_{\rz_\rj}^{-1} \biggr\rangle_{q_{5j}\left( \rv_{\rz_\rj} \right)}
\;\;;\;\;
\rvbt_{\rz}\;&=\;
\begin{bmatrix}
\rvt_{\rz_\red{1}} \ldots 
\rvt_{\rz_\rj} \ldots 
\rvt_{\rz_\rM}
\end{bmatrix}^T
\;\;;\;\;
\rVbt_{\rz} = \diag {\rvbt_{\rz}}\;
\end{split}
\label{Eq:q2_Integral_Not1_IS}
\eeq
the integral from Equation~\eqref{Eq:q2_Integral_1_IS} becomes:
\beq
\begin{split}
\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_2(\rzb) \;q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}
=&
-\frac{1}{2}
\biggl\langle 
\| \rVbt_{\rxi}^{\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
\biggr\rangle_{q_1(\rfb)}
\\&
-\frac{1}{2}
\| \rVbt_{\rz}^{\frac{1}{2}} \rzb \|.
\end{split}
\label{Eq:q2_Integral_2_IS}
\eeq
The norm from the first term in Equation~\eqref{Eq:q2_Integral_2_IS} can be developed as it follows:
\beq
\| \rVbt_{\rxi}^{\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
=
\rfb^T \rVbt_{\rxi} \rfb 
-
2 \rzb^T \bDb^T \rVbt_{\rxi} \rfb
+ \rzb^T \bDb^T \rVbt_{\rxi} \bDb \rzb
=
\| \rVbt_{\rxi}^{\frac{1}{2}} \rfb \|
-
2 \rzb^T \bDb^T \rVbt_{\rxi} \rfb 
+
\| \rVbt_{\rxi}^{\frac{1}{2}} \bDb \rzb \|,
\label{Eq:Norm_Development_IS}
\eeq  
so Equation~\eqref{Eq:q2_Integral_2_IS} can be developed as it follows:
\beq
\biggl\langle 
\| \rVbt_{\rxi}^{\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
\biggr\rangle_{q_1(\rfb)}
=
\biggl\langle 
\| \rVbt_{\rxi}^{\frac{1}{2}} \rfb \|
\biggr\rangle_{q_1(\rfb)}
-
2 \rzb^T \bDb^T \rVbt_{\rxi} \biggl\langle \rfb \biggr\rangle_{q_1(\rfb)}
+
\| \rVbt_{\rxi}^{\frac{1}{2}} \bDb \rzb \|.
\label{Eq:q2_Integral_3_IS}
\eeq  
Using Corollary~\eqref{Co:q1}, we can easily compute $\left\langle 
\| \rVbt_{\rxi}^{\frac{1}{2}} \rfb \|
\right\rangle_{q_1(\rfb)}$ and $\left\langle \rfb \right\rangle_{q_1(\rfb)}$. For the multivariate Normal distribution $q_1(\rfb)$ we will denote $\rfbh$ the corresponding mean and $\Sigmabh_{\fb}$, obtaining:
\beq
\biggl\langle \rfb \biggr\rangle_{q_1(\rfb)} 
=
\rfbh
\;\;\;\;\; ; \;\;\;\;\;
\biggl\langle 
\| \rVbt_{\rxi}^{\frac{1}{2}} \rfb \|
\biggr\rangle_{q_1(\rfb)}
=
\| \rVbt_{\rxi}^{\frac{1}{2}} \rfbh \| 
+
\Tr{\rVbt_{\rxi}\Sigmabh_{\fb}} 
\label{Eq:q2_Integral_4_IS}
\eeq
From Equations~\eqref{Eq:q2_Integral_2_IS},~\eqref{Eq:q2_Integral_3_IS},~\eqref{Eq:q2_Integral_4_IS} we obtain:
\beq
\begin{split}
\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_2(\rzb) \;q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}
=&
-\frac{1}{2} \| \rVbt_{\rxi}^{\frac{1}{2}} \rfbh \| 
+
-\frac{1}{2} \Tr{\rVbt_{\rxi}\Sigmabh_{\fb}}
+ \rzb^T \bDb^T \rVbt_{\rxi} \rfbh
\\&
-\frac{1}{2} \| \rVbt_{\rxi}^{\frac{1}{2}} \bDb \rzb \|
-\frac{1}{2} \| \rVbt_{\rz}^{\frac{1}{2}} \rzb \|
\end{split}
\label{Eq:q2_Integral_5_IS}
\eeq 
Evidently, $\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_2(\rzb) \;q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}$. The proportionality from Equation~\eqref{Eq:VBA_Proportionalities2_IS} leads to the following corollary:
\begin{corollary}
$q_2 \left( \rzb \right)$ is a multivariate Normal distribution.
\label{Co:q2}
\end{corollary}
Minimizing the criterion
\beq
J(\rzb) 
=
-\frac{1}{2} \| \rVbt_{\rxi}^{\frac{1}{2}} \rfbh \| 
+
-\frac{1}{2} \Tr{\rVbt_{\rxi}\Sigmah_{\rfb}}
+ \rzb^T \bDb^T \rVbt_{\rxi} \rfbh
-\frac{1}{2} \| \rVbt_{\rxi}^{\frac{1}{2}} \bDb \rzb \|
-\frac{1}{2} \| \rVbt_{\rz}^{\frac{1}{2}} \rzb \|,
\label{Criterion_q2_IS}
\eeq
leads to the analytical expression of the corresponding mean, denoted $\rzbh$:
\beq
\begin{split}
\frac{\partial J(\rzb) }{\partial \rzb} = 0
&\Leftrightarrow
\frac{\partial }{\partial \rzb} \rfbh^T \rVbt_{\rxi}^T \bDb \rzb
-\frac{1}{2} \frac{\partial }{\partial \rzb} \| \rVbt_{\rxi}^{\frac{1}{2}} \bDb \rzb \|
-\frac{1}{2} \frac{\partial }{\partial \rzb} \| \rVbt_{\rz}^{\frac{1}{2}} \rzb \|
=0
\Leftrightarrow
\bDb^T \rVbt_{\rxi} \rfbh - \bDb^T \rVbt_{\rxi} \bDb \rzb - \rVbt_{\rz} \rzb
=0
\\&
\Leftrightarrow
\left( \bDb^T \rVbt_{\rxi} \bDb + \rVbt_{\rz} \right) \rzb = \bDb^T \rVbt_{\rxi} \rfbh
\Rightarrow
\rzbh = \left( \bDb^T \rVbt_{\rxi} \bDb + \rVbt_{\rz} \right)^{-1} \bDb^T \rVbt_{\rxi} \rfbh
\end{split}
\label{MeanComputation_q2_IS}
\eeq
The variance can be obtained by identification:
\beq
\Sigmabh_{\zb} = \left( \bDb^T \rVbt_{\rxi} \bDb + \rVbt_{\rz} \right)^{-1}
\eeq
Finally, we conclude that $q_2(\rzb)$ is a multivariate Normal distribution with the following parameters:
\beq
q_2(\rzb) = \Nc\left( \rzb | \rzbh, \Sigmabh_{\zb} \right),
\left\{\barr{ll}
\rzbh = \left( \bDb^T \rVbt_{\rxi} \bDb + \rVbt_{\rz} \right)^{-1} \bDb^T \rVbt_{\rxi} \rfbh,
\\[10pt]
\Sigmabh_{\zb} = \left( \bDb^T \rVbt_{\rxi} \bDb + \rVbt_{\rz} \right)^{-1}.
\earr\right.
\label{Eq:q2_Analytical_1_IS}
\eeq
We note that both the expressions of the mean $\rzbh$ and variance $\Sigmabh_{\zb}$ depend on expectancies corresponding to the three variances of the hierarchical model. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%			Computation of q_1(f) II			 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_1(\rfb)$ (second part).}
We come back for computing the parameters of the multivariate Normal distribution $q_1(\rfb)$. Using the fact that $q_2(\rzb)$ was proved a multivariate Normal distribution, the norm from the latter term in Equation~\eqref{Eq:q1_Integral_2_IS} can be computed. The norm was developed in Equation~\eqref{Eq:Norm_Development_IS} and the computation of the integral uses the particular form of $q_2(\rzb)$:
\beq
\begin{split}
\biggl\langle 
\| \rVbt_{\rxi}^{\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
\biggr\rangle_{q_2(\rzb)}
&=
\| \rVbt_{\rxi}^{\frac{1}{2}} \rfb \|
-
2 \rfb^T \rVbt_{\rxi}^T \bDb \biggl\langle \rzb \biggr\rangle_{q_2(\rzb)}
+
\biggl\langle 
\| \rVbt_{\rxi}^{\frac{1}{2}} \bDb \rzb \|
\biggr\rangle_{q_2(\rzb)}
\\&
=
\| \rVbt_{\rxi}^{\frac{1}{2}} \rfb \|
-
2 \rzbh \bDb^T \rVbt_{\rxi} \rfb
+  
\| \rVbt_{\rxi}^{\frac{1}{2}} \bDb \rzbh \|
+
\Tr{\bDb^T \rVbt_{\rxi} \bDb \Sigmabh_{\zb}}.
\end{split}
\label{Eq:q1_Integral_3_IS}
\eeq
Minimizing the criterion
\beq
J(\rfb) 
=
-\frac{1}{2} \| \rVbt_{\repsilon}^{\frac{1}{2}} \left( \bgb - \bHb \rfb \right) \| 
-\frac{1}{2}\| \rVbt_{\rxi}^{\frac{1}{2}} \rfb \|
+ \rzbh \bDb^T \rVbt_{\rxi} \rfb
-\frac{1}{2} \| \rVbt_{\rxi}^{\frac{1}{2}} \bDb \rzbh \|
-\frac{1}{2} \Tr{\bDb^T \rVbt_{\rxi} \bDb \Sigmabh_{\zb}}
\label{Criterion_q1_IS}
\eeq
leads to the analytical expression of the corresponding mean, denoted $\rzbh$:
\beq
\begin{split}
\frac{\partial J(\rfb) }{\partial \rfb} = 0
&\Leftrightarrow
-\frac{1}{2} \frac{\partial }{\partial \rfb} \| \rVbt_{\repsilon}^{\frac{1}{2}} \left( \bgb - \bHb \rfb \right) \|
-\frac{1}{2} \frac{\partial }{\partial \rfb} \| \rVbt_{\rxi}^{\frac{1}{2}} \rfb \|
+ \frac{\partial }{\partial \rfb} \rzbh^T \bDb^T \rVbt_{\rxi} \rfb 
=0
\\&
\Leftrightarrow
\bHb^T \rVbt_{\repsilon} \bgb
- \bHb^T \rVbt_{\repsilon} \bHb \rfb
- \rVbt_{\rxi} \rfb
+ \rVbt_{\rxi}^T \bDb \rzbh  
=0
\\&
\Leftrightarrow
\left( \bHb^T \rVbt_{\repsilon} \bHb + \rVbt_{\rxi} \right) \rfb = \rVbt_{\rxi}^T \bDb \rzbh + \bHb^T \rVbt_{\repsilon} \bgb
\Rightarrow
\rfbh = \left( \bHb^T \rVbt_{\repsilon} \bHb + \rVbt_{\rxi} \right)^{-1} \left( \rVbt_{\rxi}^T \bDb \rzbh + \bHb^T \rVbt_{\repsilon} \bgb \right)
\end{split}
\label{MeanComputation_q1_IS}
\eeq
The variance can be obtained by identification:
\beq
\Sigmabh_{\fb} = \left( \bHb^T \rVbt_{\repsilon} \bHb + \rVbt_{\rxi} \right)^{-1}
\eeq
Finally, we conclude that $q_1(\rfb)$ is a multivariate Normal distribution with the following parameters:
\beq
q_1(\rfb) = \Nc\left( \rfb | \rfbh, \Sigmabh_{\fb} \right),
\left\{\barr{ll}
\rfbh = \left( \bHb^T \rVbt_{\repsilon} \bHb + \rVbt_{\rxi} \right)^{-1} \left( \rVbt_{\rxi}^T \bDb \rzbh + \bHb^T \rVbt_{\repsilon} \bgb \right),
\\[10pt]
\Sigmabh_{\fb} = \left( \bHb^T \rVbt_{\repsilon} \bHb + \rVbt_{\rxi} \right)^{-1}.
\earr\right.
\label{Eq:q1_Analytical_1_IS}
\eeq
We note that both the expressions of the mean $\rfbh$ and variance $\Sigmabh_{\fb}$ depend on expectancies corresponding to the three variances of the hierarchical model. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%			Computation of q_3(v_xi)		     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_{3j}(\rv_{\rxi_\rj})$.}
The proportionality relation corresponding to $q_{3j}(\rv_{\rxi_\rj})$ is presented in established in Equation~\eqref{Eq:VBA_Proportionalities3_IS}. In the expression of $p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right)$ all the terms free of $\rv_{\rxi_\rj}$ can be regarded as constants. Via Equation~\eqref{Eq:Log_Posterior_IS} the integral defined in Equation~\eqref{Eq:Def_Integral_IS} becomes:
\beq
\begin{split}
\biggl\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_{3-j}(\rvb_{\rxi_\rj})}
&=
-
\frac{1}{2} \biggl\langle \| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \| \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_{3-j}(\rvb_{\rxi_\rj})}
\\&
-
\left( \alpha_{\xi} + \frac{3}{2} \right) \ln \rv_{\rxi_\rj} 
-
\beta_{\xi} \rv_{\rxi_\rj}^{-1}
\end{split}
\label{Eq:q3_Integral_1_IS}
\eeq
Introducing the notations:
\beq
\rvbt_{\rxi_{-\rj}}^{-1}=
\begin{bmatrix}
\rvt_{\rxi_\red{1}}^{-1} \;
\ldots \;
\rvt_{\rxi_{\rj-\red{1}}}^{-1} \;
\rv_{\rxi_\rj}^{-1}  \;
\rvt_{\rxi_{\rj+\red{1}}}^{-1}  \;
\ldots \;
\rvt_{\rxi_\rM}^{-1}
\end{bmatrix}^T
\;\; ; \;\;
\rVbt_{\rxi_{-\rj}}=
\mbox{diag}\left(\rvbt_{\rxi_{-\rj}}^{-1} \right)
\label{Eq:q3_Integral_Not1_IS}
\eeq
the integral $\biggl\langle \| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \| \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_{3-j}(\rvb_{\rxi_\rj})}$ can be written:
\beq
\biggl\langle \| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \| \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_{3-j}(\rvb_{\rxi_\rj})}
= 
\biggl\langle \| \rVbt_{\rxi_{-\rj}}^{\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \| \biggr\rangle_{q_1(\rfb) \; q_2(\rzb)}
\eeq 
Considering that $q_1(\rfb)$ and $q_2(\rzb)$ are multivariate Normal distributions, Equations~\eqref{Eq:q1_Analytical_1_IS} and~\eqref{Eq:q2_Analytical_1_IS} and considering the development of the norm Equations~\eqref{Eq:Norm_Development_IS}, we have:  
\beq
\begin{split}
\biggl\langle \| \rVbt_{\rxi_{-\rj}}^{\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \| & \biggr\rangle_{q_1(\rfb) \; q_2(\rzb)}
=
\biggl\langle \| \rVbt_{\rxi_{-\rj}}^{\frac{1}{2}} \rfb \|\biggr\rangle_{q_1(\rfb)}
- 2 \biggl\langle \rzb^T \bDb^T \rVbt_{\rxi_{-\rj}} \rfb \biggr\rangle_{q_1(\rfb) \; q_2(\rzb)}
+ \biggl\langle \| \rVbt_{\rxi_{-\rj}}^{\frac{1}{2}} \bDb \rzb \|\biggr\rangle_{q_2(\rzb)}=
\\&
=
\| \rVbt_{\rxi_{-\rj}}^{\frac{1}{2}} \rfbh \|
+\Tr{\rVbt_{\rxi_{-\rj}}\Sigmabh_{\fb}}
-2\rzbh^T \bDb^T \rVbt_{\rxi_{-\rj}} \rfbh
+\| \rVbt_{\rxi_{-\rj}}^{\frac{1}{2}} \bDb \rzbh \|
+\Tr{\bDb^T \rVbt_{\rxi_{-\rj}} \bDb \Sigmabh_{\zb}}
=
\\&
=
C
+\rv_{\rxi_{\rj}}^{-1} \rfh_{\rj}^2 
+\rv_{\rxi_{\rj}}^{-1} \Sigmah_{f_{jj}}
-2\rv_{\rxi_{\rj}}^{-1} \rzbh^T \bDb_{\bj}^T \rfh_{\rj}
+\rv_{\rxi_{\rj}}^{-1} \| \bDb_{\bj} \rzbh \|
+\rv_{\rxi_{\rj}}^{-1} \sum_{k=1}^{M} \sum_{i=1}^{M} \bd_{\bj\bk} \bd_{\bj\bi} \Sigmah_{z_{ik}} 
\label{Eq:q3_Integral_2_IS}
\end{split}
\eeq
where $C$ denotes terms not containing $\rv_{\rxi_{\rj}}$ and $\bDb_{\bj}$ denotes the line $j$ of the matrix $\bDb$. From Equation~\eqref{Eq:q3_Integral_1_IS} and Equation~\eqref{Eq:q3_Integral_2_IS}: 
\beq
\begin{split}
\biggl\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi},& \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_{3-j}(\rvb_{\rxi_\rj})}
=
- \left( \alpha_{\xi} + \frac{3}{2} \right) \ln \rv_{\rxi_\rj} 
\\&
- \left( \beta_{\xi} + \frac{1}{2} \left[ \rfh_{\rj}^2 
+ \Sigmah_{f_{jj}} - \rzbh^T \bDb_{\bj}^T \rfh_{\rj}
+ \| \bDb_{\bj} \rzbh \| + \sum_{k=1}^{M} \sum_{i=1}^{M} \bd_{\bj\bk} \bd_{\bj\bi} \Sigmah_{z_{ik}} \right] \right) \rv_{\rxi_\rj}^{-1}
\end{split}
\eeq
from which it can establish the proportionality corresponding to $q_{3j}(\rv_{\rxi_\rj})$:
\beq
q_{3j}(\rv_{\rxi_\rj})
\propto
\rv_{\rxi_\rj}^{-\left( \alpha_{\xi} + \frac{3}{2} \right)}
\exp
\left\lbrace 
-
\frac{\beta_{\xi} + \frac{1}{2} \left( \rfh_{\rj}^2 
+ \Sigmah_{f_{jj}} - 2 \rzbh^T \bDb_{\bj}^T \rfh_{\rj}
+ \| \bDb_{\bj} \rzbh \| + \sum_{k=1}^{M} \sum_{i=1}^{M} \bd_{\bj\bk} \bd_{\bj\bi} \Sigmah_{z_{ik}} \right)}{\rv_{\rxi_\rj}}
\right\rbrace,
\eeq
leading to the conclusion that $q_{3j}(\rv_{\rxi_\rj})$ is an Inverse Gamma distribution with the following shape and scale parameters:
\beq
q_{3j}(\rv_{\rxi_\rj})=\Ic\Gc\left(\rv_{\rxi_\rj}|\alphah_{\xi_j},\betah_{\xi_j}\right),
\left\{\barr{ll}
\alphah_{\xi_j} = \alpha_{\xi} + \frac{3}{2}
\\[10pt]
\betah_{\xi_j} = \beta_{\xi} + \frac{1}{2} \left( \rfh_{\rj}^2 
+ \Sigmah_{f_{jj}} - 2\rzbh^T \bDb_{\bj}^T \rfh_{\rj}
+ \| \bDb_{\bj} \rzbh \| + \sum_{k=1}^{M} \sum_{i=1}^{M} \bd_{\bj\bk} \bd_{\bj\bi} \Sigmah_{z_{ik}} \right)
\earr\right.
\label{Eq:q3_Analytical_1_IS}
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%		Computation of q_4(v_epsilon)		     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_{4i}(\rv_{\repsilon_\ri})$.}
The proportionality relation corresponding to $q_{4i}(\rv_{\repsilon_\ri})$ is presented in established in Equation~\eqref{Eq:VBA_Proportionalities4_IS}. In the expression of $p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right)$ all the terms free of $\rv_{\repsilon_\ri}$ can be regarded as constants. Via Equation~\eqref{Eq:Log_Posterior_IS} the integral defined in Equation~\eqref{Eq:Def_Integral_IS} becomes:
\beq
\begin{split}
\biggl\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_{4-i}(\rvb_{\repsilon_\ri})}
=&
-
\frac{1}{2} \biggl\langle \| \rVb_{\repsilon}^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \| \biggr\rangle_{q_1(\rfb) \; q_{4-i}(\rvb_{\repsilon_\ri})}
\\&
-
\left( \alpha_{\epsilon} + \frac{3}{2} \right)  \ln \rv_{\repsilon_\ri} 
-
\frac{\beta_{\epsilon}}{\rv_{\repsilon_\ri}} 
\end{split}
\label{Eq:q4_Integral_1_IS}
\eeq
Introducing the notations:
\beq
\rvbt_{\repsilon_{-\ri}}^{-1}=
\begin{bmatrix}
\rvt_{\repsilon_\red{1}}^{-1} \;
\ldots \;
\rvt_{\repsilon_{\ri-\red{1}}}^{-1} \;
\rv_{\repsilon_\ri}^{-1}  \;
\rvt_{\repsilon_{\ri+\red{1}}}^{-1}  \;
\ldots \;
\rvt_{\repsilon_\rN}^{-1}
\end{bmatrix}^T
\;\; ; \;\;
\rVbt_{\repsilon_{-\ri}}=
\mbox{diag}\left(\rvbt_{\repsilon_{-\ri}}^{-1} \right)
\label{Eq:q4_Integral_Not1_IS}
\eeq
the integral $\biggl\langle \| \rVb_{\repsilon}^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \| \biggr\rangle_{q_1(\rfb) \; q_{4-i}(\rvb_{\repsilon_\ri})}$ can be written:
\beq
\biggl\langle \| \rVb_{\repsilon}^{-\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \| \biggr\rangle_{q_1(\rfb) \; q_{4-i}(\rvb_{\repsilon_\ri})}
= 
\biggl\langle \| \rVbt_{\repsilon_{-\ri}}^{\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \| \biggr\rangle_{q_1(\rfb)}
\eeq 
Considering that $q_1(\rfb)$ is a multivariate Normal distribution, Equations~\eqref{Eq:q1_Analytical_1_IS} we have:  
\beq
\begin{split}
\biggl\langle \| \rVbt_{\repsilon_{-\ri}}^{\frac{1}{2}} \left( \bgb - \bHb\rfb \right) \| \biggr\rangle_{q_1(\rfb)}
&=
\| \rVbt_{\repsilon_{-\ri}}^{\frac{1}{2}} \left( \bgb - \bHb\rfbh \right) \|
+ \Tr{\bHb^T \rVbt_{\repsilon_{-\ri}} \bHb \Sigmabh_{\fb}}
\\&
=C +
\rv_{\repsilon_\ri}^{-1} \left( \bg_\bi - \bHb_\bi \rfbh \right)^2
+ 
\rv_{\repsilon_\ri}^{-1}\bHb_\bi \Sigmabh \bHb_\bi^T
\label{Eq:q4_Integral_2_IS}
\end{split}
\eeq
where $C$ denotes terms not containing $\rv_{\repsilon_{\ri}}$ and $\bHb_{\bi}$ denotes the line $i$ of the matrix $\bHb$. From Equation~\eqref{Eq:q4_Integral_1_IS} and Equation~\eqref{Eq:q4_Integral_2_IS}: 
\beq
\begin{split}
\biggl\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_{4-i}(\rvb_{\repsilon_\ri})}
=
C &- \left( \alpha_{\epsilon} + \frac{3}{2} \right) \ln \rv_{\repsilon_\ri} 
\\&
-\left( \beta_{\epsilon} + \frac{1}{2} \left[ 
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2 + \bHb_\bi \Sigmabh_{\fb} \bHb_\bi^T \right] \right) \rv_{\repsilon_\ri}^{-1}
\end{split}
\eeq
from which it can establish the proportionality corresponding to $q_{4i}(\rv_{\repsilon_\ri})$:
\beq
q_{4i}(\rv_{\repsilon_\ri})
\propto
\rv_{\repsilon_\ri}^{-\left( \alpha_{\xi} + \frac{3}{2} \right)}
\exp
\left\lbrace 
-
\frac{ \beta_{\epsilon} + \frac{1}{2} \left[ 
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2 + \bHb_\bi \Sigmabh_{\fb} \bHb_\bi^T \right] }{\rv_{\repsilon_\ri}}
\right\rbrace,
\eeq
leading to the conclusion that $q_{4i}(\rv_{\repsilon_\ri})$ is an Inverse Gamma distribution with the following shape and scale parameters:
\beq
q_{4i}(\rv_{\repsilon_\ri})=\Ic\Gc\left(\rv_{\repsilon_\ri}|\alphah_{\epsilon_i},\betah_{\epsilon_i}\right),
\left\{\barr{ll}
\alphah_{\epsilon_i} = \alpha_{\epsilon} + \frac{3}{2}
\\[10pt]
\betah_{\epsilon_i} = \beta_{\epsilon} + \frac{1}{2} \left[ 
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2 + \bHb_\bi \Sigmabh_{\fb} \bHb_\bi^T \right]
\earr\right.
\label{Eq:q4_Analytical_1_IS}
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%		Computation of q_5(v_z)		     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_{5j}(\rv_{\rz_\rj})$.}
The proportionality relation corresponding to $q_{5j}(\rv_{\rz_\rj})$ is presented in established in Equation~\eqref{Eq:VBA_Proportionalities4_IS}. In the expression of $p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right)$ all the terms free of $\rv_{\rz_\rj}$ can be regarded as constants. Via Equation~\eqref{Eq:Log_Posterior_IS} the integral defined in Equation~\eqref{Eq:Def_Integral_IS} becomes:
\beq
\begin{split}
\biggl\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_2(\rzb) \; q_{5-j}(\rvb_{\rz_\rj})}
=&
-
\frac{1}{2} \biggl\langle \| \rVb_{\rz}^{-\frac{1}{2}} \rzb \|\biggr\rangle_{q_2(\rzb) \; q_{5-j}(\rvb_{\rz_\rj})}
\\&
-
\left(\alpha_{z} + \frac{3}{2} \right) \ln \rv_{\rz_\rj}
-
\frac{\beta_{f}}{\rv_{\rz_\rj}}
\end{split}
\label{Eq:q5_Integral_1_IS}
\eeq
Introducing the notations:
\beq
\rvbt_{\rz_{-\rj}}^{-1}=
\begin{bmatrix}
\rvt_{\rz_\red{1}}^{-1} \;
\ldots \;
\rvt_{\rz_{\rj-\red{1}}}^{-1} \;
\rv_{\rz_\rj}^{-1}  \;
\rvt_{\rz_{\rj+\red{1}}}^{-1}  \;
\ldots \;
\rvt_{\rz_\rM}^{-1}
\end{bmatrix}^T
\;\; ; \;\;
\rVbt_{\rz_{-\rj}}=
\mbox{diag}\left(\rvbt_{\rz_{-\rj}}^{-1} \right)
\label{Eq:q5_Integral_Not1_IS}
\eeq
the integral $\biggl\langle \| \rVb_{\rz}^{-\frac{1}{2}} \rzb \|\biggr\rangle_{q_2(\rzb) \; q_{5-j}(\rvb_{\rz_\rj})}$ can be written:
\beq
\biggl\langle \| \rVb_{\rz}^{-\frac{1}{2}} \rzb \|\biggr\rangle_{q_2(\rzb) \; q_{5-j}(\rvb_{\rz_\rj})}
= 
\biggl\langle \| \rVbt_{\rz_{-\rj}}^{\frac{1}{2}} \rzb \|\biggr\rangle_{q_2(\rzb)}
\eeq 
Considering that $q_2(\rzb)$ is a multivariate Normal distribution, Equations~\eqref{Eq:q2_Analytical_1_IS} we have:  
\beq
\begin{split}
\biggl\langle \| \rVbt_{\rz_{-\rj}}^{\frac{1}{2}} \rzb \|\biggr\rangle_{q_2(\rzb)}
&=
\| \rVbt_{\rz_{-\rj}}^{\frac{1}{2}} \rzbh \|
+ 
\Tr{\rVbt_{\rz_{-\rj}} \Sigmabh_{\zb}}
=
C +
\rv_{\rz_\rj}^{-1} \rz_{\rj}^2
+ 
\rv_{\rz_\rj}^{-1} \Sigmah_{z_{jj}}
\label{Eq:q5_Integral_2_IS}
\end{split}
\eeq
From Equation~\eqref{Eq:q5_Integral_1_IS} and Equation~\eqref{Eq:q5_Integral_2_IS}: 
\beq
\begin{split}
\biggl\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_2(\rzb) \; q_{5-j}(\rvb_{\rz_\rj})}
=
C &- \left( \alpha_{z} + \frac{3}{2} \right) \ln \rv_{\rz_\rj} 
\\&
-\left( \beta_{z} + \frac{1}{2} \left[ \rz_{\rj}^2 + \Sigmah_{z_{jj}} \right] \right) \rv_{\rz_\rj}^{-1}
\end{split}
\eeq
from which it can establish the proportionality corresponding to $q_{5j}(\rv_{\rz_\rj})$:
\beq
q_{5j}(\rv_{\rz_\rj})
\propto
\rv_{\rz_\rj}^{-\left( \alpha_{z} + \frac{3}{2} \right)}
\exp
\left\lbrace 
-
\frac{ \beta_{z} + \frac{1}{2} \left[ \rz_{\rj}^2 + \Sigmah_{z_{jj}} \right]}{\rv_{\rz_\rj}}
\right\rbrace,
\eeq
leading to the conclusion that $q_{5j}(\rv_{\rz_\rj})$ is an Inverse Gamma distribution with the following shape and scale parameters:
\beq
q_{5j}(\rv_{\rz_\rj})=\Ic\Gc\left(\rv_{\repsilon_\ri}|\alphah_{z_j},\betah_{z_j}\right),
\left\{\barr{ll}
\alphah_{z_j} = \alpha_{z} + \frac{3}{2}
\\[10pt]
\betah_{z_j} = \beta_{z} + \frac{1}{2} \left[ \rz_{\rj}^2 + \Sigmah_{z_{jj}} \right].
\earr\right.
\label{Eq:q5_Analytical_1_IS}
\eeq
Equations~\eqref{Eq:q1_Analytical_1_IS},~\eqref{Eq:q2_Analytical_1_IS},~\eqref{Eq:q3_Analytical_1_IS},~\eqref{Eq:q4_Analytical_1_IS} and~\eqref{Eq:q5_Analytical_1_IS} resume the distributions families and the corresponding parameters for $q_1(\rfb)$, $q_2(\rzb)$ ( multivariate Normal distribution), $q_{3j}(\rv_{\rxi_\rj})$, $j\in\left\lbrace 1, 2, \ldots, M \right\rbrace$, $q_{4i}(\rv_{\repsilon_\ri})$, $i\in\left\lbrace 1, 2, \ldots, N \right\rbrace$ and $q_{5j}(\rv_{\rz_\rj})$, $j\in\left\lbrace 1, 2, \ldots, M \right\rbrace$ (Inverse Gamma distributions). However, the parameters corresponding to the multivariate Normal distributions are expressed via $\rVbt_{\rxi}$, $\rVbt_{\repsilon}$ and $\rVbt_{\rz}$ (and by extension all elements forming the three matrices $ \rvt_{\rxi_\rj}$, $j \in \left\lbrace 1, 2, \ldots, M \right\rbrace $, $ \rvt_{\repsilon_\ri}$, $i \in \left\lbrace 1, 2, \ldots, N \right\rbrace $, both defined in Equation~\eqref{Eq:q1_Integral_Not1_IS} and $ \rvt_{\rz_\rj}$, $j \in \left\lbrace 1, 2, \ldots, M \right\rbrace $, defined in Equation~\eqref{Eq:q2_Integral_Not1_IS}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%			   Computation of V				 	 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expressions of $\rVbt_{\rxi}$, $\rVbt_{\repsilon}$ and $\rVbt_{\rz}$.}
For an Inverse Gamma distribution with scale and shape parameters $\alpha$ and $\beta$, $\Ic\Gc\left(x|\alpha, \beta \right)$, the following relation holds:
\beq
\biggl\langle x^{-1} \biggr\rangle_{\Ic\Gc(x|\alpha,\beta)} 
=
\frac{\alpha}{\beta}
\label{Eq:Inverse_Gamma_Integral_IS}
\eeq
The prove of the above relation is done by direct computation, using the analytical expression of the Inverse Gamma Distribution: 
\beq
\begin{split}
\biggl\langle x^{-1} \biggr\rangle_{\Ic\Gc(x|\alpha,\beta)} 
&= 
\int 
x^{-1}
\frac{{\beta}^{\alpha}}{\Gamma(\alpha)}
x^{-\alpha-1}
\exp
\left\lbrace
- \frac{\beta}{x}
\right\rbrace
\d x
=
\frac{{\beta}^{\alpha}}{\Gamma(\alpha)}
\frac{\Gamma(\alpha+1)}{{\beta}^{\alpha+1}}
\int
\frac{{\beta}^{\alpha+1}}{\Gamma(\alpha+1)}
x^{-(\alpha+1)-1}
\exp\left\lbrace -\frac{\beta}{x}\right\rbrace
\d x
=\\
&=
\frac{\alpha}{\beta}
\underbrace{
\int \Ic\Gc(x|\alpha+1,\beta)
}_{1}
\d x
=
\frac{\alpha}{\beta}
\end{split}
\nonumber
\eeq
Since $q_{3j}(\rv_{\rxi_\rj})$, $j\in\left\lbrace 1, 2, \ldots, M \right\rbrace$, $q_{4i}(\rv_{\repsilon_\ri})$, $i\in\left\lbrace 1, 2, \ldots, N \right\rbrace$ and $q_{5j}(\rv_{\rz_\rj})$, $j\in\left\lbrace 1, 2, \ldots, M \right\rbrace$ are Inverse Gamma distributions, with the corresponding parameters $\alphah_{\xi_j}$ and $\betah_{\xi_j}$, $j\in\left\lbrace 1, 2, \ldots, M \right\rbrace$, $\alphah_{\epsilon_j}$ and $\betah_{\epsilon_j}$, $j\in\left\lbrace 1, 2, \ldots, N \right\rbrace$ respectively $\alphah_{z_j}$ and $\betah_{z_j}$, $j\in\left\lbrace 1, 2, \ldots, M \right\rbrace$ the expectancies $\rvt_{\rxi_\rj}$, $\rvt_{\repsilon_\ri}$ and $\rvt_{\rz_\rj}$ can be expressed via the parameters of the two Inverse Gamma distributions using Equation~\eqref{Eq:Inverse_Gamma_Integral_IS}:
\beq
\rvt_{\rxi_\rj}
=
\frac{\alphah_{\xi_\rj}}{\betah_{\xi_\rj}}
\;\;\;;\;\;\;
\rvt_{\repsilon_\ri}
=
\frac{\alphah_{\epsilon_i}}{\betah_{\epsilon_i}}
\;\;\;;\;\;\;
\rvt_{\rz_\rj}
=
\frac{\alphah_{z_j}}{\betah_{z_j}}
\label{Eq:VepsVfExpectanciesIGSMGen_IS}
\eeq
Using the notation introduced in \eqref{Eq:q1_Integral_Not1}:
\beq
\rVbt_{\rxi}=
\begin{bmatrix}
\frac{\alphah_{\xi_1}}{\betah_{\xi_1}} \ldots 0 \ldots 0 \\
\vdots \ddots \vdots \ddots \vdots \\
0 \ldots \frac{\alphah_{\xi_j}}{\betah_{\xi_j}} \ldots 0 \\
\vdots \ddots \vdots \ddots \vdots \\
0 \ldots 0 \ldots \frac{\alphah_{\xi_M}}{\betah_{\xi_M}} \\
\end{bmatrix}
=
\rVbh_{\rf}
\;\;;\;\;
\rVbt_{\repsilon}=
\begin{bmatrix}
\frac{\alphah_{\epsilon_1}}{\betah_{\epsilon_1}} \ldots 0 \ldots 0 \\
\vdots \ddots \vdots \ddots \vdots \\
0 \ldots \frac{\alphah_{\epsilon_i}}{\betah_{\epsilon_i}} \ldots 0 \\
\vdots \ddots \vdots \ddots \vdots \\
0 \ldots 0 \ldots \frac{\alphah_{\epsilon_N}}{\betah_{\epsilon_N}} \\
\end{bmatrix}
=
\rVbh_{\repsilon}
\;\;;\;\;
\rVbt_{\rz}=
\begin{bmatrix}
\frac{\alphah_{z_1}}{\betah_{z_1}} \ldots 0 \ldots 0 \\
\vdots \ddots \vdots \ddots \vdots \\
0 \ldots \frac{\alphah_{z_j}}{\betah_{z_j}} \ldots 0 \\
\vdots \ddots \vdots \ddots \vdots \\
0 \ldots 0 \ldots \frac{\alphah_{z_M}}{\betah_{z_M}} \\
\end{bmatrix}
=
\rVbh_{\rz}
\label{Eq:V_Expectancies_IS}
\eeq
In Equation~\eqref{Eq:V_Expectancies_IS} other notations are introduced for $\rVbt_{\rxi}$,  $\rVbt_{\repsilon}$ and $\rVbt_{\rz}$. Both values were expressed during the model via unknown expectancies, but via Equation~\eqref{Eq:V_Expectancies_IS} those values don't contain any more integrals to be computed. Therefore, the new notations represent the final analytical expressions used for expressing the density functions $q_i$.
Using Equation~\eqref{Eq:V_Expectancies_IS} and Equations~\eqref{Eq:q1_Analytical_1_IS},~\eqref{Eq:q2_Analytical_1_IS} and~\eqref{Eq:q3_Analytical_1_IS}, the final analytical expressions of the separable distributions $q_i$ are presented in Equations~\eqref{Eq:q1_Analytical_2_IS},~\eqref{Eq:q2_Analytical_2_IS} and~\eqref{Eq:q3_Analytical_2_IS}.
\begin{subequations}
\begin{align}
%\left\{\barr{ll}
&q_1(\rfb) = \Nc\left( \rfb | \rfbh, \Sigmabh_{\fb} \right), \;\;\;\;\;\;\;\;\;
\left\{\barr{ll}
\rfbh = \left( \bHb^T \rVbh_{\repsilon} \bHb + \rVbh_{\rxi} \right)^{-1} \left( \rVbh_{\rxi}^T \bDb \rzbh + \bHb^T \rVbh_{\repsilon} \bgb \right),
\\[10pt]
\Sigmabh_{\fb} = \left( \bHb^T \rVbh_{\repsilon} \bHb + \rVbh_{\rxi} \right)^{-1}.
\earr\right.,
\label{Eq:q1_Analytical_2_IS}
\\[4pt]
&q_2(\rzb) = \Nc\left( \rzb | \rzbh, \Sigmabh_{\zb} \right), \;\;\;\;\;\;\;\;\;\;
\left\{\barr{ll}
\rzbh = \left( \bDb^T \rVbh_{\rxi} \bDb + \rVbh_{\rz} \right)^{-1} \bDb^T \rVbh_{\rxi} \rfbh,
\\[10pt]
\Sigmabh_{\zb} = \left( \bDb^T \rVbh_{\rxi} \bDb + \rVbh_{\rz} \right)^{-1}.
\earr\right.,
\label{Eq:q2_Analytical_2_IS}
\\[4pt]
&q_{3j}(\rv_{\rxi_\rj})=\Ic\Gc\left(\rv_{\rxi_\rj}|\alphah_{\xi_j},\betah_{\xi_j}\right),
\left\{\barr{ll}
\alphah_{\xi_j} = \alpha_{\xi} + \frac{3}{2}
\\[10pt]
\betah_{\xi_j} = \beta_{\xi} + \frac{1}{2} \left[ \left( \rfh_{\rj} - \bDb_{\bj} \rzbh \right)^2  + \bDb_\bj \Sigmabh_{\zb} \bDb_\bj^T \right]
\earr\right., j\in\left\lbrace 1, 2, \ldots, M \right\rbrace,
\label{Eq:q3_Analytical_2_IS}
\\[4pt]
&q_{4i}(\rv_{\repsilon_\ri})=\Ic\Gc\left(\rv_{\repsilon_\ri}|\alphah_{\epsilon_i},\betah_{\epsilon_i}\right), \;\;
\left\{\barr{ll}
\alphah_{\epsilon_i} = \alpha_{\epsilon} + \frac{3}{2}
\\[10pt]
\betah_{\epsilon_i} = \beta_{\epsilon} + \frac{1}{2} \left[ 
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2 + \bHb_\bi \Sigmabh_{\fb} \bHb_\bi^T \right]
\earr\right.,i\in\left\lbrace 1, 2, \ldots, N \right\rbrace,
\label{Eq:q4_Analytical_2_IS}
\\[4pt]
&q_{5j}(\rv_{\rz_\rj})=\Ic\Gc\left(\rv_{\repsilon_\ri}|\alphah_{z_j},\betah_{z_j}\right),
\left\{\barr{ll}
\alphah_{z_j} = \alpha_{z} + \frac{3}{2}
\\[10pt]
\betah_{z_j} = \beta_{z} + \frac{1}{2} \left[ \rz_{\rj}^2 + \Sigmah_{z_{jj}} \right].
\earr\right.,j\in\left\lbrace 1, 2, \ldots, M \right\rbrace.
\label{Eq:q5_Analytical_2_IS}
\end{align}
\end{subequations}
Equation~\eqref{Eq:q1_Analytical_2_IS} establishes the dependency between the parameters corresponding to the multivariate Normal distribution $q_1(\rfb)$ and the others parameters involved in the hierarchical model: the mean $\rfbh$ and the covariance matrix $\Sigmabh_{\fb}$ depend on $\rVbh_{\repsilon}$, $\rVbh_{\rxi}$ which, via Equation~\eqref{Eq:V_Expectancies_IS} are defined using $\left\lbrace \alphah_{\xi_j},\betah_{\xi_j}\right\rbrace, j\in \left\lbrace 1, 2, \ldots, M \right\rbrace $ and $\left\lbrace \alphah_{\epsilon_i},\betah_{\epsilon_i}\right\rbrace, i\in \left\lbrace 1, 2, \ldots, N \right\rbrace $ and $\rzbh$. The dependency between the parameters of the multivariate Normal distribution $q_1(\rfb)$ and the parameters of the Inverse Gamma distributions $q_{3j}(\rvb_{\rxi_\rj}) ,j \in \left\lbrace 1,2,\ldots,M \right\rbrace$ and $q_{4i}(\rvb_{\repsilon_\ri}), i \in \left\lbrace 1,2,\ldots,N \right\rbrace$ and the multivariate Normal distribution $q_2(\rzb)$ is presented in Figure~\eqref{Fig:Dependency_Scheme_1_IS}.
\begin{figure}[!htb]
\center
\begin{tabular}{c}
\begin{picture}(220,30)
\put(0,0){\framebox(140,26){$\rzbh,\Sigmabh_{\zb}, \left\lbrace \alphah_{\xi_j},\betah_{\xi_j}\right\rbrace,\left\lbrace \alphah_{\epsilon_i},\betah_{\epsilon_i}\right\rbrace$}}
\put(142,13){\vector(1,0){26}}
\put(168,0){\framebox(56,26){$\rfbh \; , \; \Sigmabh_{\fb}$}}
\end{picture}
\end{tabular}
\caption{Dependency between $q_1(\rfb)$ parameters and $q_{2}(\rzbh)$, $q_{3j}(\rvb_{\rxi_\rj})$ and $q_{4i}(\rvb_{\repsilon_\ri})$ parameters}
\label{Fig:Dependency_Scheme_1_IS}
\end{figure}
Equation~\eqref{Eq:q2_Analytical_2_IS} establishes the dependency between the parameters corresponding to the multivariate Normal distribution $q_2(\rzb)$ and the others parameters involved in the hierarchical model: the mean $\rzbh$ and the covariance matrix $\Sigmabh_{\zb}$ depend on $\rVbh_{\rxi}$, $\rVbh_{\rz}$ which, via Equation~\eqref{Eq:V_Expectancies_IS} are defined using $\left\lbrace \alphah_{\epsilon_i},\betah_{\epsilon_i}\right\rbrace, i \in \left\lbrace 1, 2, \ldots, N \right\rbrace $ and $\left\lbrace \alphah_{z_j},\betah_{z_j}\right\rbrace, j \in \left\lbrace 1, 2, \ldots, M \right\rbrace $ and $\rfbh$. The dependency between the parameters of the multivariate Normal distribution $q_2(\rzb)$ and the parameters of the Inverse Gamma distributions $q_{4i}(\rvb_{\repsilon_\ri}), i \in \left\lbrace 1,2,\ldots,N \right\rbrace$ and $q_{5j}(\rvb_{\rz_\rj}) ,j \in \left\lbrace 1,2,\ldots,M \right\rbrace$ and the multivariate Normal distribution $q_1(\rfb)$ is presented in Figure~\eqref{Fig:Dependency_Scheme_2_IS}.
\begin{figure}[!htb]
\center
\begin{tabular}{c}
\begin{picture}(220,30)
\put(0,0){\framebox(140,26){$\rfbh,\Sigmabh_{\fb}, \left\lbrace \alphah_{\epsilon_i},\betah_{\epsilon_i}\right\rbrace,\left\lbrace \alphah_{z_j},\betah_{z_j}\right\rbrace$}}
\put(142,13){\vector(1,0){26}}
\put(168,0){\framebox(56,26){$\rzbh \; , \; \Sigmabh_{\zb}$}}
\end{picture}
\end{tabular}
\caption{Dependency between $q_2(\rzb)$ parameters and $q_{1}(\rfbh)$, $q_{4i}(\rvb_{\repsilon_\ri})$ and $q_{5j}(\rvb_{\rz_\rj})$ parameters}
\label{Fig:Dependency_Scheme_2_IS}
\end{figure}
Equation~\eqref{Eq:q3_Analytical_2_IS} establishes the dependency between the parameters corresponding to the Inverse Gamma distributions $q_{3j}(\rvb_{\rxi_\rj}) ,j \in \left\lbrace 1, 2, \ldots, M \right\rbrace$ and the others parameters involved in the hierarchical model: the shape and scale parameters $\left\lbrace \alphah_{\xi_j}, \betah_{\xi_j} \right\rbrace, j \in \left\lbrace 1, 2, \ldots, M \right\rbrace$ depend on the element $j$ of the mean $\rfbh$ of the multivariate Normal distribution $q_1(\rfb)$, i.e. $\rfh_{\rj}$ and the mean $\rzbh$ and the covariance matrix $\Sigmabh_{\zb}$ of the multivariate Normal distribution $q_2(\rzb)$, Figure~\eqref{Fig:Dependency_Scheme_3_IS}.
\begin{figure}[!htb]
\center
\begin{tabular}{c}
\begin{picture}(120,30)
\put(0,0){\framebox(46,26){$\rfh_{\rj}, \; \rzbh, \; \Sigmabh_{\zb}$}}
\put(48,13){\vector(1,0){26}}
\put(76,0){\framebox(56,26){$\left\lbrace \alphah_{\xi_j},\betah_{\xi_j}\right\rbrace $}}
\end{picture}
\end{tabular}
\caption{Dependency between $q_{3j}(\rvb_{\rxi_\rj})$ parameters and $q_{1}(\rfb)$ and $q_2(\rzb)$ parameters}
\label{Fig:Dependency_Scheme_3_IS}
\end{figure}
Equation~\eqref{Eq:q4_Analytical_2_IS} establishes the dependency between the parameters corresponding to the Inverse Gamma distributions $q_{4i}(\rvb_{\repsilon_\ri}) ,i \in \left\lbrace 1,2,\ldots,N \right\rbrace$ and the others parameters involved in the hierarchical model: the shape and scale parameters $\left\lbrace \alphah_{\epsilon_i}, \betah_{\epsilon_i} \right\rbrace, i \in \left\lbrace 1, 2, \ldots, N \right\rbrace$ depend on the mean $\rfbh$ and the covariance matrix $\Sigmabh_{\fb}$ of the multivariate Normal distribution $q_1(\rfb)$, Figure~\eqref{Fig:Dependency_Scheme_4_IS}.
\begin{figure}[!htb]
\center
\begin{tabular}{c}
\begin{picture}(120,30)
\put(0,0){\framebox(46,26){$ \rfbh \; , \; \Sigmabh_{\fb}$}}
\put(48,13){\vector(1,0){26}}
\put(76,0){\framebox(56,26){$\left\lbrace \alphah_{\epsilon_i},\betah_{\epsilon_i}\right\rbrace$}}
\end{picture}
\end{tabular}
\caption{Dependency between $q_{4i}(\rvb_{\repsilon_\ri})$ parameters and $q_1(\rfb)$ parameters}
\label{Fig:Dependency_Scheme_4_IS}
\end{figure}
Equation~\eqref{Eq:q5_Analytical_2_IS} establishes the dependency between the parameters corresponding to the Inverse Gamma distributions $q_{5j}(\rvb_{\rz_\rj}) ,j \in \left\lbrace 1,2,\ldots,M \right\rbrace$ and the others parameters involved in the hierarchical model: the shape and scale parameters $\left\lbrace \alphah_{z_j}, \betah_{z_j} \right\rbrace, j \in \left\lbrace 1, 2, \ldots, M \right\rbrace$ depend on the element $j$ of the mean $\rzbh$ and the element $jj$ of the covariance matrix $\Sigmabh_{\zb}$ corresponding to the multivariate Normal distribution $q_2(\rzb)$, Figure~\eqref{Fig:Dependency_Scheme_5_IS}.
\begin{figure}[!htb]
\center
\begin{tabular}{c}
\begin{picture}(120,30)
\put(0,0){\framebox(46,26){$ \rzh_{\rj} \; , \; \Sigmah_{\zb_{jj}}$}}
\put(48,13){\vector(1,0){26}}
\put(76,0){\framebox(56,26){$\left\lbrace \alphah_{z_j},\betah_{z_j}\right\rbrace$}}
\end{picture}
\end{tabular}
\caption{Dependency between $q_{5j}(\rvb_{\rz_\rj})$ parameters and $q_2(\rzb)$ parameters}
\label{Fig:Dependency_Scheme_5_IS}
\end{figure}
\newline
The iterative algorithm obtained via PM estimation is presented Figure~\eqref{Fig:IA_PM_St_nsStL_un_IS}.
\tikzstyle{cloud} = [draw=blue!30!green,fill=orange!12, ellipse, thick, node distance=7em, text width=12em, text centered, minimum height=4em, minimum width=12em]
\tikzstyle{boxbig} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=8.5em, text width=26em, text centered, minimum height=3.6em, minimum width=26em]
\tikzstyle{boxhuge} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=12.6em, text width=29em, text centered, minimum height=3.2em, minimum width=29em]
\tikzstyle{boxsmall} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=9em, text width=9em, text centered, minimum height=4em, minimum width=9em]
%\tikzstyle{fancytitle} =[fill=green!24, text=white, ellipse]
%\tikzstyle{container} = [draw, rectangle, dashed, inner sep=2em]
\tikzstyle{line} = [draw=blue!30!green, -latex']
%\begin{figure}[htbp]
\begin{figure}[!htb]
\centering
\begin{center}
\begin{tikzpicture}[auto]
    \node [boxhuge, scale=0.9] (f) {\Large{$\rfbh = \left( \bHb^T \rVbh_{\repsilon} \bHb + \rVbh_{\rxi} \right)^{-1} \left( \rVbh_{\rxi}^T \bDb \rzbh + \bHb^T \rVbh_{\repsilon} \bgb \right)$}
\\[4.4pt]
\Large{$\Sigmabh_{\fb} = \left( \bHb^T \rVbh_{\repsilon} \bHb + \rVbh_{\rxi} \right)^{-1}$}    
\\[4.4pt]
\normalsize{(a) - update estimated $\rfb$ and covariance matrix $\Sigmabh_{\fb}$} 
};

	\node [boxbig, below of=f, scale=0.9] (z) {\Large{$\rzbh = \left( \bDb^T \rVbh_{\rxi} \bDb + \rVbh_{\rz} \right)^{-1} \bDb^T \rVbh_{\rxi} \rfbh$}
\\[4.4pt]
\Large{$\Sigmabh_{\zb} = \left( \bDb^T \rVbh_{\rxi} \bDb + \rVbh_{\rz} \right)^{-1}
$}    
\\[4.4pt]
\normalsize{(b) - update estimated $\rzb$ and covariance matrix $\Sigmabh_{\zb}$} 
};

    \node [boxbig, below of=z, node distance=11.6em, scale=0.9] (vxi)
{\Large{$ \alphah_{\xi_j} = \alpha_{\xi} + \frac{3}{2} $}
\\[5.1pt]
\Large{$\betah_{\xi_j} = \beta_{\xi} + \frac{1}{2} \left[ \left( \rfh_{\rj} - \bDb_{\bj} \rzbh \right)^2  + \bDb_\bj \Sigmabh_{\zb} \bDb_\bj^T \right]$}
\\[5.1pt]
\normalsize{(c) - update estimated $\Ic\Gc$ parameters corresponding to $\rv_{\rxi_\rj}$} 
};

    \node [boxbig, below of=vxi, node distance=11.6em, scale=0.9] (veps) {\Large{$\alphah_{\epsilon_i} = \alpha_{\epsilon} + \frac{3}{2}$}
\\[5.1pt]
\Large{$\betah_{\epsilon_i} = \beta_{\epsilon} + \frac{1}{2} \left[ 
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2 + \bHb_\bi \Sigmabh_{\fb} \bHb_\bi^T \right]$}
\\[5.1pt]
\normalsize{(d) - update estimated $\Ic\Gc$ parameters corresponding to $\rv_{\repsilon_\ri}$}     
};

    \node [boxbig, below of=veps, node distance=9em, scale=0.9] (vz) {\Large{$\alphah_{z_j} = \alpha_{z} + \frac{3}{2}$}
\\[5.1pt]
\Large{$\betah_{z_j} = \beta_{z} + \frac{1}{2} \left[ \rz_{\rj}^2 + \Sigmah_{z_{jj}} \right]$}
\\[5.1pt]
\normalsize{(e) - update estimated $\Ic\Gc$ parameters corresponding to $\rv_{\rz_\rj}$}     
};

    \node [boxsmall, above right = 0.095cm and -0.7cm of vxi, node distance=17em, scale=0.9] (Vxi) {\Large{$\rVbh_\rxi = \diag {\rvbh_{\rxi}}$}
\\[5pt]
\normalsize{(d)}
};

    \node [boxsmall, below left = -3.95cm and -0.7cm of veps, node distance=17em, scale=0.9] (Veps) {\Large{$\rVbh_\repsilon = \diag {\rvbh_{\repsilon}}$}
\\[5pt]
\normalsize{(e)} 
};

    \node [boxsmall, above right = -0.08cm and 0.86cm of vz, node distance=17em, scale=0.9] (Vz) {\Large{$\rVbh_\rz = \diag {\rvbh_{\rz}}$}
\\[5pt]
\normalsize{(e)} 
};


\node [cloud, above of=f, scale=0.9] (init)
{\Large{Initialization}};  

    \path [line] (f) -- (z)[near start];
    \path [line] (z) -- (vxi);
    \path [line] (vxi) -- (veps);
    \path [line] (veps) -- (vz);    
    \path [line] (Vxi) |- (f);
    \path [line] (Vxi) |- (z);
    \path [line] (Veps) |- (f);
    \path [line] (Vz) |- (z);    
    \path [line] (vxi) -| (Vxi);
    \path [line] (veps) -| (Veps);
    \path [line] (vz) -| (Vz);
    \path [line] (z) -| (f);
    \path [line] (init) -- (f);   
\end{tikzpicture}
\end{center}
\caption{Indirect sparsity (via $\rzb$) - Iterative algorithm corresponding to partial separability PM estimation for Student-t hierarchical model, non-stationary Student-t uncertainties model}
\label{Fig:IA_PM_St_nsStL_un_IS}
\end{figure}
More formal, the iterative algorithm obtained via PM estimation is presented Algorithm~\eqref{Alg:IA_PM_St_nsStL_un_IS}.
\begin{algorithm}
\caption{PM via VBA partial sep. - Student-t hierarchical model, non-stationary Student-t uncertainties model}
\begin{algorithmic}[1]
\Ensure INITIALIZATION $\rfbh^{(0)}$ \Comment{Where $\rfbh^{(0)} = \rfbh$ via a basic estimation method or $\rfbh^{(0)} = \zerob$}
\Function{JMAP}{$\alpha_{\epsilon},\beta_{\epsilon},\alpha_{f},\beta_{f},\bgb,\bHb,\rfb^{(0)},M,N,NoIter$} \Comment{$\alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{f}, \beta_{f}$ are set in modeling phase, Eq.~\eqref{Eq:St_nsStL_un}}

\For{$n = 0$ to ${IterNumb}$}

\For{$j = 1$ to ${M}$}

\State $\rvh_{\rf_\rj}^{(n)} = \frac{\beta_f + \frac{1}{2} (\rfh_\rj^{(n)})^2}{\alpha_f + \frac{3}{2}}$ \Comment{$\rvh_{\rf_\rj}^{(n)}$ is computed using $\alpha_{f},\beta_{f},\rfb^{(n)}$}

\EndFor

\State $\rVbh_\rf^{(n)} = \diag {\rvbh_{\rf}^{(n)}}$ \Comment{The diagonal matrix $\rVbh_\rf^{(n)}$ is build using $\rvh_{\rf_\rj}^{(n)}$, $j \in \left\lbrace 1,2,\ldots, M\right\rbrace$}

\For{$i = 1$ to ${N}$}

\State $\rvh_{\repsilon_\ri}^{(n)} = \frac{\beta_{\epsilon} + \frac{1}{2} \left( \bg_\bi - \bHb_\bi \rfbh^{(n)} \right)^2}{\alpha_{\epsilon} + \frac{3}{2}}$ \Comment{$\rvh_{\repsilon_\ri}^{(n)}$ is computed using $\alpha_{\epsilon},\beta_{\epsilon}, \bg_\bi, \bHb_\bi, \rfb^{(n)}$} 

\EndFor

\State $\rVbh_\repsilon^{(n)} = \diag {\rvbh_{\repsilon}^{(n)}}$ \Comment{The diagonal matrix $\rVbh_\repsilon^{(n)}$ is build using $\rvh_{\repsilon_\ri}^{(n)}$, $i \in \left\lbrace 1,2,\ldots, N \right\rbrace$}

\State $\rfbh^{(n+1)}  = \left( \bHb^T \left(\rVbh_\repsilon^{(n)}\right)^{-1} \bHb + \left( \rVbh_\rf^{(n)}\right)^{-1} \right)^{-1} \bHb^T \left(\rVbh_\repsilon^{(n)}\right)^{-1} \bgb$ \Comment{New value $\rfbh^{(n+1)}$}

\EndFor

\Return $\left( \rfbh^{(n+1)}, \rvbh_\rf^{(n)}, \rvbh_{\repsilon}^{(n)} \right)$ , $n = NoIter$
\EndFunction
\end{algorithmic}
\label{Alg:IA_PM_St_nsStL_un_IS}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%		 PM Estimation full separability		 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\subsubsection{Posterior Mean estimation via VBA, full separability}
\label{Subsubsec:PM_FS_St_nsStL_un_IS}
In this subsection, the Posterior Mean (PM) estimation is again considered, but via a full separable approximation. The posterior distribution is approximated by a full separable distribution $q\left( \rfb, \rzb,  \rvb_{\rxi}, \rvb_{\repsilon}, \rvb_{\rz} \right)$, i.e. a supplementary condition is added in Equation~\eqref{Eq:Posterior_Approximation_Notations1_IS}:
\beq
q_{1}(\rfb) = \prod_{j=1}^{M} q_{1j}(\rf_{\rj})
\;;\;
q_{2}(\rzb) = \prod_{j=1}^{M} q_{2j}(\rz_{\rj})
\;;\;
q_{3}(\rvb_{\rxi}) = \prod_{j=1}^{M} q_{3j}(\rv_{\rxi_\rj})
\;;\;
q_{4}(\rvb_{\repsilon}) = \prod_{i=1}^{N} q_{4i}(\rv_{\repsilon_\ri})
\;;\;
q_{5}(\rvb_{\rz}) = \prod_{j=1}^{M} q_{5j}(\rv_{\rz_\rj})
\label{Eq:Posterior_Approximation_Notations1bis_IS}
\eeq
As in Subsection~\eqref{Subsubsec:PM_PS_St_nsStL_un_IS}, the approximation is done by minimizing of the Kullback-Leibler divergence, Equation~\eqref{Eq:Kullback-Leibler_IS}, via alternate optimization resulting the following proportionalities from Equations~\eqref{Eq:VBA_Proportionalities1bis_IS},~\eqref{Eq:VBA_Proportionalities2bis_IS},~\eqref{Eq:VBA_Proportionalities3bis_IS},~\eqref{Eq:VBA_Proportionalities4bis_IS} and ~\eqref{Eq:VBA_Proportionalities5bis_IS},  
\begin{subequations}
\begin{align}
%\left\{\barr{ll}
&q_{1j}(\rf_{\rj}) \;\;\; \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_{1-j}(\rfb) \; q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon}) \; q_5(\rvb_{\rz})} \right\rbrace,
\label{Eq:VBA_Proportionalities1bis_IS}
\\[4pt]
&q_{2j}(\rz_{\rj}) \;\;\; \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_{2-j}(\rzb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon}) \; q_5(\rvb_{\rz})} \right\rbrace,
\label{Eq:VBA_Proportionalities2bis_IS}
\\[4pt]  
&q_{3j}(\rv_{\rxi_\red{j}}) \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_{3-j}(\rvb_{\rxi_\rj}) \; q_4(\rvb_{\repsilon}) \; q_5(\rvb_{\rz})} \right\rbrace,
\nonumber 
\\&
\hspace{341pt}j \in \left\lbrace 1,2 \ldots, M \right\rbrace,  
\label{Eq:VBA_Proportionalities3bis_IS}
\\[4pt]
&q_{4i}(\rv_{\repsilon_\ri}) \; \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_{4-i}(\rvb_{\repsilon_\ri}) \; q_5(\rvb_{\rz})} \right\rbrace,
\nonumber 
\\&
\hspace{342pt}i \in \left\lbrace 1,2 \ldots, N \right\rbrace,
\label{Eq:VBA_Proportionalities4bis_IS}
\\[4pt]
&q_{5j}(\rv_{\rz_\red{j}}) \propto \; \exp \biggl\lbrace \left\langle \ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z}) \biggr\rangle_{q_1(\rfb) \; q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon}) \; q_{5-j}(\rvb_{\rz_\rj})} \right\rbrace,
\nonumber 
\\&
\hspace{341pt}j \in \left\lbrace 1,2 \ldots, M \right\rbrace,
\label{Eq:VBA_Proportionalities5bis_IS}
\end{align}
\end{subequations}
using the notations introduced in Equation~\eqref{Eq:Def_q_Minus_IS}, Equation~\eqref{Eq:Def_Integral_IS} and Equation~\eqref{Eq:Def_q_Minusbis_IS}.
\beq
q_{1-j}(\rf_{\rj})=\displaystyle \prod_{k=1,k \neq j}^{M} q_{1k}(\rf_\rk)
\;\;;\;\;
q_{2-j}(\rz_{\rj})=\displaystyle \prod_{k=1,k \neq j}^{M} q_{2k}(\rz_\rk)
\label{Eq:Def_q_Minusbis_IS}
\eeq
The analytical expression of logarithm of the posterior distribution $\ln p(\rfb, \rzb, \rvb_\repsilon, \rvb_\rxi, \rvb_\rz | \bgb, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{\xi}, \beta_{\xi}, \alpha_{z}, \beta_{z})$ is obtained in Equation~\eqref{Eq:Log_Posterior_IS}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%			Computation of q_1(f)				 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_{1j}(\rf_{\rj})$.}
The proportionality relation corresponding to $q_1(\rfb)$ is presented in established in Equation~\eqref{Eq:VBA_Proportionalities1bis_IS}. In the expression of $\ln p\left(\rfb, \rvb_\rf, \rvb_\repsilon | \bgb, \alpha_{f}, \beta_{f}, \alpha_{\epsilon}, \beta_{\epsilon} \right)$ all the terms free of $\rf_\ri$ can be regarded as constants:
\beq
\begin{split}
\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) &\biggr\rangle_{q_{1-j}(\rfb) \; q_2(\rzb) \; q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}
=
%\\
%&
-\frac{1}{2}
\biggl\langle 
\|\rVb_{\repsilon}^{-\frac{1}{2}} \left(\bgb - \bHb\rfb\right) \|
\biggr\rangle_{q_{1-j}(\rfb) \; q_4(\rvb_{\repsilon}) }
\\&
-\frac{1}{2}
\biggl\langle 
\| \rVb_{\rxi}^{-\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|
\biggr\rangle_{q_{1-j}(\rfb) q_2(\rzb) q_3(\rvb_{\rxi})}.
\end{split}
\label{Eq:q1_Integral_1bis_IS}
\eeq
Using the notations introduced in Equation~\eqref{Eq:q1_Integral_Not1_IS}, the integral from Equation~\eqref{Eq:q1_Integral_1bis_IS} becomes:
\beq
\begin{split}
\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_{1-j}(\rfb) \; q_2(\rzb) \;q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}
=&
-\frac{1}{2} \biggl\langle \|\rVbt_{\repsilon}^{\frac{1}{2}} \left(\bgb - \bHb\rfb\right) \|\biggr\rangle_{q_{1-j}(\rfb)} 
\\&
- 
\frac{1}{2} \biggl\langle \| \rVbt_{\rxi}^{\frac{1}{2}} \left( \rfb - \bDb\rzb \right) \|\biggr\rangle_{q_{1-j}(\rfb) q_2(\rzb)}.
\end{split}
\label{Eq:q1_Integral_2bis_IS}
\eeq
Evidently, $\biggl\langle p \left( \rfb, \rzb, \rvb_\rxi, \rvb_\repsilon, \rvb_\rz | \bgb, \alpha_{\xi}, \beta_{\xi}, \alpha_{\epsilon}, \beta_{\epsilon}, \alpha_{z}, \beta_{z} \right) \biggr\rangle_{q_2(\rzb) \;q_3(\rvb_{\rxi}) \; q_4(\rvb_{\repsilon})}$ is a quadratic form with respect to $\rf_{\rj}$. The proportionality from Equation~\eqref{Eq:VBA_Proportionalities1bis_IS} leads to the following corollary:
\begin{corollary}
$q_{1j} \left( \rf_{\rj} \right)$ is a Normal distribution.
\label{Co:q1bis}
\end{corollary} 















Using Equation~\eqref{Eq:q1_Integral_Not1_IS}
the integral from Equation~\eqref{Eq:q1_Integral_1bis_IS} becomes:
\beq
\begin{split}
\biggl\langle \ln p(\rfb, \rvb_\rf, \rvb_\repsilon | \bgb, \alpha_{f}, \beta_{f}, \alpha_{\epsilon}, \beta_{\epsilon}) \biggr\rangle_{q_{1-j}(\rf_\rj) \; q_2(\rvb_{\rf}) \; q_3(\rvb_{\repsilon})}
&
= 
-
\frac{1}{2} 
\biggl\langle 
\|\rVbt_{\repsilon}^{-\frac{1}{2}} \left(\bgb - \bHb\rfb\right) \| 
\biggr\rangle_{q_{1-j}(\rf_\rj)} 
-
\frac{1}{2} 
\biggl\langle 
\| \rVbt_{\rf}^{-\frac{1}{2}} \rfb \| 
\biggr\rangle_{q_{1-j}(\rf_\rj)}.
\label{Eq:q1_Integral_1bis1_IS}
\end{split}
\eeq
Considering all the $\rf_\rj$ free terms as constants, the first norm can be written:
\beq
\|\rVbt_{\repsilon}^{-\frac{1}{2}} \left(\bgb - \bHb\rfb\right) \|=
C +
\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2\rf_\rj^2
-2
\bHb^{\bj T} \rVbt_{\repsilon}^{-\frac{1}{2}} \left(\bgb - \bHb^{-\bj}\rfb^{-\rj} \right)\rf_\rj
\label{Eq:q1_Integral_First_Normbis_IS}
\eeq
where $\bHb^{\bj}$ represents the column $j$ of the matrix $\bHb$, $\bHb^{-\bj}$ represents the matrix $\bHb$ except the column $j$, $\bHb^{\bj}$ and $\rfb^{-\rj}$ represents the vector $\rfb$ except the element $\rf_\rj$. 
Introducing the notation
\beq
\rft_\rj 
= \int \rf_\rj q_{1j}(\rf_{\rj})\d \rf_{\rj}
\;\;;\;\;
\rfbt^{-\rj}=
\begin{bmatrix}
\rft_\red{1} \; \ldots \; \rft_\red{j-1} \; \rft_\red{j+1} \; \ldots \; \rft_{\rM}
\end{bmatrix}^T
\label{Eq:q1_Integral_Not1bis_IS}
\eeq
the expectancy of the first norm becomes:
\beq
\biggl\langle
\|\rVbt_{\repsilon}^{-\frac{1}{2}} \left(\bgb - \bHb\rfb\right) \|
\biggr\rangle_{q_{1-j}(\rf_\rj)}
=
C +
\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2\rf_\rj^2
-2
\bHb^{\bj T} \rVbt_{\repsilon}^{-\frac{1}{2}} \left(\bgb - \bHb^{-\bj}\rfbt^{-\rj} \right)\rf_\rj
\label{Eq:q1_Integral_First_Norm_Exbis_IS}
\eeq
Considering all the free $\rf_\rj$ terms as constants, the expectancy for the second norm becomes:  
\beq
\biggl\langle
\| \rVbt_{\rf}^{-\frac{1}{2}} \rfb \|^2
\biggr\rangle_{q_{1-j}(\rf_\rj)}
 = C + \rvt_{\rf_\rj}^{-1} \rf_\rj^2
\label{Eq:q1_Integral_Second_Norm_Exbis_IS}
\eeq
From Equation~\eqref{Eq:VBA_Proportionalities1bis}, ~\eqref{Eq:q1_Integral_1bis1}, ~\eqref{Eq:q1_Integral_First_Norm_Exbis}, and ~\eqref{Eq:q1_Integral_Second_Norm_Exbis} the proportionality for $q_{1j}(\rf_\rj)$ becomes:
\beq
q_{1j}(\rf_\rj) \propto 
\exp \left\lbrace 
\left( 
\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2 + \rvt_{\rf_\rj}^{-1} 
\right)\rf_\rj^2
-2
\bHb^{\bj T} \rVbt_{\repsilon}^{-1} \left(\bgb - \bHb^{-\bj}\rfb^{-\rj} \right)\rf_\rj
\right\rbrace
\label{Eq:q1_Proportionality_IS}
\eeq
Considering the criterion $J(\rf_\rj) = \left( \| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2 + \rvt_{\rf_\rj}^{-1} \right)\rf_\rj^2 -2 \bHb^{\bj T} \rVbt_{\repsilon}^{-1} \left(\bgb - \bHb^{-\bj}\rfb^{-\rj} \right)\rf_\rj$ which is quadratic, we conclude $q_{1j}(\rf_\rj)$ is a Normal distribution.
For computing the mean of the Normal distribution, it is sufficient to compute the solution that minimizes the criterion $J(\rf_\rj)$:
\beq
\frac{\partial J(\rf_\rj)}{\partial \rf_\rj}=0 
\Leftrightarrow
\rfh_\rj = \frac{\bHb^{\bj T} \rVbt_{\repsilon}^{-1} \left( \bgb - \bHb^{-\bj} \rfb^{-\rj} \right)}{\| \rVbt_{\repsilon}^{-\frac{1}{2}}  \bHb^{\bj}\| + \rvt_{\rf}^{-1}}.
\label{Eq:q1_Criterion_Minimization_IS}
\eeq
The variance can be obtained by identification. The analytical expressions for the mean and the variance corresponding to the Normal distributions, $q_1(\rf_\rj)$ are presented in Equation~\eqref{Eq:q1_Analytical_1bis_IS}.
\beq
q_1(\rf_\rj)=\Nc\left(\rf_\rj | \rfh_\rj, \widehat{\mbox{var}}_j \right),
\left\{\barr{ll}
\rfh_\rj = \frac{\bHb^{\bj T} \rVbt_{\repsilon}^{-1} \left(\bgb - \bHb^{-\bj} \rfb^{-\rj} \right)}{\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2 + \rvt_{\rf_\rj}^{-1}}
\\[12pt]
\widehat{\mbox{var}}_j=\frac{1}{\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2 + \rvt_{\rf_\rj}^{-1}}
\earr\right.
,j \in \left\lbrace 1, 2, \ldots, M \right\rbrace
\label{Eq:q1_Analytical_1bis_IS}
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%			Computation of q_2(v_f)				 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_{2j}(\rv_{\rf_\rj})$.}
The proportionality relation corresponding to $q_{2j}(\rv_{\rf_\rj})$ established in Equation~\eqref{Eq:VBA_Proportionalities2bis_IS} refers to $\rv_{\rf_\rj}$, so in the expression of $\ln p\left(\rfb, \rvb_\rf, \rvb_\repsilon | \bgb, \alpha_{f}, \beta_{f}, \alpha_{\epsilon}, \beta_{\epsilon} \right)$ all the terms free of $\rv_{\rf_\rj}$ can be regarded as constants,
\beq
\ln p\left(\rfb, \rvb_\rf, \rvb_\repsilon | \bgb, \alpha_{f}, \beta_{f}, \alpha_{\epsilon}, \beta_{\epsilon} \right) =
C 
-\frac{1}{2}\ln \rv_{\rf_\rj}
-\frac{1}{2} \left\langle \rf_\rj^2\right\rangle_{q_{1j}(\rf_\rj)} \rv_{\rf_\rj}^{-1}
-\left( \alpha_f + 1 \right) \ln \rv_{\rf_\rj}
-\beta_f \rv_{\rf_\rj}^{-1},
\label{Eq:q2_Integral_1bis_IS}
\eeq
so the integral of the logarithm becomes:
\beq
\left\langle \ln p\left(\rfb, \rvb_\rf, \rvb_\repsilon | \bgb, \alpha_{f}, \beta_{f}, \alpha_{\epsilon}, \beta_{\epsilon} \right) \right\rangle_{q_1(\rfb) \; q_{2-j}(\rv_{\rf_\rj}) \; q_3(\rvb_{\repsilon})}
= 
C
- \left(\alpha_f + \frac{3}{2} \right) \ln \rv_{\rf_\rj} 
-\left[ 
\beta_f
+\frac{1}{2} 
\left(
\rfh_\rj^2 + \widehat{\mbox{var}}_j
\right)
\right]
\rv_{\rf_\rj}^{-1}.
\label{Eq:q2_Integral_1bis1_IS}
\eeq
Equation~\eqref{Eq:q2_Integral_1bis1_IS} leads to the conclusion that $q_{2j}(\rv_{\rf_\rj})$ is an Inverse Gamma distribution. Equation~\eqref{Eq:q2_Analytical_1bis_IS} presents the analytical expressions for to the shape and scale parameters corresponding to the Inverse Gamma distribution.
\beq
q_{2j}(\rv_{\rf_\rj})=\Ic\Gc\left(\rv_{\rf_\rj}|\alphah_{f_j},\betah_{f_j}\right),
\left\{\barr{ll}
\alphah_{f_j} = \alpha_f + \frac{1}{2}
\\[10pt]
\betah_{f_j} = \beta_f + \frac{1}{2} 
\left(
\rfh_{\rj}^2 + \widehat{\mbox{var}}_j
\right)
\earr\right.
,j \in \left\lbrace 1, 2, \ldots, M \right\rbrace
\label{Eq:q2_Analytical_1bis_IS}
\eeq
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%			Computation of q_3(v_eps)			 %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computation of the analytical expression of $q_{3i}(\rv_{\repsilon_\ri})$.} 
The proportionality relation corresponding to $q_{3i}(\rv_{\repsilon_\ri})$ established in Equation~\eqref{Eq:VBA_Proportionalities3bis_IS} refers to $\rv_{\repsilon_\ri}$ so in the expression of $\ln p\left(\rfb, \rvb_\rf, \rvb_\repsilon | \bgb, \alpha_{f}, \beta_{f}, \alpha_{\epsilon}, \beta_{\epsilon} \right)$ all the terms free of $\rv_{\repsilon_\ri}$ can be regarded as constants:
\beq
\ln p\left(\rfb, \rvb_\rf, \rvb_\repsilon | \bgb, \alpha_{f}, \beta_{f}, \alpha_{\epsilon}, \beta_{\epsilon} \right) = C 
-\left( \alpha_\epsilon + \frac{3}{2} \right)\ln \rv_{\repsilon_\ri}
-\left(
\beta_\epsilon + \frac{1}{2}\left(\bg_\bi - \bHb_\bi\rfb\right)^2
\right)
\rv_{\repsilon_\ri}^{-1}.
\label{Eq:q3_Integral_1bis_IS}
\eeq
Introducing the notation
\beq
\biggl\langle \rfb \biggr\rangle_{q_1(\rfb)}
=
\begin{bmatrix}
\rfh_{\red{1}}
\ldots
\rfh_\rj
\ldots 
\rfh_\rM
\end{bmatrix}^T
\stackrel{Not}{=}
\rfbh
\;\; ; \;\;
\Sigmabh = \diag {\widehat{\mbox{var}}_j}
\label{Eq:q3_Integral_Not1bis_IS}
\eeq
the expectancy of the logarithm becomes
\beq
\begin{split}
\left\langle
\ln p\left(\rfb, \rvb_\rf, \rvb_\repsilon | \bgb, \alpha_{f}, \beta_{f}, \alpha_{\epsilon}, \beta_{\epsilon} \right) 
\right\rangle_{q_1(\rfb) \; q_2(\rvb_\rf) \; q_{3-i}(\rv_{\repsilon_\ri})}
= C & 
-\left( \alpha_\epsilon + 1 + \frac{1}{2} \right)\ln \rv_{\repsilon_\ri}
\\
&-\left(
\beta_\epsilon + \frac{1}{2}\left[ \bHb_\bi \Sigmabh \bHb_\bi^T
+
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2\right]
\right)
\rv_{\repsilon_\ri}^{-1},
\end{split}
\label{Eq:q3_Integral_1bis1_IS}
\eeq
so and the proportionality relation for $q_{3i}(\rv_{\repsilon_\ri})$ from Equation~\eqref{Eq:VBA_Proportionalities3bis_IS} can be written:
\beq
q_{3i}(\rv_{\repsilon_\ri})
\propto
\rv_{\repsilon_\ri}^{-\left( \alpha_\epsilon + \frac{3}{2} \right)}
\exp
\left\lbrace
-\left(
\beta_\epsilon + \frac{1}{2}\left[ \bHb_\bi \Sigmabh \bHb_\bi^T
+
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2\right]
\right)\rv_{\repsilon_\ri}^{-1}
\right\rbrace
\label{Eq:q3_Proportionality_IS}
\eeq
Equation~\eqref{Eq:q3_Proportionality_IS} shows that $q_{3i}(\rv_{\repsilon_\ri})$ are Inverse Gamma distributions. The analytical expressions of the corresponding parameters are presented in Equation~\eqref{Eq:q3_Analytical_1bis_IS}.
\beq
q_{3i}(\rv_{\repsilon_\ri})=\Ic\Gc\left(\rv_{\repsilon_\ri}|\alphah_{\epsilon_i},\betah_{\epsilon_i}\right),
\left\{\barr{ll}
\alphah_{\epsilon_i} = \alpha_\epsilon + \frac{1}{2}
\\[10pt]
\betah_{\epsilon_i} = \beta_\epsilon + \frac{1}{2}\left[ \bHb_\bi \Sigmabh \bHb_\bi^T
+
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2\right]
\earr\right.
,i \in \left\lbrace 1, 2, \ldots, N \right\rbrace
\label{Eq:q3_Analytical_1bis_IS}
\eeq
Since $q_2(\rv_{\rf_\rj}), j \in \left\lbrace 1, 2, \ldots, M \right\rbrace$ and $q_{3i}(\rv_{\repsilon_\ri}), i \in \left\lbrace 1, 2, \ldots, N \right\rbrace $ are Inverse Gamma distributions, it is easy to obtain analytical expressions for $\rVbt_{\repsilon}^{-1}$, defined in Equation~\eqref{Eq:q1_Integral_Not1_IS} and $ \rvt_{\rf_\rj}^{-1}, j \in \left\lbrace 1, 2, \ldots, M \right\rbrace $, obtaining the same expressions as in Equation~\eqref{Eq:V_Expectancies_IS}. Using Equation~\eqref{Eq:V_Expectancies_IS} and Equations~\eqref{Eq:q1_Analytical_1bis_IS},~\eqref{Eq:q2_Analytical_1bis_IS} and~\eqref{Eq:q3_Analytical_1bis_IS}, the final analytical expressions of the separable distributions $q_i$ are presented in Equations~\eqref{Eq:q1_Analytical_2bis_IS},~\eqref{Eq:q2_Analytical_2bis_IS} and~\eqref{Eq:q3_Analytical_2bis_IS}.
\begin{subequations}
\begin{align}
%\left\{\barr{ll}
&q_1(\rf_\rj)=\Nc\left(\rf_\rj | \rfh_\rj, \widehat{\mbox{var}}_j \right),\;\;\;\;\;\;
\left\{\barr{ll}
\rfh_\rj = \frac{\bHb^{\bj T} \rVbt_{\repsilon}^{-1} \left(\bgb - \bHb^{-\bj} \rfb^{-\rj} \right)}{\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2 + \rvt_{\rf_\rj}^{-1}}
\\[12pt]
\widehat{\mbox{var}}_j=\frac{1}{\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2 + \rvt_{\rf_\rj}^{-1}}
\earr\right.
,j \in \left\lbrace 1, 2, \ldots, M \right\rbrace
\label{Eq:q1_Analytical_2bis_IS}
\\[4pt]
&q_{2j}(\rv_{\rf_\rj})=\Ic\Gc\left(\rv_{\rf_\rj}|\alphah_{f_j},\betah_{f_j}\right),
\left\{\barr{ll}
\alphah_{f_j} = \alpha_f + \frac{1}{2}
\\[10pt]
\betah_{f_j} = \beta_f + \frac{1}{2} 
\left(
\rfh_{\rj}^2 + \widehat{\mbox{var}}_j
\right)
\earr\right.
,j \in \left\lbrace 1, 2, \ldots, M \right\rbrace
\label{Eq:q2_Analytical_2bis_IS}
\\[4pt]
&q_{3i}(\rv_{\repsilon_\ri})=\Ic\Gc\left(\rv_{\repsilon_\ri}|\alphah_{\epsilon_i},\betah_{\epsilon_i}\right),\;\;\;
\left\{\barr{ll}
\alphah_{\epsilon_i} = \alpha_\epsilon + \frac{1}{2}
\\[10pt]
\betah_{\epsilon_i} = \beta_\epsilon + \frac{1}{2}\left[ \bHb_\bi \Sigmabh \bHb_\bi^T
+
\left( \bg_\bi - \bHb_\bi \rfbh \right)^2\right]
\earr\right.
,i \in \left\lbrace 1, 2, \ldots, N \right\rbrace
\label{Eq:q3_Analytical_2bis_IS}
\end{align}
\end{subequations}
Equations~\eqref{Eq:q1_Analytical_2bis_IS},~\eqref{Eq:q2_Analytical_2bis_IS} and~\eqref{Eq:q3_Analytical_2bis_IS} establish dependencies between the parameters of the distributions, very similar to the one presented in Figures~\eqref{Fig:Dependency_Scheme_1_IS},~\eqref{Fig:Dependency_Scheme_2_IS} and~\eqref{Fig:Dependency_Scheme_3_IS}. The iterative algorithm obtained via PM estimation with full separability, is presented Figure~\eqref{Fig:IA_PM_St_nsStL_unbis_IS}.
\tikzstyle{cloud} = [draw=blue!30!green,fill=orange!12, ellipse, thick, node distance=6em, text width=12em, text centered, minimum height=4em, minimum width=12em]
\tikzstyle{boxbig} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=8em, text width=25em, text centered, minimum height=5em, minimum width=25em]
\tikzstyle{box} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=6.5em, text width=21em, text centered, minimum height=5em, minimum width=21em]
\tikzstyle{boxsmall} = [draw=blue!30!green, fill=orange!12, rectangle, rounded corners, thick, node distance=8.5em, text width=11em, text centered, minimum height=5em, minimum width=11em]
%\tikzstyle{fancytitle} =[fill=green!24, text=white, ellipse]
%\tikzstyle{container} = [draw, rectangle, dashed, inner sep=2em]
\tikzstyle{line} = [draw=blue!30!green, -latex']
%\begin{figure}[htbp]
\begin{figure}[!htb]
\centering
\begin{center}
\begin{tikzpicture}[auto]
    \node [boxbig, scale=0.9] (f) {\Large{$ \rfh_\rj = \frac{\bHb^{\bj T} \rVbt_{\repsilon}^{-1} \left(\bgb - \bHb^{-\bj} \rfb^{-\rj} \right)}{\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2 + \rvt_{\rf_\rj}^{-1}}$}
\\[4pt]
\Large{$\widehat{\mbox{var}}_j=\frac{1}{\| \rVbt_{\repsilon}^{-\frac{1}{2}} \bHb^{\bj}\|^2 + \rvt_{\rf_\rj}^{-1}}$}
\\[8pt]
\normalsize{(a) - update estimated $\rf_\rj$ and the corespnding variance $\mbox{var}_j$} 
};

    \node [box, below of=f, node distance=11em, scale=0.9] (vf)
{\Large{$ \alphah_{f_j} = \alpha_f + \frac{1}{2} $}
\normalsize{$\leftarrow$ \textit{ct. during iterations}}
\\[4pt]
\Large{$\betah_{f_j} = \beta_f + \frac{1}{2} \left( \rfh_{\rj}^2 + \widehat{\mbox{var}}_j \right)$}
\\[8pt]
\normalsize{(b) - update estimated $\Ic\Gc$ parameters modelling the variances $\rv_{\rf_\rj}$} 
};

    \node [boxbig, below of=vf, node distance=11em, scale=0.9] (veps) {\Large{$ \alphah_{\epsilon_i} = \alpha_\epsilon + \frac{1}{2} $}
\normalsize{$\leftarrow$ \textit{ct. during iterations}}
\\[4pt]
\Large{$\betah_{\epsilon_i} = \beta_\epsilon + \frac{1}{2}\left[ \bHb_\bi \Sigmabh \bHb_\bi^T + \left( \bg_\bi - \bHb_\bi \rfbh \right)^2\right]$}
\\[8pt]
\normalsize{(c) - update estimated $\Ic\Gc$ parameters modelling the uncertainties variances $\rv_{\repsilon_\ri}$}     
};

    \node [boxsmall, above right = -0.15cm and 0.9cm of vf, node distance=17em, scale=0.9] (Vf) {\Large{$\rVbh_\rf = \diag {\frac{\alphah_{f_j}}{\betah_{f_j}}}$}
\\[8pt]
\normalsize{(d)} 
};

    \node [boxsmall, below left = -4.4cm and 0.3cm of veps, node distance=17em, scale=0.9] (Veps) {\Large{$\rVbh_\repsilon = \diag {\frac{\alphah_{\epsilon_j}}{\betah_{\epsilon_j}}}$}
\\[8pt]
\normalsize{(e)} 
};

	\node [cloud, above of=f, node distance=8em, scale=0.9] (init)
{\Large{Initialization}};  

    \path [line] (f) -- (vf)[near start];
    \path [line] (Vf) |- (f);
    \path [line] (vf) -| (Vf);
    \path [line] (vf) -- (veps);
    \path [line] (Veps) |- (f);
    \path [line] (veps) -| (Veps);
    \path [line] (init) -- (f);    
\end{tikzpicture}
\end{center}
\caption{Iterative algorithm corresponding to PM estimation via VBA - full separability for Student-t hierarchical model, non-stationary Student-t uncertainties model}
\label{Fig:IA_PM_St_nsStL_unbis_IS}
\end{figure}

